Symmetric and Spectral Realizations of Highly Symmetric Graphs

A realization of a graph $G=(V,E)$ is a map $v\colon V\to\Bbb R^d$ that assigns to each vertex a point in $d$-dimensional Euclidean space. We study graph realizations from the perspective of representation theory (expressing certain symmetries), spectral graph theory (satisfying certain self-stress conditions) and rigidity theory (admitting deformations that do not alter the symmetry properties). We explore the connections between these perspectives, with a focus on realizations of highly symmetric graphs (arc-transitive/distance-transitive) and the question of how much symmetry is necessary to ensure that a realization is balanced, spectral, rigid etc. We include many examples to give a broad overview of the possibilities and restrictions of symmetric and spectral graph realizations.

==> v.8 - arXiv/sec/future.tex <==

\tempnewpage
\section{Conclusions and open questions}
\label{sec:future}

%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{img/connections}
%\caption{The conenctions ...}
%\label{fig:conncetions}
%\end{figure}

In this paper we have taken a look at certain classes of highly symmetric graphs, their symmetric, balanced and spectral realizations.
We were able to show that certain sufficiently symmetric realizations are necessarily spectral, or at least balanced.
%This had consequences for certain classes of highly symmetric polytopes.
%For example, we have shown that distance-transitive polytopes are uniquely determined by their edge-graph and realize all its symmetries.
%We were not able to show the same for arc-transitive polytopes, but we expect it to be true.

We list some open questions.
Most of these questions have a formulation in the language of realizations, and another one in the language of arrangement spaces, and can therefore be attacked from both directions.

%\begin{question}
%Is every arc-transitive polytopes $\theta_2$-spectral, and as such
%%
%\begin{myenumerate}
%	\item is uniquely determined by its edge-graph,
%	\item realizes all the symmetries of its edge-graph, and
%	\item is the unique most symmetric realization of its combinatorial type?
%\end{myenumerate}
%\end{question}

%For distance-transitive polytopes, that answer to any of these questions is \emph{yes}.

\begin{question}\label{q:arc_transitive_balanced}
Is every irreducible arc-transitive realization balanced?

Equivalently, are the irreducible subspaces of an arc-transitive group $\Sigma\subseteq\Aut(G)$ always contained in the eigenspaces of $G$?
\end{question}

We have seen that the answer is \emph{yes} if the realization is rigid (\cref{res:rigid_implies_balanced}), full-dimen\-sional (\cref{res:full_local_dimension_is_good}), or distance-transitive (\cref{res:distance_transitive_consequences}).

\begin{question}\label{q:arc_transitive_rigid}
Are arc-transitive $\Aut(G)$-realizations always rigid?

Equivalently, if $G$ is arc-transitive, are there only finitely many $\Aut(G)$-invariant subspaces of $\RR^n$?
\end{question}

The answer is \emph{yes}, if the realization is distance-transitive (\cref{res:distance_transitive_consequences}).

Another interesting question was asked by Du and Fan in \cite{du2013graph}.
It is known that every group appears as the symmetry group of a graph \cite{frucht1939herstellung}, and with only a few exceptions, almost every group appear as the symmetry group of a \emph{vertex-transitive} graph \cite{babai1995automorphism}.
The eigenspaces of such a graph provide a first clue for the placement of the irreducible subspaces of that initial group, but as we have seen, these connections are not necessarily one-to-one.

\begin{question}
For which groups $\Sigma\subseteq\Sym(n)$ can we find a graph whose eigenspaces are exactly the $\Sigma$-irreducible subspaces of $\RR^n$?
\end{question}

We can certainly do this if $\Sigma=\Aut(G)$ for some distance-transitive graph $G$ as seen in \cref{res:eigenspaces_eq_irreducible}.
If such a graph can be constructed efficiently, this would provide an effective tool for computing invariant subspaces of permutation groups.

%\begin{question}
%If $\Sigma\subseteq\Aut(G)$ is arc-transitive, and for every $i\in V$ the stabilizer~of $\{i\}\cup N(i)$ in $\Sigma$ is trivial, is then every \msays{faithful} irreducible $\Sigma$-realization automatically of full local dimension?
%\msays{Yes, the dodecahedron}
%\end{question}

\begin{question}\label{q:dim_fix_ge_2}
Can we classify the realizations that are rigid but have $\dim\Fix(T,\Sigma_i)$ $\ge 2$ for all $i\in V$ (\cf\ \cref{res:fix_rigid}).
\end{question}

The classification of these is linked to the exceptional group structures on spheres that only exist on spheres of dimensions $d\in\{0,1,3\}$.
For example,  the realization in \cref{ex:exception} corresponds to the case $d=1$.
The exact connection is not clear to the author.


\subsection{The orbital technique}
\label{sec:orbitals}

In \cref{sec:realizations} we mentioned that symmetric realizations might not be spectral, but only balanced, and that this is a factor preventing us from obtaining all symemtric realizations with spectral methods alone.

We now briefly describe a technique that might fix this problem, though~we~only have empirical evidence for that.
For example, this technique was used to find the balanced, but non-spectral realizations of the graphs in \cref{ex:hexagonal_prism} and \cref{ex:C6_C6}.

The symmetry group $\Aut(G)$ of a graph acts element-wise on the sets $\{i,j\}\subseteq V$ with $i,j\in V$ (note that $\{i,j\}$ can be a singleton if $i=j$).
An \emph{orbital}\footnote{This is non-standard. Usually, an \emph{orbital} is an orbit of $G$ acting on $V\x V$ rather than ${V\choose 2}\cup V$.} is an orbit of this action, that is, it is of the form
%
$$\mathrm{orb}\{i,j\}:=\{\{\sigma(i),\sigma(j)\}\mid \sigma\in\Aut(G)\}.$$
%
Let $\mathcal O$ denote the set of all orbitals of $\Aut(G)$.
Consider some map $\mathcal O\ni o\mapsto x_o\in \RR$ that assigns a real number to each  orbital (randomly chosen, or, say, algebraically independent) and define the \emph{orbital matrix} $A^{\mathcal O}\in\Bbb R^{n\x n}$ with entries
%
$$A^{\mathcal O}_{ij} = x_{\mathrm{orb}\{i,j\}}.$$
%
Numerical experiments suggest, that the eigenspaces of this matrix are exactly the irreducible invariant subspaces of $\RR^n$ \wrt\ $\Aut(G)$.

While this technique is not perfect (it requires us to obtain the orbitals, which might be a computationally intensive task), it at least provides a finer decomposition of $\RR^n$ than the eigenspaces of the adjacency matrix $A$.

\begin{question}
Are the eigenspaces of the orbital matrix exactly the $\Aut(G)$-irredu\-cible subspaces of $\RR^n$?
\end{question}


%\hrulefill
%
%We have seen that computing the eigenpolytope of a graph might give you the skeleton of a polytope.
%We have investigated this phenomenon only in the case of the $\theta_2$-eigenpolytope.
%The reason: this phenomenon seems to happen only for the second-largest eigenvalue.
%
%\begin{question}
%Is there a $\theta_i$-spectral polytope for an $i\not=2$?
%\end{question}
%
%\begin{question}
%Has every irreducible arc-transitive realization an eigenvalue?
%Or even, has ever irreducible distance-transitive realization an eigenvalue? The latter was shown to be the case if $\diam(G)=2$.
%\end{question}
%
%\begin{question}
%Is every arc-transitive polytope $\theta_2$-spectral?
%\end{question}
%
%\begin{question}
%Are symmetric realizations of arc-transitive graphs always rigid?
%\end{question}
%
%
%\begin{question}
%Is there a combinatorial type of polytopes that has two realizations of maximal degree of symmetry while being incomparable as groups?
%\end{question}
%
%\begin{question}
%Is a rigid polytope always perfect?
%\end{question}
%
%\begin{question}
%If $\Sigma\subseteq\Aut(G)$ is arc-transitive, and for every $i\in V$ the stabilizer~of $\{i\}\cup N(i)$ in $\Sigma$ is trivial, is then every \msays{faithful} irreducible $\Sigma$-realization automatically of full local dimension?
%\msays{Yes, the dodecahedron}
%\end{question}
%
%\begin{question}
%Are there eigenpolytopes with trivial symmetry group?
%\end{question}
%
%For this, one first has to find a graph with no non-trivial symmetries, but whose eigenspaces are still reasonably large.
%Such graphs can be found among the distance-regular graphs.
%However, all spectral graphs among these were already determined by Godsil and all of them turned out to be distance-transitive.
%
%\begin{question}
%What characterizes the spectral polytopes that are not vertex-transitive?
%\end{question}
%
%Only one such polytope is known: the rhombic dodecahedron.
%
%In general, how else can one characterize eigenpolytopes.
%The result of Izmestiev suggests that certain sufficiently regular polytopes are $\theta_2$-eigenpolytopes.
%%
%$$X_{ij}=\frac{\vol{\sigma_i\cap\sigma_j}}{\|v_i\|\|v_j\|\sin\angle(v_i,v_j)}.$$
%
%
%\begin{question}
%Let $P\subset\RR^d$ be a polytope with the following properties:
%%
%\begin{myenumerate}
%	\item $P$ is vertex-transitive,
%	\item $P$ realizes all the symmetries of its edge-graph, and
%	\item $\Aut(P)$ is irreducible.
%\end{myenumerate}
%%
%Is is true that (the combinatorial type of) $P$ has a realization as a spectral polytope?
%\end{question}
%
%\begin{question}
%If $P$ is vertex-transitive with irreducible symmetry group, does it have a balanced realization? What if it is generic? What if it is simplicial?
%
%\end{question}









==> v.8 - arXiv/sec/introduction.tex <==

%\setcounter{section}{-1}
\section{Introduction}

Throughout the paper, $G=(V,E)$ denotes a (simple, undirected) graph with~vertex set $V=\{1,...,n\}$. % and edge set $E\subseteq{V\choose 2}$.
In general, we assume that $G$ has many symmetries, \ie~has a large symmetry group $\Aut(G)\subseteq\Sym(V)$.%, say, at least vertex- or edge-transitive.

A $d$-dimensional \emph{(graph) realization} \mbox{$v\:V\to\RR^d$} is a (not necessarily injective) embedding of the vertices of $G$ into the $d$-dimensional Euclidean space, and one~can consider this as an embedding of the whole graph by imagining the edges embedded as straight lines between the vertices: %, as illustrated in the figure below:
%
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.8\textwidth]{img/C4_realizations_2}
\end{center}
\caption{Several 2-dimensional realizations of the 4-cycle graphs $G=C_4$.}
\label{fig:C4}
\end{figure}

In this paper we shall discuss 
%encounter and work with 
various classes of such \mbox{realizations}, based on ideas from representation theory (\emph{symmetric} and \emph{rigid} realizations), and~spec\-tral graph theory (\emph{balanced} and \emph{spectral} realizations).
%Foremost, these are symmetric/rigid realizations (invoking ideas from representation theory, that is, symmetry), and balanced/spectral realizations (with connections to spectral graph theory).
For a rule of thumb: people are interested in symmetric realizations (because they tell a lot about the structure of $G$), and we can use spectral realization to obtain such (because they are fast and easily computed).
 
That spectral realizations of highly symmetric graphs are always highly symmetric (in a way we make precise below) is well-understood and frequently utilized (\eg\ in graph-drawing algorithms).
It is the other direction which provides interesting unanswered questions: \enquote{How much symmetry is necessary for a realization to be spectral?}.
We are trying to answer this question for several classes of highly symmetric graphs, most successfully in the case of distance-transitive graphs.

%The general goal of this paper is to explore the connections between symmetric realizations ($\Sigma$-realizations, irreducible realizations, rigid/flexible realizations) and spectral/balanced realizations, both of which we introduce now.
Our overall goal is to explore and to better understand the general \mbox{connections} between spectral and symmetric realizations. 
These connections were also \mbox{studied} in \cite{berkolaiko2018eigenspaces} for quantum and edge-weighted graphs, as well as in \cite{du2013graph}. In Section 4 of \cite{du2013graph} the author remarked that the \emph{Petersen graph} enjoys a remarkable property, namely, that all its eigenspaces are $\Aut(G)$-irreducible. This is part of a larger pattern that we discuss in \cref{sec:distance_transitive}.
Another classic reference for spectral properties of highly symmetric graphs is \cite{lovasz1975spectra}.
%, %symmetric and spectral graph realizations, 
%while always having an eye on the mentioned question.
%with a focus on the question on 
%\enquote{how much symmetry is necessary for a realization to be spectral?}. %, which might appear more interesting once we have introduced the relevant terms.
%Both concepts will be introduced in a minute.
Our investigation is supplemented with numerous examples that hopefully provide the reader with some intuition and visualization for these relations. % between combinatorics and geometry.

%We shall be concerned with two classes of realizations: \emph{symmetric} realizations, and \emph{spectral} realizations.
%The purpose of this paper is to investigate connections between these notions in the context of highly symmetric graphs, which for us means \emph{arc-transitive} and~\emph{dis\-tance-transitive} graphs.

A secondary goal is to demonstrate that the concept of the \emph{arrangement space} (as intro\-duced in \cite{winter2019geometry}, see also \cref{def:arrangement_space}) is the appropriate tool for defining and relating these diffe\-rent concepts within a \mbox{common} terminology.~Most~of our results have a second inter\-pretation in terms of arrangement spaces, and many proofs make use of this language.

To better explain our findings, we briefly introduce the most relevant terminology.

%\subsection{The important types of realizations}
%\subsection{Basic concepts and first results}

%A graph is a combinatorial object, and a realization of it is its geometric counterpart.

%The symmetry group of $G$ is denoted $\Aut(G)\subseteq\Sym(V)$, and is a group of permutations on $V$.

\subsection{Symmetric realizations}

Informally, a \enquote{symmetric realization} is a realization that
%The notion of the \enquote{symmetric realization} is an informal term encapsulating all realizations that 
manifests all (or many) of the combinatorial symmetries of $G$ as geometric symmetries. 
%(in this paper we work with the assumption that $G$ has many combinatorial symmetries to begin with, say, $G$ is at least vertex- or edge-transitivity). % or arc-transitive; see \cref{def:transitive}).
Formally, we have %the following:

\begin{definition}
\label{def:symmetric_realization}
For some group $\Sigma\subseteq\Aut(G)$ of symmetries of $G$, a realization is called \emph{$\Sigma$-realization} if there is a linear (orthogonal) representation\footnote{Check out \cref{sec:appendix_rep_theory} for the relevant basics of representation theory.} $T\:\Sigma\to\Ortho(\RR^d)$ with
%
\begin{equation}\label{eq:symmetric}
T_\sigma v_i=v_{\sigma(i)},\quad\text{for all $i\in V$ and $\sigma\in\Sigma$}.
\end{equation}
%
%In most cases, one looses little by assuming $\Sigma=\Aut(G)$.\footnote{When the author wrote this paper, his main motivation (though not explicitly applied in this paper) was an application of this theory to edge-graphs and skeleta of polytopes, especially highly symmetric polytopes. A polytope not necessarily realizes all the symmetries of its edge-graph, and so the generality of a subgroup $\Sigma\subseteq\Aut(G)$ was necessary.}
\end{definition}

Similar constructions, though with a distinct philosophy, are known in finite frame theory as \emph{group frames} (see \cite{waldron2018introduction} for an introduction in finite frame theory, and \cite{waldron2018group} for group frames in specific).

%In our setting (see \cref{sec:realizations}), this representation $T$ will always be uniquely determined from $v$.
%It gives geometry to the combinatorics of $G$.

%This definition formalizes what it means to \enquote{realize combinatorial symmetries}.
A realization can be at most as symmetric as its underlying graph, which happens if we have $\Sigma=\Aut(G)$.
But by choosing appropriate subgroups $\Sigma\subseteq\Aut(G)$, we have fine control over the kind of symmetries that we want to realize.
At least most of the time.
Occasionally, any $\Sigma$-realization is also a $\Sigma'$-realization for some larger group $\Sigma'\supset\Sigma$.
We say that $\Sigma$ cannot be geometrically realized \enquote{in isolation}.
We address this phenomenon in the later sections.

In the example in \cref{fig:C4}, the left-most realizations is void of any symmetries, and can be a $\Sigma$-realization only for $\Sigma=\{\id\}$.
%On the other hand, 
The right-most realization is as symmetric as possible, or, as we are going to say, is an $\Aut(G)$-realization.
In between, we also find realizations that only realize either vertex- or edge-transitivity.
Apparently, in this case, a separation of certain sub-symmetries is possible.
%In between we can find realizations that are vertex- and/or edge-transitive, which means, those are $\Sigma$-realizations for groups $\Sigma\subseteq\Aut(G)$ that act vertex- and/or edge-transitively on $G$.
%Not all $\Sigma\subseteq\Aut(G)$ can be realized without also realizing also a larger $\Sigma'\supset\Sigma$, and this will reappear to us in \cref{sec:distance_transitive}.



%for some group $\Sigma\subseteq\Aut(G)$ of symmetries of $G$, a realization is called \emph{$\Sigma$-realization} if there is a linear (orthogonal) representation $T\:\Sigma\to\Ortho(\RR^d)$ (see \cref{sec:appendix_rep_theory} for the basics on representation theory) with
%%
%\begin{equation}\label{eq:symmetric}
%T_\phi v_i=v_{\phi(i)},\quad\text{for all $i\in V$ and $\phi\in\Sigma$}.
%\end{equation}
%
%Note that $T$ takes on values in the orthogonal matrix, since the intention is that geometric symmetries are isometries.
%
%Now, by comparing the largest subgroup $\Sigma\subseteq\Aut(G)$ for which given realizations are $\Sigma$-realizations, we have a formal way to talk about realizations that are more or less symmetric than others.
%Consider for example the 2-dimensional realizations of the 4-cycle depicted below:
%%
%\begin{center}
%\includegraphics[width=0.8\textwidth]{img/C4_realizations_2}
%\end{center}
%%
%%With this terminology, one can talk formally about more or less symmetric realizations, by comparing the largest subgroup $\Sigma\subseteq\Aut(G)$ for which a given realization is is a $\Sigma$-realization (consider the realizations of the 4-cycle above).
%While the left most realization is a $\Sigma$-realization only for $\Sigma=\{\id\}$, the right~most realization is an $\Aut(G)$-realization, that is, realizes all the symmetries of the graph.
%In between we find realizations that realize only some symmetries of $G$, \eg\ only edge-transitivity or vertex-transitivity, but not both.

Among the symmetric realizations we further distinguish the \emph{irreducible} realiza\-tions (those, for which $T$ is an irreducible representation),
and \emph{rigid} realizations (those, which cannot be continuously deformed without immediately becoming less symmetric; see \cref{def:rigid}).
This notion of rigidity has to be distinguished from the one studies in rigidity theory of frameworks. We do not necessarily require that the edge-length are fixed during a deformation (but this is implicitly true if \eg\ $\Sigma$ acts edge-transitively on $G$; see \cref{sec:arc_transitive}).
Still, frameworks with symmetry constraints have been investigated before \cite{schulze2010symmetry,malestein2014generic,nixon2016symmetry}.

%Our study of rigidity of symmetric graph realizations has to be distinguished from classical rigidity theory of frameworks, with additional symmetry requirements imposed.
%Information on the latter can be found in \cite{schulze2010symmetry}.
%A largest difference: we do not require that edge lengths are preserved (though this can be enforced by symmetry requirements).

%The previously depicted realizations of the 4-cycle differ in the amount of symmetry they realize, which means formally that they differ in the largest group $\Sigma\subseteq\Aut(G)$ for which they are $\Sigma$-realizations.
%The image below shows six more or less symmetric realizations of the 4-cycle graph.
%While the square on the right is a $\Sigma$-realization for all $\Sigma\subseteq\Aut(G)$, the realization on the left is only a $\Sigma$-realization for $\Sigma=\{\id\}$.


\subsection{Balanced and spectral realizations}

Balanced and spectral realizations on the other hand are realizations related to the spectral properties of $G$ (\ie~the eigenvalues and eigenvectors of its adjacency matrix $A$)\footnote{Check out \cref{sec:appendix_spec_theory} for the relevant basics of spectral graph theory.} and do not impose any symmetry constraints a priori.

Spectral realizations have been around for quite some time and were utilized in diverse contexts.
Tracing the historical roots of this notion is beyond the scope of this article.
Naming only a few, there have been applications in data visualization (in particular, graph drawings \cite{koren2003spectral}), semi-definite optimization (\eg\ eigenvalue optimization \cite{boyd2004fastest,goring2008embedded}), geometric combinatorics (\eg\ for equiangular lines \cite{lemmens1991equiangular} and balanced point arrangements \cite{cohn2010point}) as well as polytope theory (in the form of \emph{eigenpolytopes} \cite{godsil1978graphs}).
They are further related to the Lovász theta function \cite{lovasz1979shannon} and the Colin de Verdière graph invariant \cite{van1999colin}.

There are serveral ways to introduce spectral realizations, one of which is via the balanced realizations:


\begin{definition}
\label{def:balanced}
A realization $v\: V\to\RR^d$ is said to be \emph{$\theta$-balanced} (or just \emph{balanced}) for some $\theta\in\RR$ if
%
\begin{equation}
\label{eq:balanced}
\sum_{\mathclap{j\in N(i)}} v_j= \theta v_i,\quad\text{for all $i\in V$}.
\end{equation}
\end{definition}

Equation \eqref{eq:balanced} can be interpreted as a self-stress condition (from which the name \enquote{balanced} can be motived). %, in which certain forces, some directed to the origin, some directed along the edges, cancel out.
Alternatively, and this is the perspective of this paper, \eqref{eq:balanced} can be interpreted as an eigenvalue equation for the adjacency matrix of $G$.
More precisely, if we define the so-called \emph{arrangement matrix}
%
\begin{equation}\label{eq:arrangement_matrix}
M :=\begin{pmatrix}
	\;\horzbar\!\!\!\! & v_1\T & \!\!\!\!\horzbar\;\; \\
	& \vdots & \\[0.4ex]
	\;\horzbar\!\!\!\! & v_n\T & \!\!\!\!\horzbar\;\;
\end{pmatrix}\mathrlap{\in\RR^{n\times d},}
\end{equation}
%
in which the $v_i$ are the rows, then \eqref{eq:balanced} reads $AM=\theta M$.
So, $\theta$ is an eigenvalue of the adjacency matrix $A$, and the columns of $M$ are (some) \mbox{corresponding~eigen}\-vectors.
In the extreme case, when the columns of $M$ are a complete set of  $\theta$-eigen\-vectors, \ie\ they span the $\theta$-eigenspace $\Eig_G(\theta)$, we speak of a \emph{spectral realization}.



%The details will be discussed in \cref{res:arrangement_space_spectral}, but we can already state here that $\theta$ is an eigenvalue of $G$.
%
%This eigenvalue $\theta\in\Spec(G)$ has a certain multiplicity (which is the dimension of the $\theta$-eigenspace $\Eig_G(\theta)$ of $G$), which finally brings us to the definition of spectral realizations:
%
\begin{definition}
\label{def:spectral}
A $\theta$-balanced realization $v\:V\to\RR^d$ is called \emph{$\theta$-spectral} (or just \emph{spectral}) if the multiplicity of $\theta\in\Spec(G)$ is $d$.
%A realization $v\:V\to\RR^d$ is \emph{$\theta$-spectral} (or just \emph{spectral}) if it is~$\theta$-balanced, and $\theta$ (as an eigenvalue of $G$) has mutliplicity $d$.
\end{definition}

The previous discussion already gives a description on how to construct $\theta$-spectral realizations: find a basis of the $\theta$-eigenspace, put them as columns of $M$, and read of the $v_i$ in the rows.
The reader can also find attached a short Mathematica script for computing spectral realization in \cref{sec:appendix_mathematica}.
%The simplicity of this construction, in combination with the fact that spectral realizations are always $\Aut(G)$-realizations, is where the power...

We also mentioned before that spectral realizations are as symmetric as possible, which we can now state as \enquote{spectral realizations are $\Aut(G)$-realizations} (which is well known, but we include a proof in \cref{res:spectral_then_symmetric}).

\iffalse

%\begin{definition}
%\quad
%\begin{myenumerate}
%\item
%A realization $v$ is said to be \emph{balanced} if there is a real number~$\theta\in\RR$ (which is easily seen to be an eigenvalue of $G$, see \cref{res:arrangement_space_spectral}) so that
%%
%\begin{equation}\label{eq:balanced}
%\sum_{\mathclap{j\in N(i)}} v_j= \theta v_i,\quad\text{for all $i\in V$},
%\end{equation}
%%
%where $N(i):=\{j\in V\mid ij\in E\}$ denotes the \emph{neighborhood} of $i\in V$.
%%We, however, shall deal with this equation from the perspective of spectral graph theory.
%\item
%If the dimension of $v$ matches the multiplicity of the eigenvalue $\theta\in\Spec(G)$, then $v$ is called a \emph{spectral realization} or \emph{$\theta$-realization} of $G$.
%\end{myenumerate}
%\end{definition}
%
%It is possible to interpret equation \eqref{eq:balanced} as expressing a self-stress condition for a graph framework, which again creates a bridge to rigidity theory.

The usefulness of spectral realizations comes from the following two commonly utilized facts: first, spectral realizations are easy to construct, and second, spectral realizations are as symmetric as possible, \ie\ they are $\Aut(G)$-realizations.

While imposing no symmetry requirements, a commonly utilized connection between spectral and symmetric realizations is that every spectral realization is also an $\Aut(G)$-realization, that is, it realizes all the combinatorial symmetries of $G$ (see \cref{res:spectral_then_symmetric}).
%
%More formally, in a spectral realizations the columns of the matrix
%%
%$$M :=
%\begin{pmatrix}
%	\;\horzbar\!\!\!\! & v_1\T & \!\!\!\!\horzbar\;\; \\
%	& \vdots & \\[0.4ex]
%	\;\horzbar\!\!\!\! & v_n\T & \!\!\!\!\horzbar\;\;
%\end{pmatrix}\mathrlap{\in\RR^{n\times d},}$$
%%
%span an eigenspace of $G$.
%If the columns do not span the eigenspace but are still eigenvectors, then $v$ is called \emph{balances}.
%It is classically known that any spectral realization is in fact an $\Aut(G)$-realization as defined above (that is, it realizes all the symmetries of $G$, see \cref{res: ...}).
%
%In general, spectral realizations are often used as an easier accessible substitute for symmetric realizations.
%
This implication is well-understood and used in \eg\ graph drawing algorithms \cite{koren2005drawing}.
This paper focuses on questions pointing in the opposite direction,
that is, we ask for how much symmetry is required (\ie\ how large does $\Sigma\subseteq\Aut(G)$ has to be), so that a symmetric realization is necessarily spectral (or balanced, rigid, etc.).
However, the larger goal is to explore the general connections between symmetric, balanced, spectral, irreducible, and rigid realizations (a detailed map of these connections can be found in \cref{sec:future} in \cref{fig:conncetions}).
%
\fi

%We list some exemplary connections between balanced, spectral, symmetric and rigid realizations that will be discussed in this paper:
%%
%\begin{myenumerate}
%	\item many symmetric realizations are not spectral or even balanced, but every irreducible realization can be deformed (without loosing symmetry) into a balanced realization. Every rigid realizations must therefore already be balanced.
%	\item if a realization is arc-transitive and of full local dimension (defined in \cref{def:full_local_dimension}) then it is rigid, irreducible and balanced.
%	\item if a realization is distance-transitive, then (without further assumptions) it is rigid and an $\Aut(G)$-realization (\ie\ distance-transitivity cannot be realized in isolation). If it is additionally irreducible, then it is even spectral (not only balanced).
%\end{myenumerate}

%
%We list some of the findings:
%
%\begin{myenumerate}
%	\item We prove that every irreducible realization can be made balanced without sacrificing any symmetry. Formally, every irreducible realization is flexible and can be continuously deformed into a balanced realization (conversely, every rigid realization must be already balanced, see \cref{res:...}).
%	\item If an \emph{arc-transitive} realization is of full local dimension (that is, the edge direction at every vertex span the whole space), then it balanced, rigid and irreducible.
%	\item Every \emph{distance-transitive} realization is rigid and realizes all the symmetries of the graph. %, that is, distance-transitive symmetry cannot be geometrically separated from the other symmetries of the graph (in contrast to vertex- and edge-transitivity, which can be realized in isolation as seen in the example of the 4-cycle).
%	Also, for distance-transitive realizations being irreducible,~balanced and spectral are all equivalent.
%\end{myenumerate}

%Among other things, we show that rigid realizations are always balanced, arc-transitive realizations are mostly balanced, and distance-transitive realizations are mostly spectral, in the sense that no counter-examples are known, and certain weak assumption (\eg\ \emph{full local dimension} or $\diam(G)=2$) suffice to actually prove these connections.
%Some consequences are that distance-transitive realizations always realize all the symmetries of the graph, or in other words, that distance-transitivity is a symmetry that cannot be realized geometrically without realizing all the other symmetries of the graph.

%We will find that certain classes of symmetries (namely, distance-transitivity) cannot be realized without also realizing all the other symmetries of the graph.
%In contrast, vertex-, edge- and arc-transitivity can be geometrically separated from the full symmetry group of $G$.
%
%A main tool for our work will be \emph{arrangement spaces} (see \cref{def:...}).
%The connections of which with symmetric point arrangements were discussed in \cite{winter2019geometry}.
%All the relevant properties of a realization can be formulated in terms of arrangement spaces, and in general, they provide a convenient second point of view onto any topic concerning point arrangement up to certain transformations.

%A further goal of this paper is to demonstrate that the concept of the \emph{arrangement space} (see \cref{sec:realizations}) is the appropriate tool for discussing these different concepts (symmetry, spectral properties, rigidity etc.) under a \mbox{common} terminology.~Most~of our results have a second interpretation in terms of arrangement spaces, and many proofs make use of this language.
%
%The concept of the arrangement space in connection with symmetric point arrangements was extensively discussed in \cite{winter2019geometry}, and we will cite several results without proof.

%We included many examples to demonstrate the connections between symmetry and spectral properties.
%In particular, we will draw many parallels to the theory~of \mbox{symmetric} polytopes.


\subsection{Outline of the paper}

In \cref{sec:realizations} we are setting the stage for our investigations.
We define the notion of the \emph{arrangement space} of a realization and discuss how it can be used to study graph realizations up to orthogonal transformations (see \cref{res:equivalence}), and how it characterizes symmetric, balanced and spectral realizations (see \cref{res:arrangement_space_symmetric} and \cref{res:arrangement_space_spectral}).
We prove briefly that spectral realizations are always as symmetric as the underlying graph (see \cref{res:spectral_then_symmetric}).
We introduce the notions of \emph{deformations} and \emph{rigidity} for realizations, and explain how these relate to spectral and representation theoretic properties of $G$ and $\Aut(G)$.
For example, we prove that every irreducible realization can be continuously deformed into a balanced realization (see \cref{res:deform_into_balanced}).
This section contains numerous references to a previous paper \cite{winter2019geometry} in which related notions where discussed for point arrangements (instead of graph realizations). Several proofs are cited from this source.

The rest of the papers now investigates the changes to the previous results if we impose stronger and stronger symmetry restrictions on out realizations.

In \cref{sec:vertex_transitive} we explore the consequences of vertex-transitivity, or the lack thereof. 
We argue that questions about rigidity are almost always only meaningful if we assume vertex-transitivity (\cref{res:vertex_transitive_rigid} and \cref{res:vertex_transitive_rigid_cor}).

In \cref{sec:arc_transitive} we investigate edge- and arc-transitive realizations.
\mbox{In the latter~case,} many metric properties of the realization can already be determined from $G$ and its eigenvalues (see \cref{res:cosine_and_length}).
General (irreducible) arc-transitive realizations are still not too well-behaved,~\eg\ they are not necessarily rigid or spectral (and we do not know whether they are necessarily balanced).
We can show that under mild assumption (namely, \emph{full local dimension}, see \cref{def:full_local_dimension}) an arc-transitive realization is rigid, irreducible and balanced (see \cref{res:full_local_dimension_is_good}).

The final section, \cref{sec:distance_transitive}, is devoted to realizations with exceptionally strong symmetry, namely, \emph{distance-transitivity}.
We explain how the distance-transitive realizations of a graph are completely accessible via spectral realizations (see \cref{res:irreducibe_distance_transitive_is_spectral}).
\cref{res:distance_transitive_consequences} shows that all distance-transitive realizations are rigid and realize all the symmetries of the underlying graph (or in other words, distance-transitivity cannot be realized in isolation).
We explore a generalization of this result beyond distance-transitivity with the help of \emph{cosine vectors} (see \cref{res:cosine_vectors}).





\iffalse

\newpage

%\begin{itemize}
%	\item Arc-transitive realizations have eigenvalues.
%	\item Distance-transitive realizations are spectral and realize all symmetries.
%	\item Self-reproducing polytopes have nice properties:
%	\begin{itemize}
%		\item realize all symmetries of their edge-graph.
%	\end{itemize}
%	\item Motivate that being self-reproducing is something nice.
%	\item Argue that probably all arc-transitive polytope are self-reproducing. Consequences:
%	\begin{itemize}
%		\item Uniquely determined by edge-graph.
%		\item Realizes all symmetries of edge-graph.
%		\item Perfect.
%		\item Metric properties follows from eigenvalues.
%	\end{itemize}
%	\item Show that all Distance-transitive polytopes are self-reproducing and all the nice properties apply.
%\end{itemize}
%
%\cite{blueSpectral}
%
%\vspace{1em}
%
\noindent\textbf{Table of contents}
\begin{enumerate}[label=\arabic*.]
	\item Motivations
	\item Symmetric and rigid realizations
	\begin{enumerate}[label=\theenumi\arabic*]
		\item Graph realizations
		\item Symmetric realizations
		\item Rigid realizations
	\end{enumerate}
	\item Spectral realizations
	\item Vertex-, edge- and arc-transitive realizations
	\item Distance-transitive realizations
	\item Eigenpolytopes
	\item Edge-transitive polytopes
	\item Distance-transitive polytopes
\end{enumerate}



\tempnewpage

\section{Introduction}
\label{sec:introduction}

For a (simple) graph $G=(V,E)$, a realization $v\:V \to\RR^d$ is an embedding of this graph into some Euclidean space.
Its vertices are embedded as points in $\RR^d$
, and its edges as straight lines between these points.

Two classes of realizations of major interest are the \emph{symmetric} realizations and the \emph{spectral} realizations.

A realization can be \emph{symmetric} in the sense that it realizes all (or at least some relevant) combinatorial symmetries of $G$.
A realization can be \emph{spectral} in the sense that it is constructed using spectral properties of $G$ (\ie\ eigenvalues and eigenvetcors of its adjacency matrix).

Spectral realizations have many useful properties, for example, they realize all symmetries of $G$, or have metric properties linked to the eigenvalues and eigenvectors of $G$.
These implications are well-researched, in particular in the context of highly regular graphs as \eg\ distance-regular or walk-regular graphs.

In this paper we want to ask questions in the opposite direction: given a sufficiently symmetric realization of $G$, under which conditions this realization is spectral or has other properties related to the spectrum of $G$.

This direction is interesting, for example, for the investigation of highly symmetric polytopes and their edge-graphs.
In this case on starts with a symmetric realization of the edge-graph (the skeleton of the polytope) and preferably find that these realizations emerge from spectral properties of $G$.


We want to investigate the connection of this direction with realization properties like being \emph{irreducible}, \emph{rigid} or of \emph{full local dimension}.

\hrulefill





Previously investigated were spectral properties of graphs with a lot of symmetry (vertex-transitive, arc-transitive, distance-transitive, etc.) or a lot of regularity (walk-regular, distance-regular, etc.).
This involves so-called \emph{spectral realizations} of a graph, that is, an embedding of the graph into some Euclidean space derived from its eigenvalues and eigenvectors.
Depending on the graph, these realizations are usually themselves of high symmetry.

We investigate the opposite direction: given a highly symmetric realization, is this necessarily a spectral realization?

There has been a lot of research gone into the investigation of spectral properties of highly regular graphs, including distance-regular, or more generally, $k$-walk-regular graphs.
These include as special cases certain highly symmetric graphs, as for example, the arc-transitive, or distance-transitive graphs.
It is an immediate consequence of the theory, that the spectral properties of graphs can be used to obtain spacial realizations of these graphs with a high degree of symmetry (if the graphs has these symmetries in the first place).

In this paper we shall go the opposite way, and ask, in which way sufficiently symmetric geometric realizations of graphs are linked to their spectral properties.

The purpose of this paper is threefold:
%
\begin{itemize}
%	\item To investigate the spectral properties of highly symmetric graphs, and the induced geometric realizations of these graphs.
	\item To investigate geometric realizations of highly symmetric graphs, in particular, those constructed using the spectral properties of the graph.
	\item To survey the notion of \emph{eigenpolytope}, which has not received a thorough literature review in this context.
	\item To explore the use of spectral graph theory for the study of highly symmetric polytopes.
\end{itemize}
%
The term \emph{highly symmetric} in the contex of this paper should always be understood as \enquote{having an exceptionally large symmetry group} or better as \enquote{being transitive on many substructures, as vertices, edges, etc.}.

\fi

==> v.8 - arXiv/sec/realizations.tex <==

\section{Realizations and arrangement spaces}
\label{sec:realizations}

From this section on, let $v\: V\to\RR^d$ denote a realization of \emph{full dimension}, which means that $\rank v$ $:=\dim \Span\{v_1,...,v_n\}=d$.
Equivalently, the arrangement~matrix $M$ (as defined in \eqref{eq:arrangement_matrix}) has rank $d$.

\subsection{Normalized and spherical realizations}

We do care about metric properties of realizations, as lengths and angles, but we do not care about the exact positioning of each vertex in space, that is, we do not care about the orientation of the realization.
We now introduce some terminology that enables us to study realizations up to orthogonal transformations.

%Equivalently, the matrix
%%
%$$M :=
%\begin{pmatrix}
%	\;\horzbar\!\!\!\! & v_1\T & \!\!\!\!\horzbar\;\; \\
%	& \vdots & \\[0.4ex]
%	\;\horzbar\!\!\!\! & v_n\T & \!\!\!\!\horzbar\;\;
%\end{pmatrix}\mathrlap{\in\RR^{n\times d},}$$
%%
%has rank $d$.
%This matrix is called the \emph{arrangement matrix} of $v$.

\begin{definition}\label{def:arrangement_space}
Given a realization $v$ with arrangement matrix $M$,
\begin{myenumerate}
	\item if $M\T M=\alpha\Id$ for some $\alpha>0$, then $v$ is called \emph{spherical}.
	\item if $M\T M=\Id$, then $v$ is called \emph{normalized}.
	\item the column span $U:=\Span M\subseteq\RR^n$ is called \emph{arrangement space} of $v$.
	\item realizations with the same arrangement space are called \emph{equivalent}.
\end{myenumerate}
\end{definition}

%A realization~with $M\T\!M=\alpha\Id$ for some $\alpha>0$ is called \emph{spherical}, and a realization with $M\T \!M=\Id$ is called \emph{normalized}.
%For spherical realizations we have $\rank M=\rank(M\T \! M)=\rank(\alpha \Id)=d$, and so these realizations are always of full dimension.

Spherical (and normalized) realizations are always of full dimension, since $\rank M$ $=\rank (M\T\! M)=\rank(\alpha\Id)=d$.
%
The reason for the use of the word \enquote{spherical} is illustrated in \cref{fig:spherical}.
%
\begin{figure}[h!]
\centering
\includegraphics[width=0.43\textwidth]{img/spherical}
\caption{Two realizations of a cycle graph, one of which is \enquote{spherical} (left), and one of which is not (right).}
\label{fig:spherical}
\end{figure}
%

\noindent
Normalized realizations additionally prescribe a certain scale.

Two (full-dimensional) realizations of the same graph are equivalent (\ie\ have the same arrangement space) if and only if they are related by an invertible linear transformation. This follows from well-known facts in linear algebra: two matrices $M,\bar M\in\RR^{n\x d}$ have the same column span if and only if $M=\bar MT$ for some $T\in\GL(\RR^d)$.
Thus, working with only the arrangement space of a realization already provides a tool for considering realizations up to invertible linear transformations.

But we actually want \enquote{up to orthogonal transformations}.
We can achieve this~via normalized realizations:

%This distinction can be hidden by considering realizations via their so-called \emph{arrangement space} $U:=\Span M$.
%Call two realizations \emph{equivalent} if they have the same arrangement space.
%We use the \mbox{arrangement} space to hide such distinctions:
%The arrangement space can be used to hide such distinctions:
%
%The arrangement space and related notions were used in \cite{winter2019geometry} to study symmetric point arrangements. The most relevant results are collected in this section.
%We then have:
%
\begin{theorem}[\!\cite{winter2019geometry}, Theorem 3.2]
\label{res:equivalence}
Two normalized realizations $v,w\: V\to\RR^d$ of $G$ are equivalent (\ie\ have the same arrangement space) if and only if they are related by an orthogonal transformation $T\in\Ortho(\RR^d)$, that is, $v_i=T w_i$ for all $i\in V$. %(\!\emph{\cite{winter2019geometry}}, Theorem 3.1)
%\begin{myenumerate}
%	\item $v$ and $w$ are equivalent (\ie\ have the same arrangement space) if and only if they are related by an invertible linear transformation, that is, if $Tv=w$ for some $T\in\GL(\RR^d)$. (\!\emph{\cite{winter2019geometry}}, Theorem 2.1)
%	\item if $v$ and $w$ are normalized, then they are equivalent if and only if they are related by an orthogonal transformation $T\in\Ortho(\RR^d)$. (\!\emph{\cite{winter2019geometry}}, Theorem 3.1)
%\end{myenumerate}
\end{theorem}

Motivated by \cref{res:equivalence}, we mostly restrict to study normalized realizations. This comes with no major loss of generality.
Foremost, every realization is equivalent to a normalized realization.
If a realization has arrangement space $U\subseteq\RR^n$, we can define a second realization $\bar v$ whose arrangement matrix $\bar M\in\RR^{n\x d}$ has as columns an orthonormal basis of $U$.
Then $v$ and $\bar v$ are equivalent (both have $U$ as arrangement space), and since $\bar M\T\! \bar M=\Id$, we find that $\bar v$ is normalized.

One might object that some realization that are interesting for their symmetry are not normalized (\eg\ the rhombus realization in \cref{fig:C4}).
Later on, \cref{res:irreducible_spherical} gives a reason not to worry about this.

%Another reason not to worry about this restriction is given in \cref{res:irreducible_spherical}.

%, we are going to study normalized realizations up to orthogonal transformations by considering them via their arrangement space.
%Restricting to normalized realizations is not a big deal as we explain in a second.
%
%Furthermore, given a realization $v$, let $\bar M$ be a matrix whose columns are an orthonormal basis of the arrangement space of $v$.
%This defines a realization $\bar v$ with the same arrangement space, but also $\bar M\T\! \bar M=\Id$, and so $\bar v$ is normalized.
%
%Our approach is to restrict to normalized arrangements.
%The previous comment shows that this is no loss of generality in terms of linear relations.
%A further reason is given in \cref{res:irreducible_spherical}.
%Normalized realizations have the following desirable property:

%Mostly, we do not care about the exact orientation of a realization is space, but we care about general metric properties as angles and lengths.
%Thus, our goal is to study realizations up to orthogonal transformations.
%By \cref{res:equivalence} $(ii)$ we can achieve this by restricting to normalized realizations and by consider those only via their arrangement spaces.



\begin{remark}
As a consequence of \cref{res:equivalence}, metric properties of normalized realizations are uniquely determined by the arrangement space: consider \eg\ the \emph{radius} $r(v)$ defined as follows:
%
\begin{equation}\label{eq:radius}
[r(v)]^2 := \frac 1n\sum_{\mathclap{i\in V}} \|v_i\|^2 = \frac1n \tr\underbrace{(M\T\! M)}_{=\Id} =\frac{\dim U} n = \frac dn.
\end{equation}
%
If all vertices of the normalized realization are on a common sphere around the origin (\eg\ as they are for every vertex-transitive realization, see \cref{res:vertex_transitive} in \cref{sec:vertex_transitive}), then the radius of this sphere is given by $r(v)=d/n$.
\end{remark}


\subsection{Symmetric realizations}

In the context of symmetric realizations there is another reason not to worry about a restriction to normalized (or spherical) realizations:
%
%Restricting to normalized (and spherical) realizations is also no big deal in the con\-text of symmetric realizations:
%
\begin{theorem}[\!\!\cite{winter2019geometry}, Proposition 4.7]
\label{res:irreducible_spherical}
An irreducible $\Sigma$-realization is spherical.
\end{theorem}
%
%Note that the representation $T\:\Sigma\to\Ortho(\RR^d)$ of a (full-dimensional) $\Sigma$-realization is uniquely determined, and so we can assume that being irreducible is well-defined.

\begin{remark}
\label{rem:irreducible_decomposition}
The irreducible $\Sigma$-realizations are the building blocks of general~$\Sigma$-realizations: for a $\Sigma$-realization $v$ with representation $T$, the ambient space decomposes as $\RR^d=W_1\oplus\cdots\oplus W_m$ into a direct sum of pairwise orthogonal $T$-irreducible subspaces $W_k\subseteq\RR^d$. 
The $k$-th irreducible component $v^{(k)}\:V\to\RR^{d_k}$ of $v$ ($d_k$ being the dimension of $W_k$) then is (equivalent to) the orthogonal projection of $v$ onto the subspace $W_k$.

If we assume that $v$ was conveniently oriented, so that the $W_k$ are contained in the coordinate planes, then we can write $v$ as a concatenation %of vectors:
%
\begin{equation}\label{eq:irreducible_decomposition}
v_i=\big(v_i^{(1)},...,v_i^{(m)}\big)\in\RR^{d_1+\cdots+ d_m}.
%v_i = \begin{pmatrix}
%\alpha_1 v_i^{(1)}\\
%\vdots\\
%\alpha_K v_i^{(K)}
%\end{pmatrix}
%\in\RR^{d_1+\cdots+ d_m}
\end{equation}
%
%in the sense that every $\Sigma$-realization $v$ (after an appropriate reorientation) can be written as a concatenation
%%
%\begin{equation}\label{eq:irreducible_decomposition}
%v_i=\big(\alpha_1 v_i^{(1)},...,\alpha_K v_i^{(K)}\big)\in\RR^{d_1+\cdots+ d_K}
%%v_i = \begin{pmatrix}
%%\alpha_1 v_i^{(1)}\\
%%\vdots\\
%%\alpha_K v_i^{(K)}
%%\end{pmatrix}
%%\in\RR^{d_1+\cdots+ d_K}
%\end{equation}
%%
%with normalized irreducible $\Sigma$-realizations $v^{(k)}\:V\to\RR^{d_k}$ and coefficients \mbox{$\alpha_k\in\RR$~for} all $k\in\{1,...,K\}$.
%%($v_i$ in \eqref{eq:irreducible_decomposition} should be understood as the concatenation of the vectors $v_i^{\smash{(k)}}$). 
%
If the $\Sigma$-representation of $v^{\smash{(k)}}$ is $T^{\smash{(k)}}\:\Sigma\to\Ortho(\RR^{d_k})$, then the representation $T$ of $v$ can be written in block form
%
\begin{equation}
\label{eq:representation_decomposition}
T_\sigma = \begin{pmatrix}
T_\sigma^{(1)} & & \\
 & \ddots & \\
 & & T_\sigma^{(m)}
\end{pmatrix}\in\Ortho(\RR^{d}),\quad\text{for all $\sigma\in\Sigma$}.
\end{equation}

Further discussion on reducible and irreducible realization (in the form of point arrangements) can be found in \cite{winter2019geometry} (for example, see Lemma 4.6 in \cite{winter2019geometry} for a discussion of several statements equivalent to being reducible).
\end{remark}


%Hence, dealing directly with the arrangement spaces of normalized realizations is one  way to study realizations up to orthogonal transformations.
%
%In particular, considering only normalized realizations, and those only via their arrangement spaces, allows us to study realization exactly up to orthogonal transformation.
%
%\begin{theorem}
%An irreducible $\Sigma$-realization is spherical.
%\end{theorem}
%We shall therefore assume, that if not mentioned otherwise, our realizations are always normalized.


%\hrulefill

%In the context of symmetric realizations, the restriction to normalized realizations is not a real limitation:
%Restricting to normalized realizations is not a strong limitation in the context of symmetric realization:
%%
%\begin{theorem}[\!\!\cite{winter2019geometry}, Proposition 4.7]
%An irreducible $\Sigma$-realization is spherical.
%\end{theorem}
%%
%Note that the representation $T\:\Sigma\to\Ortho(\RR^d)$ of a (full-dimensional) $\Sigma$-realization is uniquely determined, and so we can assume that being irreducible is well-defined.

%Every $\Sigma$-realization can be written as the product of irreducible $\Sigma$-realizations
%%
%$$v=\alpha_1 v^{(1)}\times \cdots \times \alpha_K v^{(K)},$$
%%
%where $(v\times w)_i := (v_i,w_i)\in\RR^{d_1\x d_2}$.

%This is convenient since we are interested in realizations up to orthogonal transformation, that is, we are interested in metric properties, but not in the exact orientation.
%Considering the arrangement space thus might be useful in hiding irrelevant distinctions.

Now, the second big use of the arrangement space is that it provides an \mbox{alternative} point of view on many properties of realizations.
For example, symmetric realizations are characterized as follows: 

%More generally, the notion of the arrangement space allows a useful second point of view on many properties of realizations.
%For example, symmetric realizations can be characterized as follows: %(see \cref{sec:appendix_rep_theory} for the basic terminology concerning representation theory):
%
%In the context of symmetric realizations, this connection was extensively discussed in \cite{winter2019geometry} (in fact, no underlying graph structure is needed there). In essence, we have the following:

\begin{theorem}%[\!\!\cite{winter2019geometry}, Theorem 4.8, 4.9 and 4.11]
\label{res:arrangement_space_symmetric}
Given a (full-dimensional) realization $v\: V\to\RR^d$ with arrangement space $U\subseteq\RR^n$, then
\quad
\begin{myenumerate}
	\item if $v$ is a $\Sigma$-realization, then $U$ is a $\Sigma$-invariant subspace of $\RR^n$ (\!\emph{\cite{winter2019geometry}}, Theorem 4.8). If $v$ is spherical, then the converse holds (\!\emph{\cite{winter2019geometry}}, Theorem 4.9).
	\item if $v$ is a $\Sigma$-realization, then it is irreducible if and only if $U$ is $\Sigma$-irreducible as invariant subspace of $\RR^n$. \!(\!\emph{\cite{winter2019geometry}}, Theorem 4.11)
%	\item if $v$ is irreducible, then it is spherical.
\end{myenumerate}
\end{theorem}

The condition of being spherical in the converse of \cref{res:arrangement_space_symmetric} $(i)$ is necessary:~a rectangle, a rhombus and a square all have the same arrangement space (they are all linear transformations of each other).
This arrangement space is $\Aut(G)$-invariant for $G=C_4$ (the cycle graph on four vertices), but only the square is an $\Aut(G)$-realization of $G$.
It is also the only realization of these which is spherical.
%Later, we discuss~situations in which being spherical can be replaced by other conditions, \eg\ being distance-transitive (see \cref{res: ...}). \TODO

%\begin{remark}
%The arrangement spaces of two non-equivalent irreducible $\Sigma$-realiza\-tions have trivial intersection (\ie\ intersect only in $\{0\}$). This is because irreducible subspaces are either identical or have trivial intersection.
%\end{remark}

\iffalse

\begin{remark}
A decomposition as in equation \eqref{eq:irreducible_decomposition} can now be obtained as follows: if $U\subseteq\RR^n$ is the arrangement space of the $\Sigma$-realization $v$, then $U$ is $\Sigma$-invariant~and decomposes like
%
\begin{equation}
\label{eq:arrangement_space_decomposition}
U=U_1 \oplus \cdots \oplus U_K
\end{equation}
%
into mutually orthogonal $\Sigma$-irreducible subspaces $U_k\subseteq U$.
These are the arrangement spaces of the $\Sigma$-realizations $v^{\smash{(k)}}$ in \eqref{eq:irreducible_decomposition}.

The decomposition \eqref{eq:arrangement_space_decomposition} might not be unique, and so this might give several \enquote{non-equivalent} decompositions \eqref{eq:irreducible_decomposition}. We revisit this when dsicussing deformations and rigidity (see \cref{def:rigid}).
%
%With \cref{res:arrangement_space_symmetric}, the decomposition \eqref{eq:irreducible_decomposition} can also be understood as the sum
%%
%$$U=U_1+ \cdots + U_K$$
%%
%where $U\subseteq\RR^n$ is the arrangement space of $v$, and the $U_k\subseteq U$ are its $\Sigma$-irreducible subspaces and simultaneously the arrangement spaces of the constituents $v^{(k)}$ in \eqref{eq:irreducible_decomposition}.
\end{remark}

\fi

\subsection{Balanced and spectral realizations}

Likewise, balanced and spectral realizations are characterized using the arrange\-ment space as follows:
%
\begin{theorem}\label{res:arrangement_space_spectral}
Given a (full-dimensional) realization $v\: V\to\RR^d$ with arrangement space \mbox{$U\subseteq\RR^n$,~then}
\quad
\begin{myenumerate}
	\item $v$ is $\theta$-balanced if and only if $U\subseteq\Eig_G(\theta)$ (where $\Eig_G(\theta)$ denotes the~$\theta$-eigenspace of $G$).% (the $\theta$-eigenspace of $G$).
	\item $v$ is $\theta$-spectral (that is, $v$ is a $\theta$-realization) if and only~if~$U=$ $\Eig_G(\theta)$.
\end{myenumerate}
%
\begin{proof}
The defining equality \eqref{eq:balanced} for being balanced can be written as $AM=\theta M$ ($A$ being the the adjacency matrix of $G$, and $M$ the arrangement matrix of~$v$).~In this form it is clear that $\theta$ is an eigenvalue of $A$, and that the columns of $M$ are corresponding eigenvectors.
Since the arrangement space $U$ is the column span of $M$,~equation~\eqref{eq:balanced} is equivalent to $U\subseteq\Eig_G(\theta)$. This proves $(i)$.

The dimension of $v$ (assuming full dimension) equals the rank of $M$, which equals the dimension of $U$.
Thus, if the dimension of a balanced realization $v$ agrees with the dimension of the eigenspace, we must have $U=\Eig_G(\theta)$. This proves $(ii)$.
\end{proof}
\end{theorem}

\Cref{res:arrangement_space_spectral} justifies that we speak of \emph{the} $\theta$-realization of $G$, as any two such~rea\-lizations have the same arrangement space, hence (if normalized) differ only by an orthogonal transformation (by \cref{res:equivalence}).

In general, if not mentioned other wise, speaking of \emph{the} $\theta$-realization, we mean the uniquely determined (up to orientation) normalized realization with $U=\Eig_G(\theta)$.
Also, balanced and spectral realizations will be assumed to be at least spherical.

\begin{observation}\label{res:eigenvectors_from_realization}
If, somehow, we got our hands on a $\theta$-balanced realization $v$, it is straight forward to extract $\theta$-eigenvectors of $G$ from that: the elements of the arrangement space $U\subseteq\RR^n$ are exactly the~vectors \mbox{$u\in\RR^n$} with components
%
\begin{equation}\label{eq:eigenvector}
u_i=\<x,v_i\>,\quad\text{for all $i\in V$},
\end{equation}
%
for some $x\in\RR^d$. This is because equation \eqref{eq:eigenvector} is equivalent to $u=Mx$ (where~$M$ is the arrangement matrix of $v$).
Therefore $u\in\Span M=U$, and since $v$ is balanced we have $U\subseteq \Eig_G(\theta)$, which shows that $u$ is a $\theta$-eigenvector.
\end{observation}

In the language of arrangement spaces it follows immediately that spectral~reali\-zations have all the symmetries of $G$, that is, are $\Aut(G)$-realizations.
This follows from the well-known fact that eigenspaces of $G$ are $\Aut(G)$-inva\-riant: %(for details, see the proof of the next corollary).

\begin{corollary}\label{res:spectral_then_symmetric}
A (spherical) spectral realization $v$ is an $\Aut(G)$-realization.
%
\begin{proof}
Let $v$ be a (spherical) spectral realization of $G$.

By \cref{res:arrangement_space_spectral} $(ii)$, the arrangement space $U\subseteq\RR^n$ of $v$ is an eigenspace, and by this, $\Aut(G)$-invariant (this is well-known, but we included an argument below).
By \cref{res:arrangement_space_symmetric} $(i)$ (and since $v$ is spherical) $v$ is thus an $\Aut(G)$-realization.
%We prove that the eigenspaces of $G$ are $\Aut(G)$-invariant.
%The rest follows via \cref{res:arrangement_space_spectral} $(ii)$ and \cref{res:arrangement_space_symmetric} $(i)$.

To see that $U$ is $\Aut(G)$-invariant, recall that the combinatorial symmetries of $G$ are characterized by $A\Pi_\sigma=\Pi_\sigma A$ for all $\sigma\in\Sym(V)$ (where $\Pi_\sigma\in\Perm(n)$~denotes the permutation matrix associated with the permutation $\sigma$).
For every $u\in U=\Eig_G(\theta)$ and $\sigma\in\Aut(G)$ then holds
%
$$A(\Pi_\sigma u)=(A\Pi_\sigma) u = (\Pi_\sigma A) u = \Pi_\sigma (Au)= \Pi_\sigma (\theta u) = \theta(\Pi_\sigma u),$$
%
thus $\Pi_\sigma u\in\Eig_G(\theta)=U$ and $U$ is $\Aut(G)$-invariant.
\end{proof}
\end{corollary}

%Using the formulations in terms of the arrangement space, 
%%With these alternative formulations in place, it is easy to 
%we can give a quick proof that every spectral realization is maximally symmetric, \ie\ is an $\Aut(G)$-realization.
%We just need to use that eigenspaces of $G$ are $\Aut(G)$-invariant.
%This can be seen as follows: recall that the combinatorial symmetries of $G$ are characterized by $A\Pi_\sigma=\Pi_\sigma A$ (where $\Pi_\sigma\in\Perm(n)$ is the permutation matrix associated to the permutation $\sigma$) for all $\sigma\in\Sym(V)$.
%We then have that for every $u\in\Eig_G(\theta)$ and $\sigma\in\Aut(G)$
%%
%$$A(\Pi_\sigma u)=(A\Pi_\sigma) u = (\Pi_\sigma A) u = \Pi_\sigma (Au)= \Pi_\sigma (\theta u) = \theta(\Pi_\sigma u),$$
%%
%thus $\Pi_\sigma u\in\Eig_G(\theta)$.
%Thus, the eigenspace $\Eig_G(\theta)$ is indeed $\Aut(G)$-invariant, and this gives a quick proof of the following:
%%
%\begin{corollary}\label{res:spectral_then_symmetric}
%Spectral realizations are $\Aut(G)$-invariant.
%\end{corollary}

This can be applied in practice: there exist fast an robust algorithms for computing eigenvalues and eigenvectors, and so spectral methods are often the tool~of~choice for obtaining symmetric realizations of a graph (for example, in graph drawings algorithms, discussed \eg\ in \cite{koren2005drawing}). 
Explicitly, the steps are as follows: one computes an \emph{orthonormal basis} $\{u_1,...,u_d\}\subseteq\RR^n$ of the $\theta$-eigenspace of $G$ and defines the matrix $M:=(u_1,...,u_d)\in\RR^{d\x n}$ in which the $u_i$ are the columns.
This is the arrangement matrix of the $\theta$-realization of $G$, and as such, an $\Aut(G)$-realization (by \mbox{\cref{res:spectral_then_symmetric}})\footnote{See \cref{sec:appendix_mathematica} for an implementation in Mathematica.
}.
This technique alone cannot control the dimension of the realization (it is always the multiplicity of $\theta$), and so some adjustments might be necessary depending on the graph and the setting.

\begin{remark}\label{rem:theta_1}
The largest eigenvalue of a graph is always of multiplicity one (see \cref{sec:appendix_spec_theory}).
Therefore, the corresponding $\theta_1$-realization is always of dimension $d=1$, which is not very interesting.
One therefore considers the $\theta_2$-realizations as the first interesting realizations of a graph.
\end{remark}

\begin{example}\label{ex:dodecahedron}
The spectrum of the edge-graph of the \emph{dodecahedron} is 
%
$$\{(-\sqrt5)^3,(-2)^4,0^4,1^5,(\sqrt 5)^3,3^1\},\quad\text{(exponents denote multiplicites)}.$$ 
%
Note in particular the two eigenvalues of multiplicity three, $\sqrt 5$ and $-\sqrt 5$.
The both corresponding 3-dimensional spectral realizations are shown below:

\begin{center}
\includegraphics[width=0.55\textwidth]{img/dodecahedron_realizations_2}
\end{center}
%
We observe that the $\sqrt5$-realization gives exactly the skeleton of the regular dodecahedron. 
Note that this is the realization to the \emph{second largest} eigenvalue $\theta_2=\sqrt 5$ of the graph.
This is not completely unexpected.
There are heuristic arguments (\eg\ via nodal domain) that suggest that if the skeleton of a polytope is a spectral realization, then it is the $\theta_2$-realization.
However, a rigorous proof of this observation is still missing.

%It is indeed expected, though not completely understood, that this~happens for the \emph{second largest} eigenvalue $\theta_2$ (it is clear that this cannot happen for the largest eigenvalue, as discussed in \cref{rem:theta_1}).
%The other 3-dimensional realization resembles the shape of the so-called \emph{great stellated dodecahedron}.

More evidence for the \enquote{specialness} of $\theta_2$ is provided by the observation that the same phenomenon occurs for the edge-graphs of all the regular polytopes.
%
%by results of Licata and Pwoers in \cite{licata1986surprising}, who have shown that the same phenomenon occurs for the edge graphs of all the other regular polytopes (excluding the exceptional 4-dimensional regular polytopes (the 24-cell, 120-cell and 600-cell).
This was shown by Licata and Powers \cite{licata1986surprising} for all regular polytopes excluding the exceptional 4-dimensional regular polytopes (the 24-cell, 120-cell and 600-cell).
We later close this gap with a note in \cref{ex:24_cell}, or via an alternative approach in \cref{ex:24_cell_cuboctahedron}.
In general however it is an open question which polytope skeleta~can be obtained as spectral realizations.% of their edge-graph.
\end{example}

Besides the fact that we cannot directly control the dimension of the realization, there~are other drawbacks in using spectral realizations when our main focus is on symmetric realizations.
Most notably, an eigenspace, while $\Aut(G)$-invariant, might not be $\Aut(G)$-irreducible. 
If this happens, then the actual irreducible $\Aut(G)$-realizations are inaccessible by spectral method alone (this can probably be fixed, which is briefly discussed in \cref{sec:orbitals}, but this involves additional techniques from computational group theory).
In the language of realizations we can say that some irreducible realizations are not spectral, but only balanced.
And it can be worse: an irreducible symmetric realization must not even be balanced.
We provide examples for both situations.

%This happens when a symmetric realization is not balanced -- or, if it is balanced but not spectral.

%As a consequence, some symmetric realizations might not be spectral, but only balanced, and thus cannot be immediately obtained with the spectral technique explained above.
%Even more, there exist symmetric realizations that are not even balanced.
%
%There follow several examples of these failures of the spectral method.


\iffalse % complete graph example

\begin{example}\label{ex:complete_graph}
Consider an arbitrary set of points $\mathcal V:=\{v_1,...,v_n\}\subset\RR^d$ in dimension $d\in\{2,..., n-2\}$, centered at the origin, that is
%
$$\sum_{i=1}^n v_i=0.$$
%
Let $\Sigma\subseteq\Sym(n)$ be the set of permutation that are induced by a Euclidean symmetry $T\in\Aut(\mathcal V)\subseteq\Ortho(\RR^d)$ of the point set.

We can consider this set of points as a realization $v$ of the complete graph $K_n$.
Since $\Aut(K_n)=\Sym(n)$, we have $\Sigma\subseteq\Aut(K_n)$ and $v$ is a $\Sigma$-realization of $K_n$.
Also, $v$ is a balanced with the eigenvalue $-1$. To see this, note that $N(i)=V\setminus\{i\}$, hence 
%
$$\sum_{\mathclap{j\in N(i)}} v_j = \underbrace{\;\sum_{\mathclap{j\in V}} v_j}_{=\,0} -\, v_i = -v_i.$$
%
But the spectrum of $K_n$ is $\{(-1)^{n-1},(n-1)^1\}$, and thus, all spectral realizations of $K_n$ have dimension 1 or $n-1$.
Thus $v$ is not spectral, but can still be arbitrarily symmetric (imagine $\mathcal V$ being the set of vertices of a highly symmetric polytope other than a regular simplex).
%
%Every realization $v$ of the complete graph $K_n$ with
%%
%$$\sum_{i\in V} v_i=0$$
%%
%is balanced with eigenvalue $-1$ (the spectrum of $K_n$ is $\{(-1)^{n-1},(n-1)^1\}$). To see this, note that $N(i)=V\setminus\{i\}$, hence 
%%
%$$\sum_{\mathclap{j\in N(i)}} v_j = \underbrace{\;\sum_{\mathclap{j\in V}} v_j}_{=\,0} -\, v_i = -v_i.$$
%%
%The spectral realizations of $K_n$ have dimension $1$ or $n-1$.
%Of course, $\Aut(K_n)=\Sym(V)$, and so any $\Sigma$-realization $v$ of $K_n$ for some group $\Sigma\subseteq\Sym(V)$ and dimension less than $n-1$ is balanced, but not spectral.
\end{example}

One might think that the realization $v$ in \cref{ex:complete_graph} is not spectral because it has not used all symmetries of $K_n$ (indeed, realizing all symmetries of $K_n$ would yield the skeleton of the regular simplex, which is a spectral realization of $K_n$).

In general however this problem can also occur for $\Aut(G)$-realizations.

\fi

\begin{example}\label{ex:hexagonal_prism}
Let $G$ be the edge-graph of the hexagonal prism with vertex~set $V=\{1,...,6,1',...,6'\}$,
labels assigned to the vertices as shown in \cref{fig:prism} (left). %where the un-dashed vertices belong to one of the hexagonal faces of $G$, and the dashed vertices belong to the other hexagonal face, so that $ii'$ is an edge of $G$ for all $i\in\{1,...,6\}$.
%
\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.65\textwidth]{img/6_prism_zero_realization}
\end{center}
\caption{The edge-graph of the prism, and an irreducible non-spectral 2-dimensional $\Aut(G)$-realization to the eigenvalue 0.}
\label{fig:prism}
\end{figure}
%

The spectrum of $G$ is $\{(-3)^1,(-2)^2,(-1)^1,0^4,1^1,2^2,3^1\}$.
Note in \mbox{particular} the  eigenvalue 0 of multiplicity \emph{four}.
We show that the 0-eigenspace is not~irreducible, by constructing a balanced $\Aut(G)$-realization to this eigenvalue of dimension less than four.

%Consider the following realization of $G$ of dimension two:
Consider the realization in \cref{fig:prism} (right).
The un-dashed vertices are placed in the shape of a hexagon centered at the origin, and each dashed vertex is placed opposite to its un-dashed neighbor, that is, $v_{i'}=-v_i$ (the figure shows only six points because the vertices are mapped on top of each other; the highlighted lines are the images of the edges incident to the vertex $1\in V$).

One checks that this is an $\Aut(G)$-realization of $G$.
One checks further, that this realization is balanced with eigenvalue zero: the three neighbors of each vertex span a regular triangle whose barycenter is the origin.
%But since the dimension of $v$ does not agree with the multiplicity of $0\in\Spec(G)$, it cannot be a spectral realization, and the 0-eigenspace of $G$ cannot be irreducible \wrt\ $\Aut(G)$.
%
%The same phenomenon can be observed with any $6k$-gonal prism.
It cannot be a spectral realization since its dimension is not four.
\end{example}

%


%\begin{example}
%Most obviously, a realization cannot be balanced if it is of a higher dimension than the largest eigenspace of $G$.
%
%For example, let $G$ be the edge-graph of the triangular prism and $v$ be its standard realizations as the skeleton of such a prism in $\RR^3$.
%It is not hard to see that this is an $\Aut(G)$-realization, that is, the prism is not less symmetric than its edge-graph.
%But the spectrum of $G$ is $\{(-2)^2,0^2,1^1,3^1\}$.
%Since there is no eigenspace of dimension at least three, $v$ cannot be balanced.
%
%Every symmetric realization of a larger dimension than the largest eigenspace is also always reducible, that is, can be projected onto a subspace while not loosing symmetry.
%\end{example}

\begin{example}\label{ex:truncated_tetrahedron}
The \emph{truncated tetrahedron} is a polyhedron obtained from the regular tetrahedron by cutting of each vertex.
The image below shows serveral distinct realizations of this polyhedron:
%
\begin{center}
\includegraphics[width=0.6\textwidth]{img/truncated_tetrahedron}
\end{center}

All of these realizations have the full symmetry of the tetrahedron, which implies that they are $\Aut(G)$-realization of the edge-graph $G$.

Now, this degree of freedom gives an uncountable family of mutually non-equivalent $\Aut(G)$-realizations, each of which corresponds to a distinct $\Aut(G)$-invariant subspace of $\RR^n$ (by \cref{res:arrangement_space_symmetric}).
The spectrum of $G$ is $\{(-2)^3,(-1)^3,0^2,2^3,3^1\}$,~and we see that there are exactly three 3-dimensional balanced realizations of $G$ (which must then also be spectral).
%
%
%But only finitely many of these can be eigenspaces of $G$.
Consequently, almost all of the previously discussed uncountably many $\Aut(G)$-reali\-zations are not balanced.
%
%In fact, investigating the spectrum of $G$, which is $\{(-2)^3,(-1)^3,0^2,2^3,3^1\}$, we see that there can be only three 3-dimensional balanced realizations.
%All the other realizations considered above turn out to be linear combinations of these two.

%Let $G$ be the edge-graph of the truncated tetrahedron.
%The spectrum of $G$ is $\{(-2)^3,(-1)^3,0^2,2^3,3^1\}$.
%There are several eigenvalues of multiplicity three that can be used to construct 3-dimensional realizations.
%
%It turns out that two of these eigenvalues, namely $2$ and $-1$, give us realizations that (if oriented appropriately) have the same representation $T:\Aut(G)\to\Ortho(\RR^3)$.
%We shall denote them $v^2$ and $v^{-1}$ respectively.
%Then, for every $t\in[0,1]$, the linear combination
%%
%$$v(t):= (1-t) v^2 + t v^{-1}$$
%%
%is also an $\Aut(G)$-realization with the same representation.
%
%If $v(t)$ would be balanced for all $t\in[0,1]$, there would be a function $\theta(t)$ with
%%
%$$\sum_{\mathclap{j\in N(i)}} v_j(t) = \theta(t) v_i(t), \quad\text{for all $i\in V$}.$$
%%
%It is not hard to see that the function $\theta(t)$ transitions \textit{continuously} from $2$ to $-1$ as $t$ transitions from $0$ to $1$.
%But any $\theta(t)$ has to be an eigenvalue of $G$, and the set of eigenvalues is a discrete set.
%Hence, not all (actually none) of the intermediate realizations can be spectral (or even balanced), but all of them are $\Aut(G)$-realizations.
\end{example}


This last example contains an instance of a continuous transition between non-equivalent realizations.
%Such will be the focus of the rest of this section.

\subsection{Deformations and rigidity}

%We discuss a sub-class of symmetric realizations that helps to circum\-vent some of these problems.
Let $\mathcal R_d(G,\Sigma)$ be the space of all full-dimensional $\Sigma$-realizations of $G$ of dimension $d$. Since realizations can be naturally associated with their arrangement matrices, we can consider $\mathcal R_d(G,\Sigma)$ as a subspace of $\RR^{n\x d}$ equipped with the  subspace topo\-logy.


\begin{definition}\label{def:rigid}
\quad 
\begin{myenumerate}
	\item Given two realizations $v,w\in\mathcal R_d(G,\Sigma)$, we say that these realizations can be \emph{deformed} into each other, if there exists a continuous curve $v(\free)\:[0,1]\to\mathcal R_d(G,\Sigma)$ with $v(0)=v$ and $v(1)=w$.
	The curve $v(t)$ is then called a~\emph{defor\-ma\-tion} between $v$ and $w$.
	%\item A deformation is \emph{proper} if the induced map $t\mapsto U(t)$, that assigns $t$ to the arrangement spaces $U(t)$ of $v(t)$, is non-constant (intuitively, this means that the deformation is not just a continuous reorientation, stretching or squishing, but an actual non-linear change) .
	\item A realization $v\in\mathcal R_d(G,\Sigma)$ is called \emph{rigid} if it cannot be deformed into~a~non-equivalent realization. It~is~called \emph{flexible} otherwise.
\end{myenumerate}
\end{definition}


Deformations and rigidity of realizations (in the form of symmetric point arrange\-ments) were extensively discussed in \cite{winter2019geometry}.
We~recap~the relevant results and try to convey an intuition for how rigidity is connected to arrangement spaces and~represen\-tation theory.

\begin{remark}
Deformations of $\Sigma$-realizations as in \cref{def:rigid} preserve the symmetries in $\Sigma$.
A rigid realization cannot be deformed without loosing these relevant symmetries. 
However, such a rigid realization might well be \enquote{flexible} in the usual sense of rigidity theory of frameworks, where one cares mainly~about preserving edge-lengths. 
Preserving edge-lengths is also \mbox{not necessary~for~a~deforma}\-tion in our sense (unless, the symmetry requirements enforce it, see \cref{rem:edge_transitive_rigidity}).
%
%For example, the \mbox{skeleton~of~the~\mbox{truncated}}~tetra\-hedron in \cref{ex:truncated_tetrahedron} is flexible, but apparently its edge lengths are changing during the deformation.
\end{remark}

\begin{observation}\label{res:t_Ut}
Of course, any continuous reorientation or rescaling is a deformation in the sense of \cref{def:rigid}.
But more interesting are the deformations that acts in a \mbox{non-linear} way, as \eg\ the deformation of the skeleton of the truncated tetrahedron in \cref{ex:truncated_tetrahedron}.

Let us call such a non-linear deformation a \emph{proper deformation}.
We can formulate this in terms of arrangement spaces: a deformation $t\mapsto v(t)$ induces a map $t\mapsto U(t)\subseteq\RR^n$, that assigned to $t$ the arrangement spaces of $v(t)$.
Recalling \cref{res:equivalence}, a \enquote{proper deformation} is a deformation for which the map $t\mapsto U(t)$ is non-constant.
%A realization $v\in\mathcal R_d(G,\Sigma)$ is then rigid, if it can~be~properly~de\-formed.
\end{observation}


\begin{observation}\label{res:deformation_intuition}
In a sense, the map $t\mapsto U(t)$ from \cref{res:t_Ut} describes a continuous curve in the \enquote{space of $d$-dimensional subspaces of $\RR^n$} (formally known as the \emph{Grassmannian} $G(d,n)$).
%
When transitioning continuously from a subspace $U(0)$ to a distinct subspace $U(1)$,
one necessarily passes though infinitely many pairwise distinct $\Sigma$-invariant subspaces $U(t)$.
This gives a necessary condition for the existence of a proper deformation: %there have to be infinitely many $\Sigma$-invariant subspaces.

\begin{corollary}\label{res:finitely_many_subspaces}
%If $v\in\mathcal R_d(G,\Sigma)$ is flexible, then there are infinitely many distinct $\Sigma$-invariant subspaces.

If there are only finitely many $\Sigma$-irreducible subspaces, then all~$\Sigma$-realizations are rigid.
\end{corollary}

Note that the statement of \cref{res:finitely_many_subspaces} is slightly stronger than what we~have argued for in \cref{res:deformation_intuition}: in the corollary we require finitely many \emph{$\Sigma$-irreducible} subspaces rather than \emph{$\Sigma$-invariant} subspaces.
%
\begin{proof}[Proof of \cref{res:finitely_many_subspaces}]
%In contrast to \cref{res:deformation_intuition}, we only require finitely many \emph{$\Sigma$-irreducible} subspaces (rather than $\Sigma$-invariant).
%
Since every $\Sigma$-invariant subspace is the direct sum of $\Sigma$-irreducible subspaces, if there are only finitely many of the latter, then there are only finitely many of the former, and no $\Sigma$-realization can be flexible as discussed im \cref{res:deformation_intuition}.
\end{proof}

%Furthermore, while transitioning from $t=0$ to $t=1$, one would expect that the angle between $U(t)$ and $U$ is changing continuously from $0$ to $\angle(U,U')$.
%Likewise, the angle between $U(t)$ and $U'$ is changing continuously from $\angle(U,U')$ to $0$.
%Intuitively, one would then expect to find that some intermediate subspace $\bar U:=U(t^*)$ is non-orthogonal to both $U$ and $U'$. 
%% (\ie\ there are $\bar u\in\Bar U$, $u\in U$ and $u'\in U'$ so that $\<u,\bar u\>\not=0$ and $\<u',\bar u\> \not=0$).
%In the case of irreducible realizations this observation was made precise on \cite{winter2019geometry} and provides a convenient tool in working with deformations.
%%In the case when all $U(t)$ are $\Sigma$-irreducible, this was made rigorous in \cite{winter2019geometry}, and we have also obtained the converse.
%%We use it in the following form:
\end{observation}

%The following theorem encapsulates the intuitive conditions motivated in \cref{res:deformation_intuition}, as well as further useful properties of deformation equivalent realization:

%We collect the relevant facts, previously proven in \cite{winter2019geometry}, in the following theorem:

%\begin{theorem}\label{res:rigidity_theorem}
%Suppose that the two irreducible realizations $v,w\in\mathcal R_d(G,\Sigma)$~can~be deformed~into each other, then
%%
%\begin{myenumerate}
%	\item there is a $\Sigma$-invariant subspace $\bar U\subseteq \RR^n$ non-orthogonal to the arrangement spaces of both $v$ and $w$ (\eg\ this is the case if the arrangement spaces of $v$ and $w$ are non-orthogonal) (\!\cite{winter2019geometry}, Theorem 5.11).
%	\item $v$ and $w$ have isomorphic representations\footnote{This is the realization version of the representations theoretic fact in \cref{res:non_orthogonal_subspaces}.}, or if we assume an appropriately reorientation, even the same representation.
%	 (\!\cite{winter2019geometry}, Corollary 5.5)
%\end{myenumerate}
%As a converse to $(i)$, if $v$ and $w$ have non-orthogonal arrangement spaces, then they can be~de\-formed into each other (\!\cite{winter2019geometry}, Theorem 5.11).
%\end{theorem}

In \cite{winter2019geometry} we have deduces several other necessary and sufficient conditions for~the~exis\-tence of deformations.
We list some of these:

%The following theorem summarizes the (for this paper) most relevant connections between deformations and rigidity on the one side, and arrangement spaces and representation theory on the other side:


\begin{theorem}\label{res:rigid}
\quad
\begin{myenumerate}
	\item If two irreducible realizations $v,w\in\mathcal R_d(G,\Sigma)$ have non-orthogonal arrangement spaces, then they can be deformed into each other, in particular, both realizations are flexible. (\!\cite{winter2019geometry}, Theorem 5.11)
	\item If an irreducible realization $v\in\mathcal R_d(G,\Sigma)$ is flexible, then $v$ can be deformed into a non-equivalent realization $w\in\mathcal R_d(G,\Sigma)$ with an arrangement space non-orthogonal to the one of $v$. (\!\cite{winter2019geometry}, Theorem 5.11)
	\item If two irreducible realizations $v,w\in\mathcal R_d(G,\Sigma)$ can be deformed into each other, then their representations are isomorphic, or if reoriented appropriately, we can assume that they have the same representation.\footnote{Together with point $(i)$, this is the realization version of the representations theoretic fact in \cref{res:non_orthogonal_subspaces}.}
	(\!\cite{winter2019geometry}, Corollary 5.5)
\end{myenumerate}
\end{theorem}

%Whether a group $\Sigma\subseteq\Aut(G)$ admits flexible realizations is hence completely encoded in the representation theoretic properties of $\Sigma$.

%\begin{corollary}
%For $\Sigma\subseteq\Aut(G)$, the following are equivalent:
%%
%\begin{myenumerate}
%	\item all irreducible $\Sigma$-realization are rigid.
%	\item there is a unique decomposition $\RR^n=U_1\oplus\cdots \oplus U_m$ of $\RR^n$ into $\Sigma$-irreducible subsapces $U_k\subseteq\RR^n$.
%\end{myenumerate}
%%
%\begin{proof}
%Suppose that $\RR^n=U_1\oplus\cdots \oplus U_m$ is a unique decomposition.
%\end{proof}
%\end{corollary}

%\begin{corollary}\label{res:rigid_corollary}
%If all irreducible $\Sigma$-realizations are rigid, then all $\Sigma$-realizations are rigid.
%%
%\begin{proof}
%$\Bbb R^n$ decomposes like
%%
%$$\RR^n=U_1\oplus\cdots \oplus U_m$$
%%
%into pairwise orthogonal $\Sigma$-invariant subspaces $U_k\subseteq\RR^n$.
%In fact, if all irreducible $\Sigma$-realizations are rigid, these must be all the $\Sigma$-irreducible subspaces there are: any further such subspace would be non-orthogonal to some $U_k$, making a realization with realization space $U_k$ flexible by \cref{res:rigid} $(i)$.
%
%So, if there are only finitely many $\Sigma$-irreducible subspaces, then there are only finitely many $\Sigma$-invariant subspacs overall (as any such decomposes into a direct sum  of irreducible ones).
%But the existence of any flexible realization means infinitely many distinct $\Sigma$-irreducible subspaces as noted in \cref{res:deformation_intuition}.
%\end{proof}
%\end{corollary}

\iffalse

\begin{corollary}\label{res:rep_theory_characterization}
For $\Sigma\subseteq\Aut(G)$, the following are equivalent:
%
\begin{myenumerate}
	\item all irreducible $\Sigma$-realization are rigid.
	\item there are only finitely many distinct $\Sigma$-irreducible subspaces $U\subseteq\RR^n$.
\end{myenumerate}
%
\begin{proof}
If there is a deformation $v(t)$ of irreducible realization, then this induces a continuous map $t\mapsto U(t)$, attaining infinitely many distinct irreducible $\Sigma$-invariant subspaces. This shows $(ii)\Longrightarrow (i)$.

For the converse, consider a decomposition $\RR^n=U_1\oplus\cdots \oplus  U_m$ into mutually orthogonal $\Sigma$-irreducible subspaces $U_k\subseteq\RR^n$.
These are finitely many $\Sigma$-irreducible subspaces.
If there are infinitely many $\Sigma$-irreducible subspaces, then there would be another such subspace $U\subseteq\RR^n$, which must then be non-orthogonal to one of the $U_k$.
Two $\Sigma$-realizations with arrangement spaces $U$ and $U_k$ can then be deformed intoe each other, hence are flexible. This shows $(i)\Longrightarrow (ii)$.
\end{proof}
\end{corollary}

\begin{corollary}
If all irreducible $\Sigma$-realizations are rigid, then all $\Sigma$-realizations are rigid.
%
\begin{proof}
If all irreducible $\Sigma$-realizations are rigid, then there are only finitely many $\Sigma$-irreducible subspaces by \cref{res:rep_theory_characterization}.
All $\Sigma$-invariant subspace $U\subseteq\RR^d$ can be obtained as direct sums of $\Sigma$-irreducible subspaces.
thus, there can be only finitely many $\Sigma$-invariant subspaces.
\end{proof}
\end{corollary}

As a useful extension of \cref{res:rigidity_theorem} to reducible realizations, not contained~in \cite{winter2019geometry}, we prove

%This is about irreducible realizations.
%There was not anything proven about reducibler realizations in \cite{winter2019geometry}.
%A version of this result we need is the following:

\begin{theorem}\label{res:reducible_rigid}
If all irreducible $\Sigma$-realizations of $G$ are rigid, then \ul{all} $\Sigma$-realiza\-tions are rigid.
\begin{proof}
Consider a decomposition of $\RR^n=U_1\oplus \cdots \oplus U_m$ into mutually orthogonal $\Sigma$-invariant subspaces $U_i\subseteq\RR^n$.
Each subspace corresponds to an irreducible $\Sigma$-realization $v^{\smash{(i)}}$ with arrangement space $U_i$.
If there were any further irreducible $\Sigma$-invariant subspace $U\subseteq\RR^n$ distinct from all $U_i$, it would need to be non-orthogonal to some $U_i$.
But then a realization $v$ with arrangement space $U$ could be deformed into $v^{\smash{(i)}}$, in contradiction to the assumption that all irreducible $\Sigma$-realizations are rigid.

Hence, there are only finitely many irreducible $\Sigma$-invariant subspaces $U_1,...,U_m\subseteq\RR^d$.
Since every $\Sigma$-invariant subspace is a direct sum of irreducible subspaces, we found that there are only finitely many $\Sigma$-invariant subspaces in general.

But any deformation $t\mapsto v(t)$ between non-equivalent realization runs through uncountably many mutually non-equivalent $\Sigma$-realization, each of which corresponds to a distinct $\Sigma$-invariant subspace of $\RR^d$. This is a contradiction, and such a deformation cannot exist.
\end{proof}
\end{theorem}

\fi


\iffalse

\begin{theorem}[\!\!\cite{winter2019geometry}, Theorem 5.11]
Two irreducible realizations $v,v'\in\mathcal R_d(G,\Sigma)$ can be deformed into each other, if and only if there is an irreducible $\Sigma$-invariant subspace $\bar U\subseteq\RR^d$ non-orthogonal to the arrangement spaces of both $v$ and $v'$.
\end{theorem}

\begin{corollary}
\label{res:rigidity_corollary}
\quad
\begin{myenumerate}
\item
If $v,v'\in\mathcal R_d(G,\Sigma)$ are irreducible and have non-orthogonal arrangement spaces, then they can be deformed into each other.
\item
An irreducible $v\in\mathcal R_d(G,\Sigma)$ is flexible, if and only if there is an irreducible $\Sigma$-invariant subspace $\bar U\subseteq\RR^n$ distinct and non-orthogonal to the arrangement space of $v$.
\end{myenumerate}
\end{corollary}

%In terms of arrangement spaces, a deformation corresponds to a continuous transition $t\mapsto U(t)$ between two $d$-dimensional $\Sigma$-invariant subspaces of $\RR^n$, each intermediate 
%
%Our notion of rigidity can be characterized using arrangement spaces.

%\begin{theorem}\label{res:non_orthogonal_deformation}
%If irreducible realizations $v^0,v^1\in\mathcal R_d(G,\Sigma)$ have non-orthogonal arrangement spaces, then they can be deformed into each other.
%\end{theorem}
%
%\begin{theorem}
%If an irreducible realization $v\in\mathcal R_d(G,\Sigma)$ is flexible, then there is a realization $w\in\mathcal R_d(G,\Sigma)$, so that $v$ and $w$ have non-orthogonal realization spaces.
%\end{theorem}

%\begin{theorem}[\!\!\cite{winter2019geometry}, Theorem 5.11 $(i)\Leftrightarrow (iii)$]
%\label{res:non_orthogonal_deformation}
%\quad\begin{myenumerate}
%\item
%If irreducible realizations $v,w\in\mathcal R_d(G,\Sigma)$ have non-orthogonal arrangement spaces, then they can be deformed into each other.
%\item
%If an irreducible realization $v\in\mathcal R_d(G,\Sigma)$ is flexible, then there is a non-equivalent irreducible realization $w\in\mathcal R_d(G,\Sigma)$, so that $v$ and $w$ have non-orthogonal realization spaces.
%\end{myenumerate}
%\end{theorem}

\begin{theorem}
Given two irreducible realizations $v,v'\in\mathcal R_d(G,\Sigma)$ that can be~de\-formed into each other, then
%
\begin{myenumerate}
\item $v$ and $v'$ have isomorphic representations, or equivalently, if reoriented appropriate, we can assume that both realizations have the exact same representation.
%after an appropriate reorientation, both realizations have the same representa\-tion. 
(\!\emph{\cite{winter2019geometry}}, Corollary 5.5)
%both realizations can be assumed to have the same representation (maybe we have to reorient one of the realizations, but this gives an equivalent one),
\item there is a $\Sigma$-invariant subspace $\bar U\subseteq\Aut(G)$ non-orthogonal to the arrangement spaces of both $v$ and $v'$. This includes the case where the arrangement spaces of $v$ and $v'$ are non-orthogonal.
\end{myenumerate}
%
Conversely, if $v,v'$ have non-orthogonal arrangement spaces (or there is a $\Sigma$-invariant subspace non-orthogonal to both), then they can be deformed into each other.
\end{theorem}

\TODO \msays{Erwähnen dass non-orthogonal subspaces identische Darstellungen implizieren}

The statement $(ii)$ and its converse are a variant of Theorem 5.11 in \cite{winter2019geometry}. 
We include a sketch for a proof aligned on the proof of Theorem 5.11 in \cite{winter2019geometry}.

\begin{proof}[Sketch of proof for $(ii)$]
Let $U,U'\subseteq\RR^n$ denote the arrangement spaces of $v$ and $v'$ respectively.

A deformation $v(t)\:[0,1]\to\mathcal R_d(G,\Sigma)$ with $v(0)=v$ and $v(1)=v'$ also induces a map $t\mapsto U(t)$ (the arrangement space of $v(t)$), hence a \enquote{continuous transition} between the subspaces $U$ and $U'$.
Some \enquote{intermediate subspace} $\bar U:=U(t^*)$ must then be non-orthogonal to both $U$ and $U'$.

Conversely, \cite{winter2019geometry} Theorem 5.11 states that for $v$ being flexible is equivalent to the existence of a $\Sigma$-invariant subspace $\bar U\subseteq\RR^n$ non-orthogonal to $U$. Moreover, $v$ can be deformed into any $\Sigma$-realization with arrangement space $\bar U$.
So a subspace $\bar U\subseteq\RR^n$ as in $(ii)$ corresponds to a $\Sigma$-realization that can be deformed into both, $v$ and $v'$, and this provides a deformation between $v$ and $v'$.
\end{proof}

\fi

%\begin{corollary}
%Two irreducible realizations $v^0,v^1\in\mathcal R_d(G,\Sigma)$ with arrangement spaces $U^0,U^1\subseteq\RR^n$ can be deformed into each other if and only of there is an irreducible $\Sigma$-invariant subspace $U\subseteq\RR^n$ non-orthogonal to both $U^0$ and $U^1$.
%\end{corollary}
%
%In short, first one shows that (after some reorientation) $v^0$ and $v^1$ can be assumed to have the same representation $T\:\Sigma\to\Ortho(\RR^d)$, and second, that as deformation one can choose a linear transition
%%
%$$v(t)=(1-t) v^0 + t v^1.$$
%%
%Irreducibility and non-equivalence are necessary to show that $v(t)$ is~full-dimensional for all $t\in[0,1]$.

A first relevant application for us is the following:


%\begin{theorem}
%An irreducible realization $v\in\mathcal R_d(G,\Sigma)$ that cannot be deformed into a non-balanced realization must be rigid.
%\end{theorem}

\iffalse

\begin{theorem}\label{res:deform_into_balanced}
Every irreducible realization $v\in\mathcal R_d(G,\Sigma)$ can be deformed into a balanced $\Sigma$-realization.
%
\begin{proof}
Consider the eigen-decomposition
%
%\begin{equation}\label{eq:eigendecomposition}
$$\RR^n=\Eig_G(\theta_1)\oplus\cdots \oplus\Eig_G(\theta_m)$$
%\end{equation}
%
of $\RR^n$ into pairwise orthogonal $\Sigma$-invariant subspaces (eigenspaces are $\Aut(G)$-invariant as seen the proof of \cref{res:spectral_then_symmetric}).
The arrangement space $U\subseteq\RR^n$~of $v$ must then be non-orthogonal to some eigenspace, say $\Eig_G(\theta)$. % (\ie\ there is a $u\in U$ and an $x\in\Eig_G(\theta)$ with $\<u,x\>\not=0$).

Since $v$ is irreducible, so is $U$ (by \cref{res:arrangement_space_spectral} $(ii)$).
And since $U$ and $\Eig_G(\theta)$~are non-orthogonal, the orthogonal projection $U':=\pi(U)\subseteq \Eig_G(\theta)$ of $U$ onto this eigenspace is still irreducible (see \cref{res:non_orthogonal_projection}) and non-orthogonal to $U$.
Then, by \cref{res:rigid}, $v$ can be deformed into any $\Sigma$-realization with arrangement space $U'$, which is balanced \cref{res:arrangement_space_spectral}.
\end{proof}
\end{theorem}

\fi


\begin{theorem}\label{res:deform_into_balanced}
Every irreducible realization $v\in\mathcal R_d(G,\Sigma)$ can be deformed into a balanced $\Sigma$-realization.

Moreover, if $v$ is not already balanced, then $v$ can be deformed into at least two balanced $\Sigma$-realizations $w$ and $w'$ to different eigenvalues.
%
\begin{proof}
Consider the eigen-decomposition
%
$$\RR^n=\Eig_G(\theta_1)\oplus\cdots \oplus\Eig_G(\theta_m)$$
%
of $\RR^n$ into pairwise orthogonal $\Sigma$-invariant subspaces (the eigenspaces are $\Aut(G)$-invariant as seen the proof of \cref{res:spectral_then_symmetric}).

If $v$ were balanced, then we were done.
So assume, that $v$ is not balanced.
Its arrangement space $U\subseteq\RR^n$ is therefore not contained in any of the eigenspace of $G$.
Hence, $U$ is non-orthogonal to at least two of the eigenspaces, say $\Eig_G(\theta_1)$ and $\Eig_G(\theta_2)$.
Let $U_i:=\pi_i(U)$ denote the orthogonal projection of $U$ onto $\Eig_G(\theta_i)$.
Since $v$ is irreducible, so is $U$ as a subspace of $\RR^n$ (by \cref{res:arrangement_space_symmetric} $(ii)$), and one can check that $U_i$~is itself $\Sigma$-irreducible and non-orthogonal to $U$ (or see \cref{res:non_orthogonal_projection} in the appendix).
Any $\Sigma$-realization $w^{\smash{(i)}}$ with arrangement space $U_i\subseteq\Eig_G(\theta_i)$ is now irreducible (by \cref{res:arrangement_space_symmetric} $(ii)$), balanced (by \cref{res:arrangement_space_spectral}), and can be deformed into $v$ (by \cref{res:rigid} $(i)$).
\end{proof}
\end{theorem}

%Conversely, if a realization is not balanced, then it cannot be rigid (for any group $\Sigma\subseteq$ $\Aut(G)$, for which it is a $\Sigma$-realization).
%Alternatively, we have

\begin{corollary}\label{res:rigid_implies_balanced}
If $v\in\mathcal R_d(G,\Sigma)$ is rigid and irreducible, then it is balanced.
\end{corollary}





\begin{theorem}\label{res:eigenvalue_multiplicity_implications}
Let $v\:V\to\RR^d$ be an irreducible $\Sigma$-realization of $G$. Suppose~that $G$ has a single eigenvalue $\theta$ of largest multiplicity $\mu_1$, and the second largest multiplicity of any eigenvalue of $G$ is $\mu_2$. Then
%
\begin{myenumerate}
	\item if $\mu_2<d$, then $v$ is balanced with eigenvalue $\theta$.
	\item if additionally $\mu_1 <2d$, then $v$ is rigid.
\end{myenumerate}
%
\begin{proof}
If $v$ is not already balanced, then by \cref{res:deform_into_balanced} it can be deformed into two balanced realizations with different eigenvalues.
Then these realizations~must~be of dimension $d$, and their arrangement spaces must be contained in different eigen\-spaces. But if $\mu_2<d$, then only one of these eigenspaces can have a large enough dimension.
Thus, $v$ must already have been balanced, and its arrangement space $U\subseteq\RR^n$ must be contained in the only large enough eigenspace $\Eig_G(\theta)$.
This proves $(i)$.

If $v$ were flexible, then it can be deformed into another non-equivalent irreducible $\Sigma$-realization $w$, also of dimension $d$.
For the same reasons as before, $w$ would be balanced with eigenvalue $\theta$, and thus its arrangement space $U'\subseteq\RR^n$ would be contained in $\Eig_G(\theta)$.
In particular, we have $U+U'\subseteq\Eig_G(\theta)$.
But since $U$ and $U'$ are irreducible, their intersection is trivial, and we have $$\mu_1=\dim\Eig_G(\theta)\ge \dim(U+U')=\dim(U)+\dim(U)-\dim(U\cap U')=2d.$$
%
Thus, if $\mu_1<2d$, then $v$ must have been rigid, proving $(ii)$.
\end{proof}
\end{theorem}

%\begin{example}
%Every $d$-dimensional realization
%\end{example}

\subsection{Summary}
The take away messages of this section are:

\begin{itemize}
\item
A realization being symmetric, spectral, balanced, irredu\-cible or rigid can be nicely encoded in the language of arrangement spaces, which makes this concept an attractive tool for us.

\item Spectral realizations are as symmetric as possible. %, or in other words, they are $\Aut(G)$-realizations. 
Since they are also fast to compute, they present a useful construction, even for those, mainly~interes\-ted in symmetric realizations.
%Also, many \enquote{famous} realizations are actually spectral realizations. 
%For example, the dodecahedral skeleton from \cref{ex:dodecahedron}, which will be one of our running examples.

\item
But, there are (irreducible) symmetric realizations that are not spectral,~only balanced, or not even that.
So in general, spectral methods are not enough.

\item Still, every irreducible realization can be deformed into a balanced realization (while keeping its symmetries). Conversely, this also means, that if a realization is rigid, then it must be balanced.
\end{itemize}



\tempnewpage

\section{Vertex-transitive realizations}
\label{sec:vertex_transitive}

Let us formally introduce what we mean when we say that a realization is vertex-transitive.%(and later, edge-transitive, arc-transitive, ...).

\begin{definition}\label{def:vertex_transitive}
Given a graph $G$.
\begin{myenumerate}
	\item $\Sigma\subseteq\Aut(G)$ is called \emph{vertex-transitive} if it acts transitively on $V$.
	\item $G$ is called \emph{vertex-transitive} if $\Aut(G)$ is vertex-transitive.
	\item A realization is called \emph{vertex-transitive} if it is a $\Sigma$-realization for some~vertex-tran\-sitive $\Sigma\subseteq\Aut(G)$.
\end{myenumerate}
\end{definition}

The notions in points $(ii)$ and $(iii)$ can be adopted for all other kinds of transitivities that we will encounter later on, as \eg\ edge- or arc-transitivity.

\begin{observation}\label{res:vertex_transitive}
In a vertex-transitive realization $v$, every vertex can be mapped onto any other vertex by an orthogonal transformation.
Thus, all vertices must be on a common sphere of radius $r(v)$ around the origin.
%We say that the realization is \emph{inscribed}.
If the realization is norma\-lized, equation \eqref{eq:radius} states that for all $i\in V$ holds
%
\begin{equation}\label{eq:radius2}
\|v_i\|^2=[r(v)]^2=\frac dn.%=\frac{\dim U}n.
\end{equation}
\end{observation}

\begin{observation}\label{res:single_vertex}
A vertex-transitive $\Sigma$-realization $v$ is already determined by its representation $T$, and the placement of a single vertex, say $v_1$.
Since for every $i\in V$ there is a $\sigma\in \Sigma$ with $\sigma(1)=i$, we have
%
$$v_i=v_{\sigma(1)}=T_\sigma v_1.$$
%
Note however, that not all choices of $v_1\in\RR^d$ are feasible (see also \cref{res:fix_rigid}, or Construction 4.4 in \cite{winter2019geometry}).
\end{observation}

%Besides this observation on the metrics of vertex-transitive realizations, 
The rest of this section is devoted to a discussion on how vertex-transitivity (or the absence of it) influences rigidity.
Recall, that we already met vertex-transitive realizations that are rigid (the dodecahedron in  \cref{ex:dodecahedron}, rigidity will be proven in \cref{sec:distance_transitive}), or that are flexible (the truncated tetrahedron in \cref{ex:truncated_tetrahedron}).

%Conversely, if a realization is not balanced, it must be flexible \wrt\ to all $\Sigma\subseteq\Aut(G)$ for which it is a $\Sigma$-realization.
%In the special case of vertex-transitive realizations, we have the following further  criterion for rigidity:
%We further discuss a condition for rigidity for vertex-transitive realizations.

We start out with a rigidity-criterion specifically for vertex-transitive \mbox{realizations:}

\begin{lemma}%[\!\cite{winter2019geometry}, Theorem 5.11 $(ii)$]
\label{res:fix_rigid}
Given a vertex-transitive realization~$v\in$ $\mathcal R_d(G,\Sigma)$ with representa\-tion \mbox{$T\:\Sigma\to\Ortho(\RR^d)$}. Let $\Sigma_i:=\{\sigma\in\Sigma\mid \sigma(i)=i\}$ denote the stabilizer of $\Sigma$~at~$i\in V$\!, and define
%
$$\Fix(T,\Sigma_i):=\{x\in\RR^d\mid T_\sigma x=x \text{ for all $\sigma\in\Sigma_i$}\}\subseteq\RR^d.
$$
%
% (\cf\ \emph{\cite{winter2019geometry}}, Construction 4.4). 
If $\dim\Fix(T,\Sigma_i)=1$ for some (and then all) $i\in V$, then $v$ is rigid.
%
\begin{proof}
By $\dim\Fix(T,\Sigma_i)=1$ and $v_i\in\Fix(T,\Sigma_i)$ we have $\Fix(T,\Sigma_i)=\Span\{v_i\}$.

Suppose that $v$ can be deformed into $w\in\mathcal R_d(G,\Sigma)$.
Then (by an appropriate reorientation) both realization can be assumed to have the same \mbox{representation} $T$ (\cref{res:rigid} $(iii)$).
But then, for the same reason as for $v_i$, we have \mbox{$w_1\in\Fix(T,\Sigma_1)$} $=\Span\{v_1\}$, \ie\ $w_1=\alpha v_1$ for some $\alpha\in\RR$.
By vertex-transitivity (see \cref{res:single_vertex}) this holds for all vertices, that is, $v=\alpha w$. 

Hence $v$ cannot be deformed into a non-equivalent realization, and is rigid.
\end{proof}
\end{lemma}

We will make use of this in the proof of \cref{res:full_local_dimension_is_good}, when we study properties of \emph{arc-transitive} realizations.

From \cref{res:fix_rigid}, we immediately have that all 1-dimensional vertex-transitive realizations are rigid.
However, the converse of \cref{res:fix_rigid} is not true, that is, that there are rigid realizations with $\dim\Fix(T,\Sigma_i)$ $\ge 2$ for all $i\in V$.
%The existence of these is linked to the existence of exceptional group structures on spheres.

\begin{example}\label{ex:exception}
This phenomenon is not primarily linked to graph realizations~(it already occurs for point arrangements), but, for better visualization, we can demonstrate its effect on the cycle graph $C_n$ on $n\ge 3$ vertices $V=\{1,...,n\}$.

Consider the cyclic subgroup $\Sigma\subset\Aut(C_n)$ generated by the one-cycle permuta\-tion \mbox{$\sigma=(12\cdots n)\in\Sigma$}.
The group $\Sigma$ acts freely on $V\!$, that is, $\Sigma_i=\{\id\}$ for~all~verti\-ces $i\in V$.

Let $T\:\Sigma\to\Ortho(\RR^2)$ be the $\Sigma$-representation that maps \mbox{$\sigma\mapsto R_{2\pi/n}\in\Ortho(\RR^2)$ -- the} rotation of the plane by $2\pi/n$ around the origin. By $\Sigma_i=\{\id\}$ we necessarily have $\Fix(T,\Sigma_i)=\RR^2$ for all vertices $i\in V$.

Nevertheless, all non-zero realizations with the representation $T$ give the skeleton of the regular $n$-gon in different orientations,
%
\begin{center}
\includegraphics[width=0.45\textwidth]{img/rotated_8_gon_2}
\end{center}
%
and so all the realizations to this representation are equivalent, and no deformation is proper.
%This is because all realizations of $G$ with this representation are uniquely determined by the image of a single vertex, say $v_0$.
%Since there is a single permutation $\sigma_i\in\Sigma$ with $\sigma_i(0)=i$ (namely, the $i$-fold concatenation of $\sigma$), we have
%%
%$$v_i=T_{\sigma_i} v_0.$$


%Consider the cycle graph on the vertex set $V=\{0,...,n-1\}$ with edges $\{i,i+1\mod n\}$.
%Let $\Sigma:=\<\sigma\>\subset\Aut(G)$ be the cyclic subgroup generated by the permutation $\sigma\in\Aut(G)$ that maps $i\mapsto (i+1\mod n)$, and consider the representation $T\:\Sigma\to\Ortho(\RR^2)$ that sends $\sigma$ to the rotation matrix $R_{2\pi/n}$.
%
%We have $\Fix(T,\Sigma_i)=\RR^2$ for all $i\in V$, but still, any two realizations $v,v'$ of $G$ with representations $T$ will look the same, anemyl, like the skeleton of a regular $n$-polygon:
%
%\begin{center}
%\includegraphics[width=0.45\textwidth]{img/rotated_8_gon}
%\end{center}
%
%We can make this rigorous as follows:
%for every  $i\in V$ there is a unique symmetry $\sigma_i\in \Sigma$ with $\sigma_i(0)=i$, namely, $\sigma_i=\sigma\circ\cdots\circ \sigma$ exactly $i$ times. 
%Then the complete realization is determined by the placement of the point $v_0$:
%%
%$$v_i=T_{\sigma_i} v_0 = T_{\sigma\circ\cdots\circ \sigma} v_0 =({R_{2\pi/n} \cdots R_{2\pi/n}}) v_0  = R_{2\pi i/n} v_0.$$
%%
%Respectively for the realization $v'$.
%
%Now, the point $v_0'$ can be mapped onto the point $v_0$ by a map $X=c R_\alpha$ for some $c\ge 0$ and $\alpha\in[0,2\pi)$ (assuming that $v_1'$ is non-zero).
%But $X$ and $R_{2\pi i/n}$ commute, and so we have
%%
%$$v_i'=R_{2\pi i/n} v_0'=R_{2\pi i/n} X v_0= X R_{2\pi i/n} v_0 =  X v_i,$$
%%
%or $v'=Xv$ and the realizations are equivalent.
\end{example}

It would be interesting to determine the complete list of all exceptions, that is, of all rigid realizations with $\dim\Fix(T,\Sigma_i)\ge 2$ (see \cref{q:dim_fix_ge_2}).


\iffalse

Finally, we want to expand the previous results to not necessarily irreducible realization.
Note that the arrangement spaces of irreducible arrangement are always either identical or have trivial intersection.
This is not true for reducible arrangement, and so being non-orthogonal for these arrangement spaces does no longer constitute a good criterion for whether the realizations can be deformed into each other.
Instead, we have the following:

\begin{theorem}
Two realization $v,w\in\mathcal R_d(G,\Sigma)$ can be deformed into each other if and only if they can be decomposed into irreducible realization $v^{(k)},w^{(k)}\in\mathcal R_{d_k}(G,\Sigma)$ for $k\in\{1,...,K\}$ so that $v^{(k)}$ can be deformed into $w^{(k)}$.
%
\begin{proof}
We can assume that $v$ and $w$ are oriented so that they decompose into their irreducible components as in \eqref{eq:irreducible_decomposition}.
%
Then any family of deformations $v^{(k)}(t)\:[0,1]\to\mathcal R_{d_k}(G,\Sigma)$ from $v^{(k)}$ to $w^{(k)}$~provides a desired deformation from $v$ to $w$ simply via concatenation
%
$$v(t):=\big(v^{(1)}(t),...,v^{(K)}(t)\big).$$

For the converse, we can assume that the representation $T:=T(t)$ of $v(t)$ stays constant during the deformation. That is, we have fixed irreducible subspaces of $T$.
Then the projection of $v(t)$ onto the $k$-th subspace give a deformation of $v^{(k)}$ into $w^{(k)}$.
\end{proof}
\end{theorem}

\fi

We close this section with a note on what happens in the absence of vertex-transi\-tivity.
We show that for a not vertex-transitive graph all \enquote{interesting} \mbox{$\Sigma$-reali}\-zations (in a sense formalized in \cref{res:vertex_transitive_rigid}) are flexible.
This is because the vertices in each orbit can be placed independently of each other, creating a degree of freedom and preventing rigidity.

\begin{observation}
\label{res:vertex_transitive_rigid}
%If $\Sigma\subseteq\Aut(G)$ is not vertex-transitive, then all \enquote{interesting} $\Sigma$-
%realizations (in a sense formalized below) are flexible.
%This is because the vertices in each orbit can be placed independently of each other, creating a degree of freedom and preventing rigidity.
%
If the group $\Sigma$ does not act transitively on $V$, then $$V=V_1\cupdot\cdots\cupdot V_m$$ \mbox{decomposes} into $m\ge 2$ $\Sigma$-orbits $V_k$.
Now, if $v\: V\to\RR^d$ is a $\Sigma$-realization and $\alpha=(\alpha_1,...,\alpha_m)\in\RR^m$ is an $m$-tuple of real numbers, then the realization $v(\alpha)\: V\to\RR^d$, with~$v_i(\alpha):=$ $\alpha_k v_i$ whenever $i\in V_k$, is also~a~$\Sigma$-realization with the same repre\-sentation.
A continuous function $\alpha(t)\:[0,1]\to $ $\RR^m$ with $\alpha(0)=(1,...,1)$ induces a deformation $v(\alpha(t))$ from $v$ into $v(\alpha(1))$ (at least it does so under some conditions, that we discuss below).

For example, the deformation of the 6-cycle $C_6$, shown below, is of this form.~The group $\Sigma\subset\Aut(G)$ is choosen to have two orbits on $V$, indicated by the colors of the points. 
On the right, one of the orbits collapses to a single point in the origin.
%
\begin{center}
\includegraphics[width=0.8\textwidth]{img/non_balanced_with_symmetry_2}
\end{center}

Now, does this imply that a not vertex-transitive realization is always \mbox{flexible?~Not} necessarily: the deformation induced by $\alpha(t)$ might not be proper, as \eg\ in the~case of the \enquote{rhombus realization} of the 4-cycle $C_4$ shown below:
%
\begin{center}
\includegraphics[width=0.65\textwidth]{img/rhombus_deformation}
\end{center}
%
Again, this is a deformation of the form discussed above, but this time, all $v(\alpha(t))$ are equivalent.
Note further, that the realization on the right is not part of this deformation as it is not full-dimen\-sional (recall that $\mathcal R_d(G,\Sigma)$ contains only full-dimensional realizations).
In~fact,~these $\Sigma$-realizations of $C_4$ are reducible, and~the right-most image shows one of the irreducible components of this $\Sigma$-realization instead.

%%
%The image shows the previously described deformation of the rhombus-realization of the 4-cycle $C_4$ (for a $\Sigma\cong \Bbb Z_2 \times \Bbb Z_2$, the vertex-orbits are indicated by color).
%Firstly, the \enquote{squishing} if the square is not a proper deformation, but happens by linear transformation. Secondly, the right-most image is not part of the deformation
%
%\TODO
%
%Let $\Sigma\subseteq\Aut(G)$ be some non-transitive group of symmetries, so that we have a decomposition $V=V_1\cupdot\cdots \cupdot V_m$ of the vertex set $V$ into~$m\ge 2$ $\Sigma$-orbits.
%Let further $v\: V\to\RR^d$ be an irreducible $\Sigma$-realization with $\Sigma$-representation $T$.
%For each $\mathcal N_k:=\{v_i\mid i\in V_k\}$, the subspace $\Span (\mathcal N_k)$ is $T$-invariant.
%Since $v$ is irreducible, $\Span (\mathcal N_k)$ is either $\{0\}$ or $\RR^d$.
%%In the following, assume that $\Span(\mathcal N_k)=\RR^d$ for all $k\in\{1,...,m\}$.
%
%
%Then~any~tuple~\mbox{$\alpha=(\alpha_1,...,$} $\alpha_m)\in\RR^m$ of non-zero real numbers gives us another $\Sigma$-realization $w(\alpha)\: V\to\RR^d$ via~$w_i:=\alpha_k v_i$ whenever $i\in V_k$.
%A continuous curve $\alpha(t)\:[0,1]\to\RR^m$ with, say $\alpha(1)=(1,...,1)$, gives use a deformation $w(\alpha(t))$ from $w(\alpha(0))$ into $w(\alpha(1))=v$.
%An example is shown in the image below:
%%
%\begin{center}
%\includegraphics[width=0.65\textwidth]{img/non_balanced_with_symmetry_2}
%\end{center}
%%
%In this example $\Sigma\subset\Aut(C_6)$ is a subgroup of the symmetry group of the 6-cycle that acts edge-transitively, but not vertex-transitively on $C_6$.
%
%So, does this give us that $v$ is flexible?
%Not necessarily, as this deformation must not be proper.
%\TODO\msays{Example rhombus}

Let us try to understand what distinguishes these two examples.
%For simplicity, assume that $v$ is irreducible and that $m=2$, \ie\ $V=V_1\cupdot V_2$.
Suppose that $v$ is irreducible with representation $T$.
Define the sets $\mathcal N_k:=\{v_i\mid i\in V_k\}$ for all $k\in\{1,...,m\}$ (the image of the orbit $V_k$ under the realization $v$).
If $\mathcal N_k =\{0\}$ (as for the \enquote{white} orbits in the two right images), then~this is equivalent to ignoring the orbit $V_k$, and we could have studies $V\setminus  V_k$ instead.
Let us therefore assume that all these sets are non-zero.
Note that $\Span (\mathcal N_k)$ is a $T$-invariant subspace of $\RR^d$.
Since $v$ is irreducible and $\mathcal N_k$ is non-zero, we necessarily have $\Span(\mathcal N_k)=\RR^d$.
But then, if a transformation of $\RR^d$ fixes one of the $\mathcal N_k$ point-wise, this transformation must be the identity, hence fixes all $\mathcal N_k$ point-wise.
For such realizations, deformations of the form $v(\alpha(t))$ are indeed proper, and $v$ is flexible.
%
\end{observation}

\begin{corollary}
\label{res:vertex_transitive_rigid_cor}
If an irreducible realization is not vertex-transitive but has at least two non-zero orbits on the vertices (the $\mathcal N_i$ in \cref{res:vertex_transitive_rigid}), then the realization is flexible.
\end{corollary}
%Some nice examples of these deformations can be found in \cref{sec:arc_transirive}, when we discuss edge-transitive realizations.

The quintessence of \cref{res:vertex_transitive_rigid} and \cref{res:vertex_transitive_rigid_cor} is meant to be the following: the study of rigidity is much more interesting for vertex-transitive realizations, and we shall therefore focus on these.





%\subsection{Summary}
%
%The take away messages of this section are:
%
%\begin{itemize}
%\item When studying rigidity, it seems plausible to focus 
% on vertex-transitive~reali\-zations.
%\end{itemize}





\iffalse

\tempnewpage
\section{Vertex-transitive realizations}

For a vertex-transitive realization $v$, the arrangement space $U\subseteq\RR^n$ contains a distinguished vector:

\begin{definition}
The \emph{cosine vector} $u\in\RR^n$ of a vertex-transitive realization $v$ with a fixed vertex $i\in V$ is the vector with components $u_j:=\<v_i,v_j\>$ for all $j\in V$.
\end{definition}

Since $v$ is vertex-transitive, this vector is indeed well-defined and independent of the choice of $i\in V$.

\begin{corollary}
If two irreducible vertex-transitive realizations have non-orthogonal cosine vectors, then they can be deformed into each other.
\end{corollary}


\begin{proposition}
If $\Eig_G(\theta)$ is $\Sigma$-reducible, then there exist two balanced $\Sigma$-realizations with eigenvalue $\theta$ and orthogonal cosine vectors.
\end{proposition}


\fi




\iffalse

\tempnewpage
\section{Symmetric and rigid graph realizations}
\label{sec:realizations}

This section collects basic terminology and results for graph realizations, arrange\-ment spaces, symmetric and rigid realizations, as well as the necessary prerequisites in representation theory.
Details can be found in \cite{winter2019geometry}, in particular, proof for all~the listed theorems.

For the rest of the paper, let $G=(V,E)$ denote a (simple) graph on the vertex~set $V=\{1,...,n\}$, that is, with $n$ vertices.

\subsection{Graph realizations}
\label{sec:graph_realizations}

A graph is a purely combinatorial object without any geometric information.
Such information can be attached to the graph using \emph{graph realizations}.
One can imagine this as embedding the vertices of the graph in Euclidean space, and consider its edges embedded as straight lines.

\begin{definition}
\quad %Given a graph $G$.
\begin{myenumerate}
\item
A \emph{($d$-dimensional) realization} of $G$ is a map $v\:V\to\RR^d$. The image of a vertex $i\in V$ is denoted using the subscript $v_i$.
\item The realization is \emph{full-dimensional} if $\rank v:= \dim \Span\{v_1,...,v_n\}=d$.
%\item Two realizations $v,w:V\to\RR^d$ are called \emph{equivalent}, if they are related by an invertible linear transformation, that is, there is a $T\in\GL(\RR^d)$ so that $v_i=T w_i$ for all $i\in V $, or short, $v=Tw$.
\end{myenumerate}
\end{definition}

%Note that we neither require a realization to map different vertices onto different points in $\RR^d$, nor to ensure that edges are disjoint or do not contain vertices.

Our intention is to study full-dimensional realizations up to orthogonal transformations.
If a realization is not full-dimensional, one can restrict it to its span.
We can therefore assume that our realizations are always full-dimensional.

We do mostly care about metric properties of the realizations, that is, angles and distances, but less about its orientation in space.
That is, we will not distinguish between a realization $v$, and a realization $w:= Tv$\footnote{We use this shorthand notation for $w_i=T v_i$ for all $i\in V$.} for some orthogonal map~$T\in\Ortho(\RR^d)$.

%The intention of this paper is to look at full-dimensional realizations.
%Also, we are mostly interested in arrangements up to orthogonal transformations.
%That is, we care about metric properties like angles and distances, but do not care about the orientation in space.
%Occasionally, if we are only interested in the angles, we do also ignore scale.

\subsection{Arrangement spaces}
\label{sec:arrangement_spaces}

Arrangement spaces provide a different perspective onto arrangements of points in general.

%We introduce our main tool for handling realizations:

\begin{definition}
Given a realization $v\:V\to\RR^d$ of $G$.
\begin{myenumerate}
\item
The \emph{(arrangement) matrix} of $v$ is the matrix
%
$$M :=
\begin{pmatrix}
	\;\horzbar\!\!\!\! & v_1\T & \!\!\!\!\horzbar\;\; \\
	& \vdots & \\[0.4ex]
	\;\horzbar\!\!\!\! & v_n\T & \!\!\!\!\horzbar\;\;
\end{pmatrix}\mathrlap{\in\RR^{n\times d},}$$
%
in which the $v_i$ are the rows.
\item 
The realization is called \emph{spherical} if $M\T\!M\!=\alpha\Id$ for some $\alpha> 0$, and is called \emph{normalized} if $M\T\!M=\Id$.
\item
The \emph{arrangement space} of $v$ is the column span $U:=\Span(M)\subseteq\RR^n$.
\item Two realizations with the same arrangement space are called \emph{equivalent}.
\end{myenumerate}
\end{definition}

%If not mentioned otherwise, in the following $M$ shall always denote the arrangement matrix of $v$, and $U$ its arrangement space.

The arrangement spaces of a realization is a convenient tool in a variety~of~situation, as we shall demonstrate in the upcoming sections.
Foremost, the arrangement spaces helps us to hide the distinction between realizations that we want to consider the same:

\begin{theorem} Given two $d$-dimensional realizations $v,w\:V\to\RR^d$.
\begin{myenumerate}
	\item 
	$v$ and $w$ are equivalent if and only if they are related by an invertible linear transformation $T\in\GL(\RR^d)$.
	\item 
	if $v$ and $w$ are \ul{spherical}, they are equivalent if and only if they are related~by a conformal transformation $\alpha T$, where $T\in\Ortho(\RR^d)$ and $\alpha\in\RR\nozero$.\footnote{We use the term \emph{conformal} to mean an angle preserving linear transformation.}
	\item 
	if $v$ and $w$ are \ul{normalized}, they are equivalent if and only if they~are~related by an orthogonal transformation $T\in\Ortho(\RR^d)$.
\end{myenumerate}
\end{theorem}

Consequently, properties independent of invertible transformations are uniquely determined by the arrangement space alone.
For example, it holds \mbox{$\rank v = \rank M$} $= \dim U$.
So, if $v$ is full-dimensional, then $\dim U=d$.
In particular, this is the case if $v$ is spherical, since then $M\T\! M=\alpha\Id$ is of rank $d$, and so is $M$.

If $v$ is spherical, the arrangement space determines properties preserved by conformal maps, that is, angles, and if $v$ is even normalized, it additionally determines distances.
For example, the \emph{radius} $r(v)$ of a normalized realization satisfies
%
\begin{equation}\label{eq:radius}
[r(v)]^2:= \frac1n \sum_{i\in V} \|v_i\|^2 = \frac1n \tr\underbrace{(M\T\! M)}_{\Id} =\frac dn = \frac{\dim U}n.
\end{equation}
%
%where in $(*)$ we use that $v$ is normalized, that is $M\T\!M=\Id$, and in $(**)$ we used that spherical realizations are full-dimensional.
%

%Most of the time it will be convenient and permissible to assume that all our~reali\-zations are normalized, which in the case of a spherical realization can be achieved by a simple rescaling.

%Here are some conveniences of the term spherical and normalized:

%\begin{proposition} \quad%Let $v:V\to\RR^d$ be a realization of $G$.
%\begin{myenumerate}
%	\item Spherical realizations are full-dimensional.
%	\item Two normalized arrangements are equivalent (have the same arrangement space) if and only if they are related by an orthogonal transformation.
%\end{myenumerate}
%\end{proposition}
%

\begin{observation}\label{res:realizations_and_arrangement_spaces}
Conversion between realizations and their arrangement spaces is straight-forward in practice:
%
\begin{myenumerate}
	\item For any subspace $U\subseteq\RR^n$, one can construct all full-dimensional \mbox{realizations} with arrangement space $U$ as follows:
	choose any basis $\{u_1,...,u_d\}\subset~U$~and let $M=(u_1,...,u_d)\in\RR^{n\times d}$ be the matrix with the $u_i$ as columns.~The reali\-zation $v\:V\to\RR^d$, for which $v_i$ is the $i$-th row of $M$, is full-dimensional,~has matrix $M$ and arrangement space $U$.
	
If one choose $\{u_1,...,u_d\}\subset U$ as an \emph{orthonormal basis}, then $v$ is a~\emph{norma\-lized} realization.
In general, if we construct a realization from its arrangement space, it is convenient to assume that the result is normalized.

	\item
	If $v$ is a realization with arrangement space $U$, then the vectors $u\in U$ are exactly the vectors with components
	%
	\begin{equation}
	\label{eq:vectors}
	u_i = \<v_i,x\>,\qquad\text{for all $i\in V$},
	\end{equation}
	%
	for some $x\in\RR^d$. To see this, note that \eqref{eq:vectors} can be written as $u=Mx$.%,~and that $U=\im M$ when considering $M$ as a map $M\:\RR^d\to\RR^n$.
\end{myenumerate}
\end{observation}

%\begin{proposition}\label{res:vectors}
%If $v$ is a $d$-dimensional realization with arrangement space $U\subseteq\RR^n$, then the vectors $u\in U$ are exactly the vectors with components
%%
%\begin{equation}
%\label{eq:vectors}
%u_i = \<v_i,x\>,\qquad\text{for all $i\in V$},
%\end{equation}
%%
%for some $x\in\RR^d$.
%%
%\begin{proof}
%If $M$ is the arrangement matrix of $v$, then \eqref{eq:vectors} is equivalent to $u=Mx$.
%
%\TODO
%\end{proof}
%\end{proposition}


\subsection{Symmetric realizations}
\label{sec:symmetric_realizations}

Often it is desired to realize a graph not just in~any way, but so that important features of its structure become apparent.
For example, one could ensure that all (or at least some important) combinatorial symmetries of $G$ become geometric symmetries of the realization.
Such realizations shall be called \emph{symmetric realizations}.
The formal counterpart are the \emph{$\Sigma$-realizations}:


%This leads to the concept~of~\emph{sym\-metric realizations}.

\begin{definition}
Given a group $\Sigma\subseteq\Aut(G)$ of symmetries of $G$.
\begin{myenumerate}
\item 
A realization $v$ is called a \emph{$\Sigma$-realization} of $G$ if there exists a linear (orthogonal) representation  $T\:\Sigma\to\Ortho(\RR^d)$ with
%
\begin{equation}\label{eq:symmetric_realization}
T_\sigma v_i=v_{\sigma(i)},\quad\text{for all $i\in V$ and $\sigma\in\Sigma$}.
\end{equation}
%
%We call $v$ a \emph{symmetric realization} if $\Sigma$ is not further specified.
If $v$ is full-dimensional (as we shall always assume), then this representation is uniquely determined and we call it \emph{the realization} of $v$.

%\item 
%A $\Sigma$-realization with $\Sigma=\Aut(G)$ is called \emph{symmetric realization} of $G$.
\item 
A $\Sigma$-realization is called \emph{irreducible} if its representation is irreducible, and it is called \emph{reducible} otherwise %(if $v$ is full-dimensional, the representation is unique and irreducibility is well-defined; if $v$ is not full-dimensional, every representation is reducible.).
\end{myenumerate}
\end{definition}

%We will use the term \emph{symmetric realization} in a partially informal sense to mean any realization of $G$ that realizes some (or all) of its symmetries.

Note that we defined the representation of a $\Sigma$-realization to attains values~in~the \emph{orthogonal} matrices only, since finally, we are interested in the Euclidean symmetries of geometric objects, and these are isometries of $\RR^d$.

The group $\Aut(G)$ of combinatorial symmetries of $G$ is a subgroup of $\Sym(V)$,~\ie\ the group of permutations on $V$.
To any permutation $\phi\in\Aut(G)$ we can associate a \emph{permutation matrix} $\Pi_\phi\in\Perm(n)\subseteq\Ortho(\RR^n)$.

Recall the following basics of representation theory:
a subspace $U\subseteq\RR^n$ is called \emph{$\Sigma$-invariant} (or just \emph{invariant}) if for any $\phi\in\Sigma$ holds $\Pi_\phi U\subseteq U$.
Trivially, $\{0\}$ and $\RR^n$ are always invariant.
A $\Sigma$-invariant subspace $U\subseteq \RR^d$ is called \emph{irreducible}~if~it~has no non-zero $\Sigma$-invariant subspaces.

The connection of symmetric realizations to arrangement spaces is as follows:

%Symmetric realizations can be characterized using their arrangement spaces:

\begin{theorem}\label{res:symmetric_realizations}
Given a group $\Sigma\subseteq\Aut(G)$ of symmetries of $G$.
\begin{myenumerate}
	\item If $v$ is a $\Sigma$-realization, then its arrangement space is a $\Sigma$-invariant subspace of $\RR^n$. If $v$ is spherical, then the converse holds.
	% If $v$ is normalized, then~the representation can be given explicitly as 
	%
	%$$T_\phi := M\T\! \Pi_\phi M, \qquad\text{for all $\phi\in\Sigma$}.$$
	\item If $v$ is an irreducible $\Sigma$-realization, then it is spherical.
\end{myenumerate}
\end{theorem}

%It is point $(ii)$ in above theorem which justifies to restrict to spherical and normalized realizations in most cases.

In theory, one can determine the $\Sigma$-invariant subspaces of $\RR^n$, and from this,~expli\-citly construct the $\Sigma$-realizations of $G$ as explained in \cref{res:realizations_and_arrangement_spaces} $(i)$.
In~prac\-tice, this is more complicated.
There is an easier way if one has already access to~a linear representation $T\:\Sigma\to\Ortho(\RR^d)$: %, then there are straight-forward procedure to construct all $\Sigma$-realization with representation $T$.

\begin{example}\label{ex:fix}
For simplicity, suppose $\Sigma\subseteq\Aut(G)$ atcs transitively on the vertices.
%
Let $\Sigma_1:=\{\sigma(1)=1\mid\sigma\in\Sigma\}\subseteq\Sigma$ be the \emph{stabilizer} of $1\in V$ of $\Sigma$.
Choose~a~point
%
$$v_1\in\Fix(T,\Sigma_1):=\{v\in \RR^d \mid T_\sigma v =  v \text{ for all }\sigma\in \Sigma_1\}.$$
%
By transitivity, for any $i\in V$ there is a $\sigma_i\in\Sigma$ with $\sigma_i(1)=i$.
The realization~$v$~with $v_i:=T_{\sigma_i} v_1$ is then a $\Sigma$-realization of $G$.
%A~$\Sigma$-reali\-zation with representation $T$ can then be defined via $v_i:= T_{\sigma_i} v_1$.
\end{example}

If $\Fix(T,\Sigma_1)=0$, then this indicates that no (non-trivial) $\Sigma$-realization with this representation exists.
On the other hand, if $\dim\Fix(T,\Sigma_1)\ge 2$, then one~has~non-trivial choices for the value of $v_1$, and different such choices might lead to non-equi\-valent $\Sigma$-rea\-li\-zations.
A continuous transition between different such values for $v_1$ then induces a continuous transition between non-equivalent realization.
This leads to the notion of \emph{rigidity}.


\subsection{Rigid realizations}
\label{sec:rigid_realizations}

Let $\mathcal R_d(G,\Sigma)$ denote the space of \emph{full-dimensional} \mbox{$\Sigma$-reali}\-zations of $G$ in $\RR^d$, equipped with its natural topology.

We are interested in continuous transitions between symmetric realizations, so that each intermediate realization is not less symmetric.

\begin{definition}\quad
\begin{myenumerate}
	%\item A \emph{$\Sigma$-deformation} is a continuous tranformation of a non-zero $\Sigma$-realization so that any intermediate step is itself a non-zero $\Sigma$-realization.
	%\item A \emph{$\Sigma$-deformation} $v(\free)$ is a continuous curve in $\mathcal R_d(G,\Sigma)$.
	\item
	Given two $\Sigma$-realizations $v^0,v^1\in\mathcal R_d(G,\Sigma)$, we say that $v^0$ can be \emph{\mbox{deformed} into} $v^1$ if there is a continuous curve $v(\free)\:[0,1]\to\mathcal R_d(G,\Sigma)$ with~$v(0)=v^0$ and $v(1)=v^1$.
	%\item A $\Sigma$-deformation $v(\free)$ is called \emph{trivial} if the arrangement space $U(t)$ of $v(t)$ does not depend on $t$.
	\item A $\Sigma$-realization is called \emph{rigid} if it cannot be deformed into a non-equivalent $\Sigma$-realization. It is called \emph{flexible} otherwise.
\end{myenumerate}
\end{definition}


Note that equivalent arrangements are not necessarily congruent.
A \mbox{deformation} of a square into a rhombus or a rectangle involves only invertible linear transformations and is no witness of flexibility.

\begin{center}
\includegraphics[width=0.7\textwidth]{img/flexible_rigid}
\end{center}

%The standard way to product a transition between two non-equivalent $\Sigma$-realiza\-tions $v^1,v^2\in\mathcal R_d(G,\Sigma)$ is by linear interpolation:
%%
%$$v(t):= tv^1 + (1-t) v^2.$$
%%
%If both realizations have the same representation $T$, then $v(t)$ as representation $T$ for all $t\in[0,1]$.
%If further the $v^i$ are irreducible, then $v(t)$ is full-dimensional.

%There are different way by which to check whether a given realization is actually rigid. 

Ultimately, whether a certain $\Sigma$-realization is rigid or flexible has to do with~the decomposition of the permutation representation $\Sigma\ni\phi\mapsto\Pi_\phi$ into irreducible constituents.
%
For us, the following geometric criteria are sufficient:

%For our purpose, we can use the following more geometric criteria.

\begin{theorem}\label{res:rigidity_criteria}
\quad

\begin{myenumerate}
\item 
If $v$ is a $\Sigma$-realization with representation $T$ and $\dim\Fix(T,\Sigma_i)=1$ for all $i\in V$ (\cf\ \cref{ex:fix}), then $v$ is rigid.
\item
If two irreducible $\Sigma$-realizations have non-orthogonal arrangement spaces, then they can be deformed into each other.
\end{myenumerate}
\end{theorem}

By \cref{res:rigidity_criteria} $(i)$, 1-dimensional realizations are always rigid.
Also, the converse of $(i)$ is not true: there exist realizations with $\dim\Fix(T,\Sigma_i)\ge 2$, which are still rigid.
These are linked to the exceptional groups structures on spheres.

 \iffalse


\begin{theorem}\label{res:fix_rigid}
If $v$ is a $\Sigma$-realization with representation $T$ and $\dim\Fix(T,\Sigma_i)=1$ for all $i\in V$ (\cf\ \cref{ex:fix}), then $v$ is rigid.
\end{theorem}


%However, $\dim\Fix(T,\Sigma_i)= 1$ is not necessary for rigidity.
%For \mbox{example,~let} $v$ be~a $\Sigma$-realization of the cycle graph $C_n$ where $\Sigma\subset\Aut(C_n)$ is the cyclic group~on~$n$~ele\-ments (rather than the full dihedral group).

\begin{theorem}\label{res:arrangement_space_rigid}
If two irreducible $\Sigma$-realizations have non-orthogonal arrangement spaces, then they can be deformed into each other.
\end{theorem}

%\begin{theorem}
%If the irreducible $\Sigma$-realization $v$ has arrangement space $U\subseteq\RR^n$ and there is another $\Sigma$-invariant subspace $\tilde U\subseteq\RR^n$ with $U\cap\tilde U=\eset$ but $U\not\perp\tilde U$, then $v$ is flexible.
%\end{theorem}
%
%\begin{theorem}
%Given an irreducible $\Sigma$-realization $v$ with arrangement space \mbox{$U\subseteq\RR^n$}.
%\begin{myenumerate}
%\item
%If there is a $\Sigma$-invariant subspace $U'\subseteq\RR^d$, non-orthogonal to $U$ but $U\cap U'=\eset$, then $v$ is flexible.
%\item
%If $w$ is an irreducible $\Sigma$-realization with an arrangement space non-orthogonal to $U$, then $w$ can be deformed into $v$.
%\end{myenumerate}
%\end{theorem}

Each decomposition of $\RR^n=U_1\oplus \cdots \oplus U_m$ into mutually orthogonal $\Sigma$-invariant subspaces $U_i\subseteq\RR^n$ provides another cirterior for flexibility:

\begin{corollary}
Let
 $v$ is a $\Sigma$-realization with its arrangement space not contained in any of the $U_i$, then $v$ is flexible.
\end{corollary}




There is a generic way by which to generate criteria for flexibility.
For this,~fix a decomposition of $\RR^d=U_1\oplus\cdots\oplus U_m$ into mutually orthogonal $\Sigma$-invariant subspaces $U_i\subseteq\RR^n$.
If an irreducible $v$ now has arrangement space $U$ that is not contained in any of the $U_i$, its necessarily non-orthogonal to some $U_i$.
The orthogonal projection $U':=\pi_{U_i}(U)$ of $U$ onto $U_i$ is again an irreducible invariant subspace of $\RR^n$.
If now $v'$ is the irreducible $\Sigma$-realization with arrangement space $U'$, then $v$ and $v'$ have non-orthogonal arrangement spaces, can be deformed into each other and are flexible.

\fi








\tempnewpage

\begin{itemize}
\item define graph realization
\item define symmetric realization
\item define balanced realization
\item define spectral realization
\item define arrangement matrix/space and show that these terms can be expressed using these
\item define spherical/normalized arrangement
\end{itemize}


\tempnewpage

Given a (simple) graph $G=(V,E)$, a \emph{realization} $v\:V \to\RR^d$ of $G$ is an embedding of this graph into some Euclidean space.
Its vertices are embedded as points in $\RR^d$, and its edges as straight lines between these points.

The purpose of this paper is to study the connections between two interesting classes of such realizations: \emph{symmetric} realizations, and \emph{spectral} realizations.



%The image below depicts four different 2-dimensional realizations $v^1,v^2,v^3$ and $v^4$ of the cycle graph $C_4$, some of which appear as more symmetric than others.
The image below depicts several different 2-dimensional realizations of the cycle graph $C_4$, some of which appear to be more symmetric than others.
%
\begin{center}
%\includegraphics[width=0.6\textwidth]{img/C4_realizations}
\includegraphics[width=0.9\textwidth]{img/C4_realizations_2}
\end{center}

The idea of being \enquote{more or less symmetric} can be formalized using the concept of \emph{symmetric realizations}:
%
given a group $\Sigma\subseteq\Aut(G)$ of some or all symmetries of $G$, a realization is called \emph{$\Sigma$-realization}, if 
% $v$ geometrically realizes the combinatorial symmetries in $\Sigma$.
%More formally,
there is a linear (orthogonal) representation $T\:\Sigma\to\Ortho(\RR^d)$ of $\Sigma$ so that
%
$$T_\phi v_i= v_{\phi(i)},\quad\text{for all $i\in V$ and $\phi\in\Sigma$}.$$

In this paper we study the symmetric realizations of graphs with a lot of symmetries, which for us means at least vertex- or edge-transitivity.
We investigate the various implications of a realization being symmetric, for example \wrt\ geometry, topology and spectral graph theory.


\tempnewpage

\section{Graph realizations}
\label{sec:realizations}

\begin{definition}
A $d$-dimensional \emph{realization} of $G$ is a map $v\: V\to\RR^d$.
The image of $i\in V$ is denotes as subscript $v_i$.
\end{definition}

In the following we shall suppose that our realizations are \emph{full-dimensional}, that is, that $\rank v:=\dim\Span\{v_1,...,v_n\}=d$.

The image below depicts four different 2-dimensional realizations $v^1,v^2,v^3,v^4$ of the cycle graph $C_4$, some of which are apparently more symmetric then others.
%
\begin{center}
\includegraphics[width=0.6\textwidth]{img/C4_realizations}
\end{center}
%
This idea of being \enquote{more or less symmetric} is captured by the concept of \emph{symmetric realizations}:

\begin{definition}
Given a group $\Sigma\subseteq\Aut(G)$ of symmetries of $G$.
%
%\begin{myenumerate}
	%\item 
	
	A realization $v$ is called \emph{$\Sigma$-realization} if there is a linear (orthogonal) representation $T\:\Sigma\to\Ortho(\RR^d)$ with
	%
	$$T_\phi v_i= v_{\phi(i)},\quad\text{for all $i\in V$ and $\phi\in\Sigma$}.$$
	%
	If $v$ is full-dimensional (as we shall always assume), then $T$ is uniquely determined and we call it \emph{the representation} of $v$.
	
	A $\Sigma$-realization is called \emph{irreducible} if its representation is irreducible.
%\end{myenumerate}
\end{definition}

The square $v^4$ is a $\Sigma$-realizations for all $\Sigma\subseteq\Aut(G)$.
The rectangle $v^3$ cannot be a $\Sigma$-realization for $\Sigma$ that act transitively on the edges of $C_4$, and the rhombus $v^2$ cannot be a $\Sigma$-realization for $\Sigma$ that act transitively on the edges of $C_4$.
The realization $v_1$ is a $\Sigma$-realization only for $\Sigma=\{\id\}$.
Of these, only $v^4$ can have an irreducible representation if \eg\ $\Sigma=\Aut(G)$.

Note that we require $T$ to be a representation taking on values in the \emph{orthogonal matrices} (rather than general invertible matrices), as this is more in line with our idea of rigid symmetries.
If we allow general linear representations, the rectangle and rhombus would also be $\Sigma$-realizations for all $\Sigma\subseteq\Aut(G)$.

Here is an easy way to construct symmetric realizations:

\begin{example}\label{ex:construction}
Suppose that we are given a \emph{vertex-transitive} group $\Sigma\subseteq\Aut(G)$ of symmetries and a representation $T\:\Sigma\to\Ortho(\RR^d)$ thereof.

Let $\Sigma_1:=\{\phi\in\Sigma\mid\phi(1)=1\}\subseteq \Sigma$ denote the \emph{stabilizer} of $\Sigma$ at $1\in V$ and define
%
$$\Fix(T,\Sigma_1):=\{x\in\RR^d\mid T_\phi x=x\text{ for all $\phi\in \Sigma_1$}\}=\bigcap_{\mathclap{\phi\in\Sigma_1}} \ker(T_\phi-\Id)\subseteq\RR^d,$$
%
which is a linear subspace or $\RR^d$.

Fix a $v_1\in\Fix(T,\Sigma_1)$.
Since $\Sigma$ is vertex-transitive, for any $i\in V$ we can further fix a $\phi_i$ with $\phi_i(1)=i$.
Then let $v\: V\to\RR^d$ be the realization that maps $i\in V$ to $v_i:=T_{\phi_i} v_1$.
This is indeed a $\Sigma$-realization of $G$ with representation $T$.
\end{example}

In general, only given the graph $G$, one has neither easy access to $\Aut(G)$ nor~to any specific representation thereof, and it is hard to construct a symmetric realization as in \cref{ex:construction}.
Spectral realizations are an easy fix for this problem.

First we introduce the little brother of spectral realizations:



\begin{definition}
A realization $v\:V\to\RR^d$ of the graph $G$ is called \emph{balanced}, if there is a number $\theta\in\RR$ with
%
\begin{equation}\label{eq:balanced}
\sum_{\mathclap{j\in N(i)}} v_j = \theta v_i,\quad\text{for all $i\in V$}.
\end{equation}
\end{definition}

The image below depicts two realizations of the cycle graph $C_8$.
The left realiza\-tion is balanced with $\theta=\sqrt 2$, the right one is not balanced.
%
\begin{center}
\includegraphics[width=0.45\textwidth]{img/balanced}
\end{center}
%
To understand which values are possible for $\theta$, define the \emph{arrangement matrix} $M\in\RR^{n\times d}$ in which the $i$-th row is given by $v_i^{\smash\top}$:
%
$$
M:=
\begin{pmatrix}
	\;\horzbar\!\!\!\! & v_1\T & \!\!\!\!\horzbar\;\; \\[-0.4ex]
	& \vdots & \\[0.45ex]
	\;\horzbar\!\!\!\! & v_n\T & \!\!\!\!\horzbar\;\;
\end{pmatrix}\in\RR^{n\times d}.
$$
%
Then equation \eqref{eq:balanced} can be written as $AM=\theta M$, where $A$ is the adjacency matrix of $G$.
It becomes apparent, that the columns of $M$ are eigenvectors to eigenvalue $\theta\in\Spec(G)$.
In other words, there is a balanced realization with value $\theta$ if and only if $\theta$ is an eigenvalue of $G$ (that is, of its adjacency matrix).
The value $\theta$ is therefore also called the \emph{eigenvalue} of the balanced realization $v$.

\begin{definition}
$v$ is called \emph{spectral realization} of $G$, or \emph{$\theta$-realization}, if it is balanced with eigenvalue $\theta$, and its dimension is the multiplicity of $\theta$.
\end{definition}


Such realizations can be constructed as follows:

\begin{example}
Let $u_1,...,u_d\in\RR^n$ be a complete set of $\theta$-eigenvectors of $G$, that is, they span the $\theta$-eigenspace $\Eig_G(\theta)$ of $G$.
Let $M=(u_1,...,u_d)\in\RR{n\x d}$ be the matrix in which the $u_i$ are the columns.
This is the arrangement matrix of the $\theta$-realization.
\end{example}

Given the fact that we have usually access to fast and accurate algorithm to compute all eigenvectors to an eigenvalue of $G$, this provides a worthy substitute to symmetric realizations.
For this to be true, we have to show that spectral realizations are symmetric in some sense. We shall do this in the context of arrangement spaces.


\tempnewpage

\section{Arrangement spaces}

Arrangement spaces often provide a convenient second point of view on concepts and problems involving point arrangement.
Most results in this paper will have an interpretation in the context of arrangement spaces.

\begin{definition}
For a realization $v$ with arrangement matrix $M$, the column span $U:=\Span M$ is called \emph{arrangement space} of $v$.

Two realizations with the same arrangement space are called \emph{equivalent}.
\end{definition}

\begin{theorem}
Two realizations $v$ and $w$ are equivalent if and only if they are related by an invertible linear transformation, that is, there is a $T\in\GL(\RR^d)$ so that $Tv=w$.
\end{theorem}

\begin{theorem}
Given a realization $v$ with arrangement space $U$.
\begin{myenumerate}
	\item If $U$ is $\Sigma$-invariant, then $v$ is a $\Sigma$-realization. If $v$ is spherical, then the~con\-verse holds.
	\item $v$ is the $\theta$-realization of $G$ if and only if $U=\Eig_G(\theta)$.
	\item $v$ is balanced if and only if $U\subseteq\Eig_G(\theta)$.
\end{myenumerate}
\end{theorem}

Since eigenspaces of $G$ are always $\Aut(G)$-invariant, the following is an immediate consequence:

\begin{corollary}
Spectral realizations realize all the symmetries of $G$, that is, they are $\Aut(G)$-realizations.
\end{corollary}

The converse is not true in general, not even if we restrict to
 irreducible realizations: not every irreducible $\Aut(G)$-realization is spectral or even balanced.
There are two obstructions to this:
%
\begin{myenumerate}
	\item eigenspaces need not be irreducible as an $\Aut(G)$-invariant subspace. In other words, an irreducible $\Aut(G)$-invariant subspace might not be the whole eigenspace, but only a subspace. If this would be the only problem, irreducible $\Aut(G)$-realizations would at least be balanced. But
	\item invariant subspaces might not even be contained in eigenspaces, hand hence the corresponding realization might not be balanced. This leads to the notion of rigid realizations.
\end{myenumerate}
This is because eigenspaces are not necessarily irreducible \wrt\ $\Aut(G)$, but might decompose into several irrecubiel invariant subspaces.







\tempnewpage

\section{Spectral graph realizations}
\label{sec:spectral_realizations}

Symmetric realizations are useful but hard to obtain in practice.
There are~techniques to construct the invariant subspaces of $\Aut(G)$, but chances are, one has not even immediate access to $\Aut(G)$ and~has~to~first~extract it from the combinatorial data of the graph.

In most cases, spectral realizations present a worthy substitute. 
Here, one makes use of the well developed theory for computing eigenvalues and eigenvectors. 

Recall that by \emph{spectrum}, \emph{eigenvalue}, \emph{eigenvector} and \emph{eigenspace} of a graph $G$,~one actually refers to the respective quantities of the adjacency matrix $A\in\RR^{n\x n}$ of $G$, where
%
$$A_{ij}= [ij\in E] = \begin{cases} 1 & \text{if $ij\in E$}\\ 0 & \text{otherwise}\end{cases}.$$
%
By convention, we shall enumerating the eigenvalues $\theta_1>\cdots >\theta_m$ in decreasing order without repetition for multiplicites.
A letter $\theta$ without a subscript will denote an arbitrary eigenvalue of $G$.

Another matrix associated with a graph is the \emph{Laplacian} $L\in\RR^{n\x n}$.
For regular graphs of degree $\deg(G)$ (in fact, all our graphs are regular), this matrix~is given by $L:=\deg(G)\Id-A$.
We will not use the Laplacian itself, but we will occasionally refer to its eigenvalues $\lambda_i=\deg(G)-\theta_i$. 
The letter $\lambda$ without subscript~shall always denote the corresponding Laplacian eigenvalue to an eigenvaluen $\theta$ of the adjacency matrix.

\begin{definition}
Given a realization $v\:V\to\RR^d$ of $G$.
\begin{myenumerate}
	\item The realization $v$ is called \emph{spectral realization} of $G$ if the arrangement space of $v$ is an eigenspace of $G$.
	\item More specifically, if the arrangement space is the $\theta$-eigenspace $\Eig_\theta(G)$ for eigenvalue~$\theta\in\Spec(G)$, then $v$ is called \emph{$\theta$-realization} of $G$.
	\item If the arrangement space $U\subseteq\RR^n$ of $v$ is just a subspace of the $\theta$-eigenspace $\Eig_G(\theta)$, then $v$ is said to \emph{have eigenvalue $\theta$}.
\end{myenumerate}
\end{definition}

We shall write \emph{the} $\theta$-realization of $G$, and by that, refer to a normalized \mbox{realization} with arrangement space $\Eig_G(\theta)$.
This realization is then unique up to reorientation.
In general we shall assume that our spectral realizations are normalized.


%Note that \enquote{the spectral realization} of $G$ is not a well-defined notion per se, but is only determined up to invertible linear transformations.
%By convention, we assume that it is a \emph{normalized} realization, which now determines it up to reorientation.~This is sufficient to determine all its relevant metric properties.


Note further, that the dimension of a spectral realization cannot be chose freely, but is predetermined by the multiplicity of the chosen eigenvalue.
That is, if~$\theta\in\Spec(G)$ has multiplicity $d$, then the $\theta$-realization is $d$-dimensional


Spectral constructions similar to the ones introduced above are actually a common tool in the visualization of graphs (see, \eg\ \cite{koren2005drawing}).
Since one is unable to control the dimension of the realization, some adjustments to these techniques are neces\-sary.
Especially beautiful is the collection \cite{blueSpectral}, which contain \enquote{spectral drawings} for the edge graphs of all the uniform polytopes to all their eigenvalues.


Now, how is it justified to replace symmetric realizations by spectral realization?
This is because eigenspaces of $G$ are also always invariant subspaces for $\Aut(G)$.

\begin{proposition}\label{res:spectral_implies_symmetric}
A spectral realization of $G$ is a symmetric realization.
%
\begin{proof}
Recall the following property of the adjacency matrix $A$: for all permutations $\phi\in\Sym(V)$ holds
%
$$(*)\quad \phi\in\Aut(G)\;\Longleftrightarrow\; \Pi_\phi A=A\Pi_\phi.$$
%
%$$\Aut(G):=\{\phi\in \Sym(V)\mid \Pi_\phi A=A\Pi_\phi\}.$$

If $u\in\Eig_G(\theta)$ is an eigenvector to an eigenvalue $\theta\in\Spec(G)$, and~\mbox{$\phi\in\Aut(G)$}~is a symmetry of $G$, then follows
%
$$A(\Pi_\phi u) = (A\Pi_\phi) u \overset{\smash{(*)}}= (\Pi_\phi A) u = \Pi_\phi (Au)= \Pi_\phi (\theta u)=\theta(\Pi_\phi u),$$
%
and $\Pi_\phi u\in\Eig_G(\theta)$ as well.
Conclusively, $\Eig_G(\theta)$ is $\Aut(G)$-invariant.

The $\theta$-realization now as an $\Aut(G)$-invariant arrangement space and is spherical (by convention), thus symmetric by \cref{res:symmetric_realizations} $(i)$.
\end{proof}
\end{proposition}

However, the converse is not true.
Not every invariant subspace is an eigenspace, and so not every symmetric realization is a spectral realization.
Not even if we~restrict to irreducible realizations.
Still worse, not even every irreducible symmetric realization has an eigenvalue.
%
It is this deficiency of~\mbox{spectral} realizations \wrt\ symmetric realizations that complicates our treatment of symmetric~\mbox{(eigen-)}polytopes in later sections.

One way to infer the existence of an eigenvalue is by assuming rigidity:

\begin{theorem}\quad

\begin{myenumerate}
	\item 
	An irreducible and rigid $\Sigma$-realization has an eigenvalue.
	
	\item 
	If an irreducible $\Sigma$-realization is flexible, then it can be deformed into at least two balanced realizations.
\end{myenumerate}
\end{theorem}

\begin{proposition}
\label{res:rigid_implies_eigenvalue}
An irreducible and rigid $\Sigma$-realization $v$ has an eigenvalue.
\begin{proof}
Suppose that $v$ does not have an eigenvalue.
Its arrangement space $U\subseteq\RR^n$ is then not contained in any of the eigenspace of $G$.
But since $\RR^n$ is a direct sum of the eigenspaces of $G$, $U$ is then non-orthogonal to some eigenspace.

Since the eigenspaces of $G$ are $\Aut(G)$-invariant, they are also $\Sigma$-invariant, and $v$ is flexible by \cref{res:arrangement_space_rigid}. \msays{BETTER}
\end{proof}
\end{proposition}

%Nevertheless, we shall see later, in \cref{sec:arc_transitive_realizations}, that things look better for certain realizations of arc-transitive graphs (\cf\ \cref{def:transitive}), and even better for distance-transitive graphs (\cf\ \cref{def:distance_transitive}) in \cref{sec:distance_transitive_realizations}.


%However, not all symmetric realizations can necessarily be obtained using spectral realizations: 
%eigenspaces, while $\Aut(G)$-invariant, may not be irreducibly inva\-riant.
%In other words, an irreducible $\Aut(G)$-invariant subspaces, while always~also a subspace of an eigenspace of $G$, may be a \emph{proper} subspace, and is therefore not accessible by spectral constructions only.
%It is this obstruction which complicates our theory of symmetric~\mbox{(eigen-)}polytopes in later sections.

%\begin{proposition}
%An irreducible symmetric realization has an eigenvalue.
%%
%\begin{proof}
%Every irreducible 
%\end{proof}
%\end{proposition}

%We close this section with two observations concerning realizations with eigenvalue.
%
%First, if $v$ has eigenvalue $\theta$, every vector $u\in\RR^n$ with components $u_i=\<v_i,x\>$ for some $x\in\RR^d$ is a $\theta$-eigenvector of $G$ (this follows from \cref{res:vectors}).
%Second, spoken geometrically, each realization with eigenvalue is in a specific balanced~con\-figuration. \msays{give the first observation a number}

%\begin{proposition}\label{res:eigenvalue}
%A realization $v$ has eigenvalue $\theta\in\Spec(G)$ if and only if
%%
%\begin{equation}\label{eq:eigenvalue}
%\sum_{\mathclap{j\in N(i)}} v_j = \theta v_i,\quad\text{for all $i\in V$},
%\end{equation}
%%
%where $N(i):=\{j\in V\mid ij\in E\}$ denotes the set of neighbors of $i\in V$.
%%
%\begin{proof}
%Equation \eqref{eq:eigenvalue} can be equivalently written as
%%
%$$AM = \theta M,$$
%%
%which in turn is equivalent to $U=\Span M\subseteq\Eig_G(\theta)$.
%\end{proof}
%\end{proposition}

\begin{observation}\label{res:eigenvalue}
Let $v\:V\to\RR^d$ be a realization.
%
\begin{myenumerate}
	\item
	$v$ having eigenvalue $\theta\in\Spec(G)$ can be geometrically interpreted as~it~being in a certain balanced configuration. More precisely,
%
\begin{equation}\label{eq:eigenvalue}
\sum_{\mathclap{j\in N(i)}} v_j = \theta v_i,\quad\text{for all $i\in V\!$},
\end{equation}
%
where $N(i):=\{j\in V\mid ij\in E\}$ denotes the set of neighbors of $i\in V$. This is because \eqref{eq:eigenvalue} is equivalent to $AM=\theta M$.

	\item 
	For each $x\in \RR^d$, if $v$ has eigenvalue $\theta$, the vector $u\in\RR^n$ with components $u_i=\<v_i,x\>$ for all $i\in V$ is an eigenvector of $G$ by \cref{res:realizations_and_arrangement_spaces} $(ii)$.
\end{myenumerate}
\end{observation}


$\RR^n$ decomposes into eigenspaces, and each eigenspace decomposes into irreducible $\Sigma$-invariant subspaces.



\begin{proposition}
If $v$ is a $d$-dimensional irreducible and flexible $\Sigma$-realization, then there are~irre\-ducible $d$-dimensional $\Sigma$-realizations $v^{(1)},...,v^{(k)}$ with eigenvalues, so that
%
$$v=v^{(1)}+\cdots+v^{(k)}.$$
%
\begin{proof}
The eigenspaces provide a decomposition
%
$$\RR^n=\Eig_G(\theta_1)\oplus\cdots\oplus\Eig_G(\theta_m)$$
%
into mutually orthogonal $\Sigma$-invariant subspaces of $\RR^n$.
Any in
\end{proof}
\end{proposition}



\begin{lemma}
If a $\Sigma$-realization $v$ is flexible, then this is because it appears as an intermediate realization when deforming a $\Sigma$-realization $w$ with eigenvalue $\theta$ into a $\Sigma$-realization $w'$ with eigenvalue $\theta'$.
%
\begin{proof}
If $v$ itself has an eigenvalue, then this is trivial.

So suppose it has none.
Then its arrangement space $U$ is not contained in any eigenspace of $G$.
But since the eigenspaces of $G$ provide a complete decomposition
%
$$\RR^n=\Eig_G(\theta_1)\oplus\cdots\oplus\Eig_G(\theta_m)$$
%
of $\RR^n$ into mutually orthogonal subspaces, $U$ must be non-orthogonal to at least two of these.
\end{proof}
\end{lemma}

\begin{example}
Every \emph{centered} realization of the complete graph $K_n$ has eigenvalue $-1\in\Spec(K_n)$.
A realization $v\:V\to\RR^d$ is centered if
%
$$\sum_{i\in V} v_i=0,$$
%
which can be achieved by translation.
Since $N(i)=V\setminus\{i\}$ for all $i\in V$, we have
%
$$\sum_{\mathclap{j\in N(i)}} v_j = \underbrace{\sum_{j\in V}v_j}_{=0}-\,v_i=-v_i.$$
%
So $v$ has indeed eigenvalue $\theta=-1$ (\cf\ \cref{res:eigenvalue} $(i)$).
\end{example}

For general graphs however, most realization cannot be just translated to make them have an eigenvalue.

It is the purpose of this paper to investigate how an assumption about symmetry of a realization allows us to infer that it is spectral or has an eigenvalue.
Here is a very simple example.

\begin{example}
Let $G=K_{2,...,2}$ a complete $d$-partite graph (also, the edge-graph of the $d$-dimensional crosspolytope).
Let $\phi\in\Aut(G)$ denote the symmetry of $G$ that exchanges each vertex with its unique non-neighbor. The set $\Sigma:=\{\id,\phi\}\subseteq\Aut(G)$ is a subgroup of the symmetry group of $G$.

If we have a $\Sigma$-realization $v$ of $G$ that expresses $\phi$ in a particular way, then we can conclude that $v$ has an eigenvalue.
For example, if the representation $T$ of $v$ saitsfies $T_\phi=-\Id$, then the realization must have eigenvalue $0$.
If $T_\phi=\Id$, then it must have eigenvalue $-2$. \TODO

We can interpret this in terms of arrangement spaces: \TODO %each $\Sigma$-invariant subspace of $\RR^n$ is completely contained in an eigenspace of $G$.
\end{example}




\fi



\tempnewpage

\section{Edge- and arc-transitive realizations}
\label{sec:arc_transitive}

In this section we explore the properties of edge- and arc-transitive realizations.
Recall that an \emph{arc} in a graph is an incident vertex-edge pair.
The notions of edge- and arc-transitive graphs and realizations are defined parallel to \cref{def:vertex_transitive}.

%Let us first formalize being vertex-, edge- and arc-transitive for groups, graphs and realizations.

%\begin{definition}\label{def:transitive}
%Given a graph $G$ and $\square\in\{\text{vertex},\text{edge},\text{arc}\}$:
%\begin{myenumerate}
%	\item $\Sigma\subseteq\Aut(G)$ is called \emph{$\square$-transitive} if it acts $\square$-transitively on $V$.
%	\item $G$ is called \emph{$\square$-transitive} if $\Aut(G)$ is $\square$-transitive.
%	\item A realization is called \emph{$\square$-transitive} if it is a $\Sigma$-realization for some $\square$-tran\-sitive $\Sigma\subseteq\Aut(G)$.
%\end{myenumerate}
%\end{definition}

%It should be clear how to define an \emph{arc-transitive polytope}.
%Note that in the case of a polytope $P\subset\RR^d$, its (Euclidean) symmetry group $\Aut(P)\subset\Ortho(\RR^d)$ consists of orthogonal matrices, that is, isometries that fix the origin.
%In particular,~the~polytope $P$ is assumed to be centered at the origin.
%
%Our interest in arc-transitive graphs stems from our interest in arc-transitive~polytopes.
%Those in turn are interesting for the following reason: as explained in~\cref{sec:motivation}, we put some hope in \enquote{sufficiently symmetric polytopes} for them to generalize several classic results on reconstruction and rigidity.
%We elaborated that vertex-transitivity is too weak of a restriction to make this work.
%The~next weakest form of symmetry is edge-transitivity.
%
%Surprisingly little is known about the edge-transitive polytopes in general dimension.
%It is known that there are infinitely many edge-transitive polygons, and exactly \emph{nine} edge-transitive polyhedra \cite{grunbaum1987edge}.
%No classification for $d\ge 4$ seems to be in reach.
%However, in \cite{winter2020polytopes} we proved that in dimension $d\ge 4$, any edge-transitive polytope must be vertex-transitive as well.
%Being edge- and \mbox{vertex-transitive~is~only} a tiny step away from being arc-transitive.
%While there are graphs that are vertex- and edge-transitive without being arc-transitive (the so-called \emph{half-transitive} graphs, see \cite{holt1981graph}), the same distinction is not expected to make any difference for convex polytopes.
%
%Conclusively, arc-transitive realizations and polytopes are the next candidates~in line, and as it turns out, they indeed provide the right setting for the desired~exten\-sions.



%\subsection{Arc-transitive realizations}
%\label{sec:arc_transitive_realizations}


%\begin{observation}\label{res:vertex_transitive}
%In a vertex-transitive realization $v$, every vertex can be mapped onto any other vertex by an orthogonal transformation.
%Thus, all vertices must be on a common sphere of radius $r(v)$ around the origin.
%%We say that the realization is \emph{inscribed}.
%If the realization is norma\-lized, equation \eqref{eq:radius} states that for all $i\in V$ holds
%%
%\begin{equation}\label{eq:radius2}
%\|v_i\|^2=[r(v)]^2=\frac dn=\frac{\dim U}n.
%\end{equation}
%\end{observation}

\begin{observation}\label{res:edge_transitive}
If $v$ is edge-transitive, then all edges can be mapped onto each other by orthogonal transformations.
Thus, all edges have the same length,~and~their end vertices have the same inner product.
That is, the following notions are well-defined:
%
$$\omega(v):=\<v_i,v_j\>,\qquad\ell(v):=\|v_i-v_j\|$$
%
for any $ij\in E$.
The latter is called \emph{edge length} of $v$.
\end{observation}


\begin{remark}\label{rem:edge_transitive_rigidity}
Let $v(t)\:[0,1]\to\mathcal R_d(G,\Sigma)$ be a deformation for some edge-transitive $\Sigma\subseteq\Aut(G)$.
Then, the deformation $w(t):=v(t)/\ell(v(t))$ has edge length \mbox{$\ell=1$~for~all} $t\in[0,1]$.

In this sense, a deformation \wrt\ an edge-transitive groups can always be consi\-dered as a flex in the usual sense of rigidity theory, which preserves edge-lengths.
\end{remark}

Under certain conditions, the quantities from \cref{res:edge_transitive} can be computed~ex\-plicitly.

\begin{proposition}\label{res:cosine_and_length}
If $v$ is normalized, vertex- and edge-transitive, and $\theta$-balanced~for some eigenvalue $\theta\in\Spec(G)$ (\resp\ Laplacian eigenvalue $\lambda :=\deg(G)-\theta$, see also \cref{sec:appendix_spec_theory}), then
%
\begin{equation}\label{eq:cosine_and_length}
\omega(v)=\frac{\theta d}{2|E|},\qquad [\ell(v)]^2=\frac{\lambda d}{|E|}.
\end{equation}
%
\begin{proof}
Using equations \eqref{eq:balanced} and \eqref{eq:radius2} we see that for all $ij\in E$ holds
%
$$
\deg(G)\cdot\omega(v)
=\sum_{\mathclap{j\in N(i)}} \<v_i,v_j\>
=\Big\< \!v_i,\sum_{\mathclap{j\in N(i)}} v_j\Big\> \overset{\text{\eqref{eq:balanced}}}= \<v_i,\theta v_i\> 
=\theta \cdot \|v_i\|^2
\overset{\text{\eqref{eq:radius2}}}= \frac{\theta d}n.
$$
%
Expression \eqref{eq:cosine_and_length} for $\omega(v)$ then follows by $\deg(G)\cdot n=2\card E$.
The expression for $\ell(v)$ can now be derived as follows:
%
%$$[\ell(v)]^2 = \|v_i-v_j\|^2 = \|v_i\|^2+\|v_j\|^2-2\<v_i,v_j\> = 2\big( [r(v)]^2-\omega(v)\big).$$
\begin{align*}
[\ell(v)]^2 
&= \|v_i-v_j\|^2 
= \|v_i\|^2+\|v_j\|^2-2\<v_i,v_j\> 
\\&= 2\big( [r(v)]^2-\omega(v)\big)
= 2\Big(\frac dn-\frac{d\theta}{2|E|}\Big) = 2d\Big(\frac{\deg(G)}{2|E|}-\frac\theta{2|E|}\Big)
\\&= \frac{2d(\deg(G)-\theta)}{2|E|} = \frac{\lambda d}{|E|}.
\end{align*}
%
%\vspace{-0.5cm}
%
%Substituting the known values of $r(v)$ and $\omega(v)$ leaves an elementary computation to obtain the claimed result.
\end{proof}
\end{proposition}

If $v$ is spherical instead of normalized, one can still compute the follow\-ing relative 
quantities
%
\begin{equation}\label{eq:relative}
\frac{\omega(v)}{[r(v)]^2} = \frac{\theta}{\deg(G)},\wideand \Big[\frac{\ell(v)}{r(v)}\Big]^2 = \frac{2\lambda}{\deg(G)} = 2\Big(1-\frac\theta{\deg(G)}\Big),
\end{equation}
%
named \emph{cosine} and \emph{relative length} of $v$.
The name \enquote{cosine} is because for $ij\in E$~holds
%
\begin{equation}\label{eq:angle}
\cos \angle(v_i,v_j) = \frac{\<v_i,v_j\>}{\|v_i\|\|v_j\|} = \frac{\omega(v)}{[r(v)]^2} = \frac{\theta}{\deg(G)}.
\end{equation}

We can use these formulas to perform some quick computations on some special poly\-topes.
These are quite laborious if done by hand.

\begin{example}\label{ex:circumradius}
In \cref{ex:dodecahedron}, we have seen that the skeleton of the dodecahedron can be obtained as the $\theta_2$-realization of its edge graph (where $\theta_2=\sqrt 5$).
We can then use \eqref{eq:relative} to compute the circumradius of the dodecahedron with edge length $\ell=1$:
%
$$r(v)= \sqrt{\frac{\deg(G)}{2\lambda_2}} = \sqrt{\frac{3}{2(3-\sqrt{5})}}\approx 1.401258.$$
%
\end{example}

\begin{example}\label{ex:dihedarl_angle}
The \emph{dihedral angle} of a $d$-dimensional polytope $P\subset\RR^d$ at a $(d-2)$-dimensional face $\sigma$ (also called a \emph{ridge} of $P$) is the angle between the two facets incident to $\sigma$, when measured on the inside of the polytope.
In the 3-dimensional case, the ridges are just the edges of $P$.

For example, for the icosahedron (the dual of the dodecahedron), this angle is the same for each edge.
The dihedral angle $\alpha$ of a the icosahedron is exactly $\pi$~minus the angle between incident vertices in its dual. %, that is, the dodecahedron.
The angle between vertices can be computed via \eqref{eq:angle}, and we find:
%
$$\alpha = \pi -\arccos\Big( \frac{\theta_2}{\deg(G)}\Big) = \pi-\arccos\Big(\frac{\sqrt 5}{3}\Big)\;\hat\approx\; 138.1896^\circ.$$

\begin{center}
\includegraphics[width=0.5\textwidth]{img/ico_dode}
\end{center}
\end{example}

The computations in \cref{ex:circumradius} and \cref{ex:dihedarl_angle} work equivalently for all the other regular polytopes as noted in the last paragraph of \cref{ex:dodecahedron}.

%The same trick for computing these geometric quantities via the spectrum of the edge-graph works for other polytopes as long as they ... \TODO

%In both examples we exploited that the skeleton of the dodecahedron is balanced.
%Equivalent calculations work for all regular polytopes (proven in \cite{licata1986surprising} except for the three exceptional 4-dimensional polytopes; this however can be checked by the results of the following section).
%In general however, it is an open question to which polytopes these computations can be applied.
%Also, the relevant eigenvalue seems to be always the second-largest eigenvalue $\theta_2$.
%While this seems plausible (considering results on nodal domains, see \eg\ \cite{...}), no formal reason for this is known.

We have seen that general symmetric realizations are not necessarily spectral, balanced or rigid.
This includes vertex-transitive realizations as we have seen~in~\cref{ex:truncated_tetrahedron}.
We also discussed that vertex-transitivity appears as a plausible minimal require\-ment for obtaining rigidity result (see \cref{res:vertex_transitive_rigid}).
In particular, purely edge-transitive realizations are not expected to be either rigid or balanced.

\begin{example}
The skeleton of the (edge-transitive) \emph{rhombic dodecahedron} (a \emph{Catalan solid}, see the middle image below), is an $\Aut(G)$-realization of its edge-graph.
The image below shown a deformation of this realization (of the form, as constructed in \cref{res:vertex_transitive_rigid}):
%
\begin{center}
\includegraphics[width=0.65\textwidth]{img/rhombic_dodecahedron_rescale}
\end{center}
%
It was also realized by Licata and Powers \cite{licata1986surprising}, that the $\theta_2$-realization of the edge-graph of the rhombic dodecahedron gives exactly its skeleton, rather than any of the infinitely many other deformations.
This is because its skeleton is balanced,~but in contrast to the regular polytopes, this cannot be explained from general symmetry considerations (see \cref{res:full_local_dimension_is_good} and \cref{ex:24_cell}) and appears more accidental.
\end{example}


For the reasons presented before, we from now on also assume vertex-transitivity.
%
While there is a difference between being simultaneously vertex- and edge-transitive and being arc-transitive (the latter is strictly stronger, in between these classes there exist the so-called \emph{half-transitive graphs}, see \cite{bouwer1970vertex, holt1981graph}), in the following we primarily focus on arc-transitive graphs and realizations.

As all the symmetry classes before, also arc-transitive realizations are not necessarily rigid or spectral, though it becomes increasingly more complicated to construct counterexamples.



%We are not going to make this precise.
%Instead we are going to focus on edge-transitive realizations.
%Those are either simultaneously vertex-transitive,~or~they~are not.
%In the latter case, it is known that the underlying graph must be bipartite, and the bipartition classes are the vertex-orbits, of which there are exactly two (see \eg\ \cite{godsil2013algebraic}, Lemma 3.2.1).
%The following example demonstrates that we cannot expect an edge-transitive but not vertex-transitive realization to be rigid or balanced:

%We briefly note that rigidity-questions for edge-transitive realizations are much closer to the usual notions of rigidity theory for frameworks.


%Irreducible edge- and arc-transitive realization are not necessarily spectral, but it seems unknown whether all irreducible edge- and arc-transitive realizations are balanced.
%It would be sufficient to show that they are rigid (by \cref{res:rigid_implies_balanced}), but this turns out to be false:

\iffalse

\begin{example}
\label{ex:edge_transitive_cycle}
%The spectrum of the $n$-cycle $C_n$ consists of eigenvalue of multiplicity one and two.
An irreducible $\Aut(G)$-realization of the $n$-cycle $C_n$ (which is vertex- and edge-transitive) is in fact spectral and rigid (as we shall see later in \cref{sec:distance_transitive}).
However, there are edge-transitive $\Sigma\subseteq\Aut(G)$ that allows for non-balanced irreducible $\Sigma$-realization.
For example, consider the following realizations of the 6-cycle:
%
\begin{center}
\includegraphics[width=0.65\textwidth]{img/non_balanced_with_symmetry_2}
\end{center}
%
By visual inspection, we see that these $\Sigma$-realizations are edge-transitive, and that that they belong to an infinite family of edge-transitive realization. 
Thus, none of them is rigid.

The spectrum of $C_6$ is $\{(-2)^1,(-1)^2,1^2,2^1\}$ (there are at most two balanced realizations of dimension two), and so, like in \cref{ex:truncated_tetrahedron}, we can therefor conclude that infinitely many members of that family of edge-transitive realizations cannot be balanced.
\end{example}

\begin{example}
Let $v\:V\to\RR^d$ be an edge-transitive but not vertex-transitive $\Sigma$-reali\-zation of a graph $G$.
Then $G$ is bipartite with bipartition $V=V_1\cupdot V_2$, and the $V_i$ are simultaneously the vertex-orbits \wrt\ $\Sigma$.

We claim that for all $\alpha_1,\alpha_2\in\RR$ the realization $w\: V\to\RR^d$ with
%
$$w_i:=\begin{cases}\alpha_1 v_i & \text{if $i\in V_1$} \\ \alpha_2 v_i & \text{if $i\in V_2$}\end{cases}$$
%
is also an edge-transitive realization of $G$.
Clearly, a smooth transition in the values of the $\alpha_i$ provides us with a deformation of $v$ that preserves edge-transitivity.

\begin{center}
\includegraphics[width=0.65\textwidth]{img/rhombic_dodecahedron_rescale}
\end{center}
\end{example}

\fi

%\begin{remark}
%That last example is part of a general pattern:
%as soon as $\Sigma\subseteq\Aut(G)$ acts edge-transitively but not vertex-transitively, the graph $G$ must be bipartite, and the bipartition classes are the vertex-orbits of $\Sigma$ (see the white and black dots in the image in \cref{ex:edge_transitive_cycle}).
%These vertex-orbits 
%\end{remark}


\begin{example}\label{ex:K_nn}
Consider the complete bipartite graph $K_{n,n}$ on $2n$ vertices,~which is arc-transitive. %,~that~is $V=$ $\{1,...,n,1',...,n'\}$. 
Its spectrum is $\{(-n)^1,0^{2(n-1)},n^1\}$, and indeed, the 0-eigen\-space~is $\Aut(K_{n,n})$-irreducible.
But there are many arc-transitive subgroups of $\Aut(K_{n,n})$ for which this~eigen\-space decomposes into smaller irreducible subspaces, giving rise to non-spectral arc-transitive realization of $K_{n,n}$.
Many of these are also flexible.
We describe a general procedure to construct such.

Let $v(t)\:[0,1]\to\mathcal R_d(G,\Sigma)$ be proper deformation between irreducible vertex-transitive $\Sigma$-realization of some graph $G$ on the vertex set $V=\{1,...,n\}$ (\eg\ the graph from \cref{ex:truncated_tetrahedron}).
Consider $K_{n,n}$ with vertex set $V_1\cupdot V_2$, where the $V_i$ are disjoint copies of $V$.
Let $\Sigma_i\subseteq \Aut(K_{n,n})$ be an isomorphic copy of $\Sigma$ acting on $V_i$ instead of $V$, and let $\tau\in\Aut(K_{n,n})$ be the involution that exchanges the both partition classes in the obvious way.
Then set $\Sigma':=\<\Sigma_1,\Sigma_2,\tau\>\subseteq\Aut(K_{n,n})$.
Note first, that $\Sigma'$ indeed acts arc-transitively on $K_{n,n}$.
We further claim that the 0-eigenspace of $K_{n,n}$ is \emph{$\Sigma'$-reducible}, and that some irreducible subspace corresponds to a \emph{flexible} arc-transitive realizations.

To see this, consider the following deformation $w(t)\: [0,1]\to\mathcal R_{2d}(K_{n,n},\Sigma')$:
%
$$w_i(t) = \begin{cases} (v_i(t),0) & \text{if $i\in V_1$}\\ (0,v_i(t)) & \text{if $i\in V_2$}\end{cases}.$$
%
Since $v(\free)$ is a proper deformation, so is $w(\free)$.
One checks that for all $t\in[0,1]$ $w(t)$ is indeed an irreducible $\Sigma'$-realization, which, by the existence of the deformation, must be flexible.

% ($\RR^d\times \{0\}$ is $\Sigma_1$-irreducible, $\{0\}\times \RR^d$ is $\Sigma_2$-irreducible, but neither is irreducible \wrt\ $\tau$).
Since $d\ge 2$ and $K_{n,n}$ has only a single non-simple eigenvalue, from \cref{res:eigenvalue_multiplicity_implications} $(i)$ follows that $w(t)$ must be balanced with eigenvalue $0$. 
Since $w(t)$ is flexible, the premise of \cref{res:eigenvalue_multiplicity_implications} $(ii)$ cannot be satisfied.
The multiplicity of the eigenvalue $0$ must therefore be at least $4d$ (twice the dimension of $w(t)$), and so $w(t)$ cannot be spectral, but must only balanced.
\end{example}

The trick in \cref{ex:K_nn} was to choose $\Sigma\subset\Aut(K_{n,n})$ as not the full symmetry group of $K_{n,n}$, but as a proper subgroup.
It is unclear whether this was necessary, that is, whether an $\Aut(G)$-realization of an arc-transitive graph is always rigid (see \cref{q:arc_transitive_balanced}).
An $\Aut(G)$-realization of an arc-transitive graph needs not be spectral though, as we shall see in \cref{ex:C6_C6} further below.
All realizations in \cref{ex:K_nn} are balanced, and it is equally unclear, whether this is the case for all irreducible arc-transitive realizations (see \cref{q:arc_transitive_rigid}).

In the next section, we restrict to a class of arc-transitive realizations for which these questions can be resolved.




%\begin{example}
%Consider the following realizations of the 6-cycle $C_6$:
%%
%\begin{center}
%\includegraphics[width=0.65\textwidth]{img/non_balanced_with_symmetry}
%\end{center}
%%
%The upper row show members of a continuous family of vertex-transitive realization of $C_6$.
%\end{example}
%
%
%It is therefore interesting to ask whether it is sufficient to combine vertex- and edge-transitivity to imply being spectral/balanced.
%No counterexample is known, but no proof either (see Question \cref{q:...}).

%For the upcoming section we shall restrict to arc-transitivity.


%While there is a difference between being simultaneously vertex- and edge-transitive and being arc-transitive (the latter is strictly stronger, in between these classes there exist so-called \emph{half-transitive graphs}, see \cite{holt1981graph}), in the following we restrict to arc-transitive graphs and realizations.

%In \cref{sec:motivation} we gave an example of an irreducible vertex-transitive realization without eigenvalue.
%A respective example with arc-transitivity instead of vertex-transitivity is not known.
%Neither is known whether every irreducible arc-transitive realization has an eigenvalue.

%Ultimately we are interested in arc-transitive polytopes.
%Skeleta of polytope have the convenient property of being full-dimensiona

%While it would be enough to assume rigidity to imply being balanced (see \cref{res:...}), not all arc-transitive, realizations are rigid.

%\begin{example}
%Consider an irreducible but flexible $\Sigma$-realization $v:V\to\RR^d$ for some vertex-transitive $\Sigma\subseteq\Sym(n)$ (on, say, the edge-less graph on $n\ge 3$ vertices, \ie\ basically just a transitive realization of points in $\RR^d$), with representation $T\:\Sigma\to\Ortho(\RR^d)$.
%From this we shall construct an irreducible, flexible and arc-transitive realization of the complete bipartite graph $K_{n,n}$.
%
%Suppose $K_{n,n}$ has bipartition $V_1\cupdot V_2$.
%Fix two bijections $c_i:V\leftrightarrow V_i$.
%Define $\Sigma_i:=\{c_i\circ \sigma\circ c_i^{-1}\mid \sigma\in\Sigma\}\subseteq\Aut(K_{n,n})$, considered as a permutation group on $V_1\cupdot V_2$ that fixes $V_2$ (if $i=1$) \resp\ $V_1$ (if $i=2$).
%%
%Finally, let $s:=c_1\circ c_2^{-1} \in\Aut(K_{n,n})$ be the involution that exchanges $V_1$ and $V_2$ accordingly.
%
%We can now consider the group $\hat\Sigma:=\<\Sigma_1,\Sigma_2,s\>\subseteq\Aut(K_{n,n})$, and one can check that it acts arc-transitively on $K_{n,n}$.
%We now describe an irreducible $\hat\Sigma$-realization $w\:V_1\cupdot V_2\to\RR^{2d}$:
%%
%$$
%w_i := \begin{cases}
%(v_{c_1^{-1}(i)},0) &\text{if $i\in V_1$} \\
%(0,v_{c_2^{-1}(i)}) &\text{if $i\in V_2$}
%\end{cases}.
%$$
%\TODO
%\end{example}

%Note that this example uses a proper subgroup $\Sigma\subset\Aut(K_{n,n})$, as any symmetric realization of $K_{n,n}$ is indeed rigid.
%The question remains whether a symmetric realization of any arc-transitive $G$ (\ie\ realizing all its symmetries) can be flexible.



\subsection{Full local dimension}
\label{sec:full_local_dimension}

In this section we focus on  realizations of \emph{full local dimension}, which means that the edge directions at each vertex span the whole space.
For example, this is always the case for the skeleta of convex polytopes.

\begin{definition}
\label{def:full_local_dimension}
A realization $v$ is said to be of \emph{full local dimension} if 
%
$$\rank\{v_j-v_i\mid j\in N(i)\}=d,\quad\text{for all $i\in V$}.$$
\end{definition}

Being of full local dimensional implies being of full dimension,
but not every~full-dimensional realization is of full local dimension, not even if it is arc-transitive.

\begin{example}\label{ex:not_full_local_dim}
Consider the 4- and 5-dimensional spectral realizations of the edge-graph of the dodecahedron (we have seen in \cref{ex:dodecahedron} that this graph indeed has eigenvalues of multiplicity four and five).
%Thus, they are spherical, and in particular, they are of full dimension (\cref{res:irreducibe_distance_transitive_is_spectral}).
As spectral realizations, they are~arc-transitive.
We will later see (in \cref{res:irreducibe_distance_transitive_is_spectral}) that these realizations are even~irre\-ducible.
However, they cannot be of full \emph{local} dimension since the edge-graph of the dodecahedron is only of degree three.
%An easy way to construct such, is to take an arc-transitive $\Sigma\subset\Aut(G)$ so that for every $i\in V$ the stabilizer of $\{i\}\cup N(i)$ in $\Sigma$ is non-trivial (\eg\ let $G$ be the Petersen graph, and $\Sigma=\Aut(G)$).
%Let $\phi$ be a non-trivial permutation in this stabilizer.
%Then $T_\phi$ fixes $v_i$ as well as all $v_j,j\in N(i)$.
%If $v$ would have full local dimension, this would fix all of $\RR^d$, hence, could not permute the other vertices.
\end{example}

In general, a realization of full local dimension must neither be rigid/balanced (see \cref{ex:truncated_tetrahedron}) nor irreducible (\eg\ the skeleton of a prism).
This is different in the case of arc-transitive realizations.

%For arc-transitive realizations, being of full local dimension has at least three~nice consequences: being irreducible, being rigid, and having an eigenvalue.

\begin{theorem}\label{res:full_local_dimension_is_good}
Let $v$ be an arc-transitive realization of full local dimension. Then
\begin{myenumerate}
	\item $v$ is irreducible,
	%\item $v$ is spherical.
	\item $v$ is rigid, and
	\item $v$ is balanced.
\end{myenumerate}
%
%In particular, $(i)+(ii)$ implies $(iii)$ for arc-transitive realizations.
%
\begin{proof}
Suppose $v$ is a $\Sigma$-realization for some arc-transitive $\Sigma\subseteq\Aut(G)$ and $T\:\Sigma\to\Ortho(\RR^d)$ its representation.

Let $\Sigma_i\subseteq\Sigma$ denote the stabilizer of $\Sigma$ at the vertex $i\in V$.
We want to determine the invariant subspaces of the restriction $T|_{\Sigma_i}\:\Sigma_i\to\Ortho(\RR^d)$.
Clearly, $\Span\{v_i\}$ is invariant, and $T|_{\Sigma_i}$ acts on it by identity (we say, it acts trivially).
In other words, $\Span\{v_i\}\subseteq\Fix(T,\Sigma_i)$ (as defined in \cref{res:fix_rigid}).
We show that we actually have equality.

%Let $\Sigma_i\subseteq\Sigma$ denote the stabilizer of $\Sigma$ at $i\in V$, and consider the set $\Fix(T,\Sigma_i)$ (\cf\ \cref{res:fix_rigid}).
%Clearly, $\Span\{v_i\}\subseteq\Fix(T,\Sigma_i)$, and we shall prove that we have equality.
By arc-transitivity, $T|_{\Sigma_i}$ acts transitively on the set $\mathcal N_i:=\{v_j\mid j\in N(i)\}$.
That is, for any two $w_1,w_2\in \mathcal N_i$ there exists a $\sigma\in\Sigma_i$ with $T_\sigma w_1=w_2$.
And so for any $x\in\Fix(T,\Sigma_i)$ (and by using that $T_\sigma$ is orthogonal) we have
%
$$\<x,w_1\> = \<T_\sigma x,T_\sigma w_1\> = \<x,w_2\> \quad\implies\quad \<x,w_1-w_2\> = 0.$$
%
And since this holds for all $x\in\Fix(T,\Sigma_i)$ and all pairs $w_1,w_2\in\mathcal N_i$, we obtained $\Fix(T,\Sigma_1) \subseteq \aff (\mathcal N_i)^\bot$.~So we found $\Span\{v_i\}\subseteq\Fix(T,\Sigma_i)\subseteq\aff(\mathcal N_i)^\bot$.
But from full local \mbox{dimension follows} $\dim\aff(\mathcal N_i)\ge d-1\implies \dim\aff(\mathcal N_i)^\bot\le 1$.
Thus, the dimensions of the~sub\-spaces in the inclusion chain must agree, and we actually have $\Span\{v_i\}=\Fix(T,\Sigma_i)=\aff(\mathcal N_i)^\bot$.
In particular, we have $\dim\Fix(T,\Sigma_i)=1$ for~all $i\in V$, and so $v$ is rigid by \cref{res:fix_rigid}. This proves $(ii)$.

%There are two immediate consequences.
%First, from $\dim\Fix(T,\Sigma_i)=1$ for all $i\in V$ follows rigidity via \cref{res:fix_rigid}.
%And since
%%
%$$\sum_{\mathclap{j\in N(i)}} v_j \in\Fix(T,\Sigma_i)=\Span\{v_i\}\quad\implies\quad \sum_{\mathclap{j\in N(i)}} v_j=\theta v_i ,$$
%%
%for some $\theta\in\RR$, vertex-transitivity yields that $v$ is balanced (this would have also followed from rigidity as soon as we would have shown irreducibility, see \cref{res:...}, but it can also be seen geometrically as demonstrated above).

To proceed, we show that all $T|_{\Sigma_i}$-invariant subspace, besides $\Span\{v_i\}$, are~contained in the orthogonal complement $v_i^\bot$.
So suppose that $W\not\subseteq v_i^\bot$ is a \mbox{$T|_{\Sigma_i}$-irre}\-ducible subspace, not contained in the orthogonal complement of $v_i$.
In other words, $W$ is non-orthogonal to $\Span\{v_i\}$. 
But if irreducible subspaces are non-orthogonal, then the representation acts isomorphically on them (see \cref{res:non_orthogonal_subspaces}).
So, since $T|_{\Sigma_i}$ acts trivially on $\Span\{v_i\}$, it must act trivially on $W$ too.
But then $W\subseteq\Fix(T,\Sigma_i)=\Span\{v_i\}$.

We can now show that $v$ is irreducible.
For this, suppose that $W\subseteq\RR^d$ is a~$T$-invariant subspace of $\RR^d$.
Such a subspace must also be invariant \wrt\ all the $T|_{\Sigma_i}$, that is, for each $i\in V$ it must either contain $\Span\{v_i\}$, or must be contained in $v_i^\bot$.
Because of vertex-transitivity, if $\Span\{v_i\}\subseteq W$ for some $i\in V$, then for all $i\in V$. 
Since $v$ is full-dimensional, this would give $W=\RR^d$.
Likewise, if $W\subseteq v_i^\bot$ for some $i\in V$, then for all $i\in V$.
Since $v$ is full-dimensional, this would give $W=\{0\}$.
Thus, $W$ is a trivial invariant subspace, and $v$ is irreducible.
This proves $(i)$.

Finally, since $v$ is rigid and irreducible, it follows that $v$ is balanced by \cref{res:rigid_implies_balanced}, which proves $(iii)$.
\end{proof}
\end{theorem}

%This result has some noteworthy consequences.
%In general, reducible realizations can have full local dimension.
%Not so, if we have arc-transitivity.

\begin{corollary}
If an arc-transitive realization is reducible, then it cannot be of full local dimension.
\end{corollary}

In particular, these results apply to the skeleta of arc-transitive polytopes.
We discuss this in the case of regular polytopes:

%Note also that an arc-transitive $\Sigma$-realization of full local dimension is not only irreducible \wrt\ $\Sigma$, but also irreducible \wrt\ to all arc-transitive $\Sigma'\subset\Sigma$.

\begin{example}\label{ex:24_cell}
\Cref{res:full_local_dimension_is_good} now assures us that the skeleta of regular polytopes (actually, of arc-transitive polytopes) are balanced. 
As mentioned in \cref{ex:dodecahedron}, they are actually spectral, which was shown in \cite{licata1986surprising} for all regular polytopes excluding the exceptional 4-dimensional regular polytopes.
We fill in this gap now.

Since we can now apply  \eqref{eq:relative} (which requires being balanced), it remains purely a matter of checking tabulated values for circumradii and edge-lengths of regular polytopes, as well as eigenvalues of their edge-graphs, to find that their skeleta are indeed $\theta_2$-realizations.

We demonstrate this on the example of the 24-cell, whose edge-graph we shall~call $G$.
One of the notable properties of the 24-cell is that the edge length equals~the~cir\-cumradius, or $\ell(v)/r(v)=1$ for its skeleton $v$.
Since $v$ is an arc-transitive realization, \ie~balanced by \cref{res:full_local_dimension_is_good}, we know that \eqref{eq:relative} applies.
We \mbox{can~rearrange} \eqref{eq:relative} for $\theta$ to find
%
\begin{equation}\label{eq:theta_from_metrics}
\theta=\deg(G)\Big(1-\frac12\cdot\Big[\frac{\ell(v)}{r(v)}\Big]^2\Big)=8\cdot\Big(1-\frac12\Big)=4.
\end{equation}
%
Indeed, the spectrum of $G$ is $\{(-8)^1,(-4)^4,0^6,4^4,8^1\}$ with eigenvalue $\theta_2=4$~of~multi\-plicity \emph{four}.
So the skeleton of the 24-cell is spectral with eigenvalue $\theta_2$.

The same technique works verbatim for all other regular polytopes as well.
The table below lists the degree, circumradius and edge-length of the three exceptional 4-dimensional regular polytopes, as well as the second largest eigenvalue $\theta_2$ for their edge-graphs (which have multiplicity four in all cases).
The reader can then check~that these values satisfy an equation analogue to \eqref{eq:theta_from_metrics}, \ie\ the equation produces the second-largest eigenvalue.
%
\begin{center}
\begin{tabular}{l|l|l|l|l}
polytope & $\deg(G)$ & $\ell(v)$ & $r(v)$ & $\theta_2$ \\
\hline
24-cell & \phantom08 & 1 & 1 & 4 \\
120-cell & \phantom04 & $3-\sqrt 5$ & $\sqrt 8$ & $2\phi-1$ \\
600-cell & 12 & $\phi^{-1}$ & $1$ & $2(1+\sqrt 5)$
\end{tabular}
\end{center}
%
Here, $\phi:=(\sqrt 5+1)/2$ denotes the \emph{golden ratio}.
Despite that we can check this on~a case-by-case basis, it remains a mystery why all these skeleta are spectral realizations.
In contrast, for all regular polytopes excluding these 4-dimensional exception, a satisfying answer will be given in the next section, in \cref{ex:regular_licata}.

We shall give a second proof for the 24-cell in \cref{ex:24_cell_cuboctahedron} where we do not~need to know the spectrum of the edge-graph.
\end{example}



%\begin{theorem}
%If an arc-transitive realization $v$ is of full local dimension, then it has an eigenvalue.
%%
%\begin{proof}
%Suppose $v$ is a $\Sigma$-realization for some arc-transitive $\Sigma\subseteq\Aut(G)$ and $T:\Sigma\to\Ortho(\RR^d)$ is its realization.
%Fix a vertex $i\in V$ and let $\Sigma_i:=\{\phi\in \Sigma\mid \phi(i)=i\}$ denote the stabilizer of $\Sigma$ at $i$.
%
%Clearly, $\Span\{v_i\}$ is an invariant subspace of $T(\Sigma_i)$.
%
%\end{proof}
%\end{theorem}

We close this section with an example of an arc-transitive realization of full-local dimension that is \emph{not} spectral, showing that \cref{res:full_local_dimension_is_good} $(iii)$ cannot be improves in general.

\begin{example}\label{ex:C6_C6}
Consider the graph $G:=C_6\times C_6$, best visualized as the edge-graph of the hexagonal torus:
%
\begin{center}
\includegraphics[width=0.4\textwidth]{img/torus}
\end{center}
%
While the torus is not arc-transitive, the graph $G$ is.
Its spectrum is 
%
$$\{(-4)^1,(-3)^4,(-2)^4,(-1)^4,0^{10},1^4,2^4,3^4,4^1\},$$
%
in particular, $G$ has an eigenvalue 0 of multiplicity ten.
The following formula~des\-cribes a 2-dimensional balanced $\Aut(G)$-realization with eigenvalue zero:
%
$$V(C_6)\times V(C_6)\ni(i,j)\;\mapsto\; \begin{pmatrix}
(-1)^i\\
(-1)^j
\end{pmatrix}\in\RR^2.$$
%
This realization is of full local dimension, but it is not spectral, since its dimension is smaller than 10.
\end{example}

%\TODO\msays{Make better, or remove:}
%\begin{remark}
%The rigidity notion of realizations is related to the idea of \emph{perfect polytopes} in polytope theory.
%Intuitively, a polytope is \emph{perfect} if it is the unique most symmetric realization of its combinatorial type.
%For example, the regular polytopes are perfect (they have a unique realization), but the truncated tetrahedron in \cref{ex:truncated_tetrahedron} is not (it has many equally symmetric realizations).
%
%With \cref{res:full_local_dimension_is_good} we can give an criterion for checking for being perfect. If a polytop $P\subset\RR^d$ has an arc-orbit that is
%%
%\begin{myenumerate}
%	\item spanning (\ie\ it contains all vertices), and
%	\item of full local dimension,
%\end{myenumerate}
%%
%then $P$ is perfect.
%While the skeleton of $P$ might not be arc-transitive itself,~it~con\-tains an arc-transitive \enquote{sub-realization}. This is sufficient to imply rigidity~via~\cref{res:full_local_dimension_is_good}, and this translates to $P$ being perfect.
%\end{remark}



\subsection{Summary}

The take away messages of this section are:

\begin{itemize}
\item If an arc-transitive realization is balanced, many metric properties can already be compute from only knowing $G$ and the eigenvalue.
\item Arc-transitive realizations seem to be better behaved than more general~(\eg\ vertex-transitive) realizations, but they still do not have to be rigid or spectral.
\item We do not know whether they have to be balanced.
\item If we assume full local dimension, everything becomes better, and we can now show that the realization is rigid, irreducible and balanced (but not necessarily spectral).
\end{itemize}







\tempnewpage

\section{Distance-transitive realizations}
\label{sec:distance_transitive}

In this final section of the paper we discuss a class of realizations with a particularly high degree of symmetry, called \emph{distance-transitivity}.

Distance-transitive graphs, and their generalizations, the \emph{distance-regular graphs}, %(see \cref{res:...} for a note on their definition), 
form a class of graphs especially accessible by spectral graph theory methods.
The standard literature for these is the monograph by Brouwer, Cohen and Neumaier \cite{brouwer1989distance}.
The generic distance-regular graph has a trivial automorphism group, and thus, those are less relevant to this discussion, and we shall restrict to the \mbox{distance-tran}\-sitive graphs.
Nevertheless, the reader familiar with distance-regular graphs will recognize many of our arguments.

Throughout this section, let $\dist(i,j)$ denote the \emph{distance} between any two vertices $i,j\in V$,~\ie\ the length of the shortest path between $i$ and $j$.
The \emph{diameter} $$\diam(G):=\max_{i,j\in V}\dist(i,j)$$ of $G$ is the maximal distance between any two of its vertices.
%For any $i\in V$ and~$\delta\in$ $\{0,...,\diam(G)\}$, let
%%
%$$N_\delta(i):=\{j\in V\mid\dist(i,j)=\delta\}$$
%%
%denote the $\delta$-th neighborhood of $i$.

%Most conjectures about the spectral properties of arc-transitive realizations can~be actually proven for the following strictly stronger symmetry:

\begin{definition}\label{def:distance_transitive}
A group $\Sigma\subseteq\Aut(G)$ acts \emph{distance-transitively} on $G$ if it acts~transitively on each of the sets
%
$$D_\delta:=\{(i,j)\in V\times V \mid \dist(i,j)=\delta\} ,\quad\text{for each $\delta\in\{0,...,\diam(G)\}$}.$$
%
%where $\dist(i,j)$ denotes the graph-theoretic \emph{distance} between two vertices $i,j\in V$, and $\diam(G)=\max_{i,j\in V}\dist(i,j)$ is called the \emph{diameter} of $G$.
\end{definition}

Distance-transitive graphs and realizations are defined parallel to \cref{def:vertex_transitive}.
%It is clear from this definition how to define distance-transitive graphs and realizations.
Note that being arc-transitive is equivalent to being transitive on the set $D_1$.
Hence, distance-transitivity implies arc-transitivity.


\begin{example}
Complete graphs and cycle graphs are distance-transitive.
More~ge\-ne\-rally, the edge-graphs of the regular polytopes are distance-transitive, with the usual 4-dimensional exceptions. %, the edge-graphs of the 24-cell, 120-cell and 600-cell.
Even stronger, the skeleton of any of these regular polytopes is a distance-transitive realization of the edge-graph (this is easy to check for the simplices and $n$-cubes, and the only two remaining cases are the dodecahedron and the icosahedron, which can be checked by hand).
%
%In fact, we shall see that every regular polytope is distance-transitive, \mbox{excluding} these three exceptions.

Other examples of distance-transitive graphs that are not necessarily edge-graphs are the Petersen-graph and all complete $r$-partite graphs $K_{n,...,n}$.
\end{example}

A very relevant observation concerning distance-transitive symmetry was already made in \cite{brouwer1989distance}:

%Distance-transitive graphs are themselves also a subclass of the so-called \emph{distance-regular graphs} (see \cref{res:...}).
%The standard literature on these is the monograph by Brouwer, Cohen and Neumaier \cite{brouwer2012distance}.
%There, one finds the following result:

\begin{theorem}[\!\cite{brouwer1989distance}, p.\ 137,  Proposition 4.1.11]
\label{res:eigenspaces_eq_irreducible}
For every distance-transitive group $\Sigma\subseteq\Aut(G)$, the $\Sigma$-irreducible subspaces of $\RR^n$ are exactly the eigenspaces of $G$.
\end{theorem}

We highlight again the stark contrast to the arc-transitive case, where eigenspaces are not necessarily irreducible (we were not even able to prove that every irreducible subspace is contained in an eigenspace).
The observation in \cref{res:eigenspaces_eq_irreducible} was also made specifically for the Petersen graph by Du and Fan in \cite{du2013graph}.%, but is actually part of its distance-transitivity.

We shall give a partial proof for \cref{res:eigenspaces_eq_irreducible} in \cref{sec:cosine_vectors}, that is, we will~show that the eigenspaces are irreducible \wrt\ distance-transitive symmetry (see \cref{res:cosine_vectors_are_determined}).
The technique used there (namely, \emph{cosine vectors}) admits a generalization to not necessarily distance-transitive graphs.

%While we use the proof in \cite{brouwer2012distance} as a blackbox for this result in its entirety, we later provide a proof for the fact that all eigenspaces are irreducible using the so-called \emph{cosine vectors} (see \cref{sec:cosine_vectors}).

\Cref{res:eigenspaces_eq_irreducible} in the form of realizations reads as follows:

\begin{theorem}\label{res:irreducibe_distance_transitive_is_spectral}
The spectral realizations of a distance-transitive graphs $G$ are exactly the irreducible distance-transitive realizations of $G$.
\end{theorem}

In other words, all symmetric realizations of a distance-transitive graph can be obtained by spectral methods.
%The full distance-transitive symmetry of such a graph can be explored purely with spectral methods.
We list some further consequences.

\begin{corollary}
\label{res:distance_transitive_consequences}
Given a distance-transitive realization $v$, then
%
\begin{myenumerate}
\item $v$ is rigid,
\item $v$ is an $\Aut(G)$-realization, and
%\item If $v$ is balanced, then $v$ is spectral and irreducible.
\item the following are equivalent: $v$ being balanced, spectral and irreducible.
\end{myenumerate}
%
\begin{proof}
Suppose that $v$ is a $\Sigma$-realization with distance-transitive group $\Sigma\subseteq\Aut(G)$
%, representation $T\:\Sigma\to\Ortho(\RR^d)$ 
and arrangement space $U\subseteq\RR^n$.

Since $G$ has only finitely many eigenspaces, by \cref{res:eigenspaces_eq_irreducible} there are only finitely many $\Sigma$-irreducible subspaces of $\RR^n$. By \cref{res:finitely_many_subspaces}, all $\Sigma$-realizations are rigid. This proves $(i)$.

For $(ii)$, first assume that $v$ is irreducible.
Then $v$ is spectral by \cref{res:irreducibe_distance_transitive_is_spectral}, and~therefore an $\Aut(G)$-realization by \cref{res:spectral_then_symmetric}.
%
%Also, if $v$ would be flexible, then by \cref{res:rigid} $(ii)$ we would find an irreducible $\Sigma$-invariant subspace $\bar U\not= U$ that is non-orthogonal to $U$.
%But all  $\Sigma$-irreducible subspaces of $\RR^n$ must be eigenspaces of $G$ (again by \cref{res:irreducibe_distance_transitive_is_spectral}), including $U$ and $\bar U$, and any two such are orthogonal. Thus, $v$ must be rigid.
%If all irreducible $\Sigma$-realizations are rigid, then all $\Sigma$-realizations are rigid by \cref{res:reducible_rigid}. This proves $(i)$.
%
Now, if $v$ is not irreducible, then we can consider a decomposition of $v$ into~irre\-ducible $\Sigma$-realizations $v^{(1)},...,v^{(k)}$ as in \cref{rem:irreducible_decomposition} (we assume that $v$ is appropriately oriented). 
Each of these irreducible constituents is now an $\Aut(G)$-realization of $G$ with an irreducible $\Aut(G)$-representation $$T^{(k)}\:\Aut(G)\to\Ortho(\RR^{d_k}).$$
From this we construct an $\Aut(G)$-representation $T\:\Aut(G)$ $\to\Ortho(\RR^d)$ for $v$ as in \eqref{eq:representation_decomposition}. Thus, $v$ is an $\Aut(G)$-realization, proving $(ii)$.

%Now suppose that $v$ is flexible. Then $v$ can be deformed into a non-equivalent $\Sigma$-realization $v'$ with arrangement space $U'\not= U$.
%Both $U$ and $U'$ are direct sums of irreducible subspaces, that is, eigenspaces of $G$.
%If they are not identical, then they consist of distinct eigenspaces.

%Let $U'':=U\cap U'$ and defined $W:= (U'')^\bot \cap U$ and $W':= (U'')^\bot \cap U'$.
%Note that $U'',W$ and $W'$ are all $\Sigma$-invariant, and that $W$ and $W'$ have trivial intersection. Then $W(t):= (U'')^\bot\cap U(t)$ defines a \enquote{continuous transition} between $W$ and $W'$, and thus a deformation between corresponding $\Sigma$-realizations $w$ and $w'$.
%However, these are ...


%Now suppose that $v$ is flexible.
%Then there is a deformation $v(t)\:[0,1]\to\mathcal R_d(G,\Sigma)$ from $v$ into some non-equivalent $\Sigma$-realization $w$.
%We can assume that the representation $T:=T(t)$ of $v(t)$ stays constant during the deformation.
%Let $W\subseteq \RR^d$ be a $T$-irreducible subspace of $\RR^d$, and let $v'(t)$ be the orthogonal projection of $v(t)$ onto $U$.
%Then $v'(0)$ and $v'(1)$ correspond to an irreducible constituent of $v$ and $w$ respectively, and $v'(t)$ is a deformation between these.
%But these constituents are distance-transitive $\Sigma$-realizations, hence rigid (as we have seen before) and thus $v'(0)=v'(1)$.
%Since this holds for all $T$-invariant subspaces $W\subseteq\RR^d$, we have $v=w$.
%This is a contradiction to the assumption that $v$ and $w$ are non-equivalent, and so $v$ must be rigid.

%The rigidity of $v$ follows from the irreducible case via \cref{res:reducible_rigid}. This proves $(i)$.


Finally, we prove $(iii)$.
Being spectral and being irreducible are equivalent by \cref{res:irreducibe_distance_transitive_is_spectral}. 
Also spectral implies balanced, and so we only have to prove the converse: if $v$ is balanced, then $U\subseteq\Eig_G(\theta)$ for some eigenvalue $\theta\in \Spec(G)$. Now $U$ contains at least one irreducible subspace, but $\Eig_G(\theta)$ already is irreducible. Thus $U=\Eig_G(\theta)$, $v$ is spectral, and we proved $(iii)$.
%
%
%
%\TODO
%
%
%Suppose that $v$ is a $\Sigma$-realization with distance-transitive $\Sigma\subseteq\Aut(G)$ and arrangement space $U\subseteq\RR^n$.
%
%Suppose that $v$ is irreducible, then $U$ is an irreducible $\Sigma$-invariant subspace of $\RR^n$, hence an eigenspace of $G$ by \cref{res:eigenspaces_eq_irreducible}.
%Thus $v$ is a spectral realization and, in particular, an $\Aut(G)$-realization by \cref{res:spectral_then_symmetric}, which proves $(ii)$ in the irreducible case.
%If $v$ would be flexible, then there would exist a $\Sigma$-irreducible subspace $\bar U\subseteq\RR^n$ non-orthogonal to $U$ by \cref{res:non_orthogonal_deformation}.
%But by \cref{res:eigenspaces_eq_irreducible}, $\bar U$ must be an eigenspace, and since the eigenspaces are mutually orthogonal, we have $U\perp \bar U$ and $v$ is rigid.
%This proves $(i)$ in the irreducible case.
%
%Both results $(i)$ and $(ii)$ carry naturally over to the reducible case.
%
%Now, if $v$ is balanced, then $U\subseteq\Eig_G(\theta)$ for some $\theta\in\Spec(G)$. $U$ contains at least one $\Sigma$-irreducible subspace, but since $\Eig_G(\theta)$ is already irreducible, we find $U=\Eig_G(\theta)$ and $(iii)$ follows.
\end{proof}
\end{corollary}

%\begin{corollary}
%Every balanced distance-transitive realization is spectral.
%\end{corollary}
%
%\begin{corollary}
%Every distance-transitive realization is rigid.
%%
%\begin{proof}
%It suffices to show this for irreducible realization.
%
%If there are non-equivalent two distance-transitive realizations $v^0,v^1:V\to\RR^d$ that can be deformed into each other, then also their arrangement spaces must transition into each other.
%But both have as arrangement space a complete eigenspace of $G$, and any \enquote{intermediate space} cannot be an eigenspace, and the intermediate realization cannot be distance-transitive.
%
%\end{proof}
%\end{corollary}

Note especially part $(ii)$ which can be informally stated as follows:
the distance-transitive symmetries of $G$ cannot be geometrically separated from the other symmetries of $G$.
As soon as one tries to realize the distance-transitive symmetry of $G$, one automatically realizes all symmetries of $G$.
%\begin{proof}
%The arrangement space $U\subseteq\RR^n$ of a distance-transitive $\Sigma$-realization $v$ is $\Sigma$-invariant.
%Hence, $U$ is the direct sum of irreducible $\Sigma$-invariant subspaces of $\RR^n$.
%Each of these irreducible subspaces is an eigenspaces of $G$, thus $\Aut(G)$-invariant.
%Therefore, also $U$ is $\Aut(G)$-invariant and $v$ is an $\Aut(G)$-realization.
%\end{proof}
%\end{corollary}

This is remarkable, as we have already encountered vertex-, edge- and even arc-transitive realizations that are not $\Aut(G)$-realizations, that is, they still leave some symmetries unrealized.
%
It appears as if distance-transitivity lies beyond a threshold, from which on symmetries can no longer be distinguished geometrically.

\begin{remark}\label{ex:regular_licata}
Licata and Powers \cite{licata1986surprising} have proven their result about regular polytopes (discussed in \cref{ex:dodecahedron} and \cref{ex:24_cell}) by explicit computation.

We can now obtain their result as follows: the skeleton of a regular polytope (not a 4-dimensional exception) is distance-transitive (in particular, arc-transitive) and of full local dimension, thus irreducible by \cref{res:full_local_dimension_is_good}. But if it is irreducible and distance-transitive, then~it must be spectral by \cref{res:irreducibe_distance_transitive_is_spectral}.
\end{remark}


\subsection{Cosine vector and cosine sequence}
\label{sec:cosine_vectors}

The remainder of this section is devoted to an idea that can be used to prove a part of \cref{res:irreducibe_distance_transitive_is_spectral}, but which also admits some interesting generalizations.

\begin{definition}
For a vertex-transitive realization $v$ and some vertex $i\in V$, the \emph{cosine vector} $u\in\RR^n$ of $v$ is the vector with components $u_j:=\<v_i,v_j\>$ for all $j\in V$.
\end{definition}

Vertex-transitivity ensures that this definition of the cosine vector is independent of our choice of $i\in V$ up to some coordinate permutation. We can therefore~assume that $u_i:=\<v_1,v_i\>$.
Recall further, that the cosine vector is contained in the arrangement space of $v$ as seen in  \cref{res:eigenvectors_from_realization}.

The central idea concerning the consine vector is explained in the following observation:

\begin{observation}\label{res:cosine_vectors}
Suppose that we are given a $\theta$-balanced $\Sigma$-realization $v$ and we want to know whether $v$ is spectral.
This is easy if we know the multiplicity of $\theta$, so suppose that we do not.

Let $U\subseteq\RR^n$ be the arrangement space of $v$.
If $v$ were not spectral, then we find that the subspace $\bar U:=U^\bot\cap\Eig_G(\theta)$ is non-zero and $\Sigma$-invariant.
The corresponding realization $\bar v$ with arrangement spaces $\bar U$ is then also a $\theta$-balanced $\Sigma$-realization.
If $u,\bar u\in\RR^n$ are the consine vectors of $v$ and $\bar v$ respectively, then $\<u,\bar u\>=0$ because they are contained in the orthogonal subspaces $U$ and $\bar U$.

%then the $\theta$-eigenspace decomposes as $\Eig_G(\theta)=U\oplus U'$ into orthogonal $\Sigma$-invariant subspaces $U,U'\subseteq\RR^n$, where $U$ is the arrangement space of $v$.
%The other subspace $U'$ gives rise to a second balanced $\Sigma$-realization $v'$.
%Let $u,u'\in\RR^n$ be the cosine vectors of $v$ and $v'$ respectively.
%Since they are contained in orthogonal subspaces, we have $\<u,u'\>=0$.

The idea is to show that, in the right setting, being balanced $\Sigma$-realizations to the same eigenvalue is already so restrictive, that the corresponding cosine vectors have no chance to be orthogonal.
If this is the case, then we found that $\Eig_G(\theta)$ is $\Sigma$-irreducible and $v$ is the $\theta$-realization.
\end{observation}

This idea most directly applies to distance-transitive realizations.
For these, one shows that the cosine vector depends only on $G$ and $\theta$ (\cref{res:cosine_vectors_are_determined}). %, hence is the same for all distance-transitive realizations.

\begin{observation}
If $v$ is distance-transitive, then the value of $u_i=\<v_1,v_i\>$ depends only on $\delta:=\dist(1,i)$.
One therefore groups all entries with the same distance to $1\in V$ and writes $u_\delta$ for all $\delta\in\{0,...,\diam(G)\}$.
The sequence $u_0,...,u_{\diam(G)}$ is called \emph{cosine sequence} of $v$.
\end{observation}

Clearly the cosine sequence and cosine vector of a distance-transitive realization determine each other. We show the following:

%This technique works perfectly well in the context of distance-transitive realization, as we shall demonstrate now.
%More precisely, we show that the cosine vector of any distance-transitive realization is completely determined by the graph $G$ and the chosen eigenvalue.
%Two distance-transitive realizations to the same eigenvalue can then impossibly have orthogonal cosine vectors (except if they are zero, a case we can ignore).

\begin{lemma}\label{res:cosine_vectors_are_determined}
\label{res:cosine_vector_of_distance_transitive_realization}
The cosine sequence of a $\theta$-balanced distance-transitive realization (of radius $r(v)=1$) does only depend on $G$ and the eigenvalue $\theta$.
%
\begin{proof}
Let $N_\delta(i):=\{j\in V\mid\dist(i,j)=\delta\}$ denote the set of all vertices at distance $\delta$ from $i$.
In a distance-transitive graph, the cardinality of the intersection $N_{\delta_1}(i)\cap N_{\delta_2}(j)$ does only depend on $\delta_1,\delta_2$ and $\dist(i,j)$.
The following parameters are therefore well-defined:
%
%\begin{equation}
$$
c_\delta := |\underbrace{N_{\delta-1}(i)\cap N_1(j)}_{=:N_c}|,\quad 
a_\delta := |\underbrace{N_\delta(i)\cap N_1(j)}_{=:N_a}|,\quad 
b_\delta := |\underbrace{N_{\delta+1}(i)\cap N_1(j)}_{=:N_b}|,
$$
%\end{equation}
%
whenever $\dist(i,j)=\delta$\footnote{The order of the parameter names $a$, $b$ and $c$ might appear counter intuitive, but is standard in the~litera\-ture (these parameters are used to define distance-regular graphs), and so we shall adopt it here. %Furthermore, a \emph{distance-regular} graph is defined exactly by the existence of these parameters, \ie\ by the fact that the cardinality of these intersections depends only on $\dist(i,j)$
}.
The list of the parameters $a_\delta,b_\delta$ and $c_\delta$ is called the~\emph{inter\-section array} of $G$.
Note that $N(j)=N_a\cupdot N_b\cupdot N_c$.

Now suppose that $v$ is a balanced distance-transitive realization with eigenvalue $\theta\in \Spec(G)$ and cosine sequence $u_\delta$. 
Then for all $\delta\in\{0,...,\diam(G)\}$ there is an $i\in N_\delta(1)$, and from that we derive
%
\vspace{-0.5em}
\begin{align*}
\theta u_\delta 
=  \<v_1,\theta v_i\> 
\overset{\eqref{eq:balanced}} = \Big\< v_1, \sum_{\mathclap{j\in N(i)}} v_j\Big\> 
&= 
\sum_{\mathclap{j\in N_c}} \overbrace{\overset{\phantom.}\<v_1,v_j\>}^{u_{\delta-1}}+
\sum_{\mathclap{j\in N_a}} \overbrace{\overset{\phantom.}\<v_1,v_j\>}^{u_{\delta}}+
\sum_{\mathclap{j\in N_b}} \overbrace{\overset{\phantom.}\<v_1,v_j\>}^{u_{\delta+1}}
\\ &= c_\delta u_{\delta-1} + a_\delta u_\delta + b_\delta u_{\delta+1}.
\end{align*}
%
Rearranging for $u_{\delta+1}$ yields a three term recurrence for the components of the cosine sequence that only involves $\theta$ and the intersection array:
%
\begin{equation}
\label{eq:recurrence}
u_{\delta+1} = \frac1{b_\delta}\big((\theta-a_\delta)u_\delta-c_\delta u_{\delta-1}\big).
\end{equation}
%
We assume that $r(v)=1$, and since $v$ is also arc-transitive we have initial conditions:
%
$$u_0=[r(v)]^2 = 1,
\qquad 
u_1=\omega(v)\overset{\eqref{eq:relative}}=\frac{\theta}{\deg(G)}.$$
%
The initial conditions only depends on $\theta$ and $G$, and so the whole cosine sequence does only depend on $\theta$ and $G$ (its degree, and intersection array).
%
\end{proof}
\end{lemma}

\Cref{res:cosine_vectors_are_determined} together with \cref{res:cosine_vectors} shows that all eigenspaces of a distance-transitive graph are $\Sigma$-irreducible for all distance-transitive $\Sigma\subseteq\Aut(G)$.

We close with an example that demonstrates the potential of the cosine vector approach by applying it outside the realm of distance-transitive realizations.
%The next example shows how this cosine vector technique extends beyond the distance-transitive realizations.


\begin{example}\label{ex:24_cell_cuboctahedron}
We show that the skeleton of the 24-cell is a spectral realization without computing its spectrum (as we have done in \cref{ex:24_cell}).
Note that the 24-cell is arc-transitive, but not distance-transitive, and that its skeleton is balanced by \cref{res:full_local_dimension_is_good}. % because $D_2$ consists of two orbits \wrt\ $\Aut(G)$ (all other $D_\delta$ are a single orbit).

The coordinates of the vertices of the 24-cell are all coordinate permutations and sign selections of
%
$$\sqrt2\cdot (\pm 1,0,0,0)\wideand \sqrt2\cdot (\pm1/2,\pm1/2,\pm1/2,\pm1/2).$$%
%
From this we find that the cosine vector is $u=(2^1,1^8,0^6,(-1)^8,(-2)^1)$ (ignoring the exact ordering of the entries, only caring about the multiplicities).
%The following table shows to which orbit each of these numbers belongs to:
%
%\begin{center}
%\begin{tabular}{c|c|c}
%$\<v_1,v_i\>$ &  $\dist(1,i)$ & \# \\ 
%\hline
%$\phantom+\overset{\phantom.}2$ & 0 & 1 \\
%$\phantom+1$ & 1 & 8 \\
%$\phantom+0$ & 2 & 6 \\
%$-1$ & 2 & 8 \\
%$-2$ & 3 & 1 \\
%\end{tabular}
%\end{center}

Note that the single entry of value 2 in the cosine vector belongs to the radius $r(v)=\sqrt 2$ of this realization. Also, the eight entries with value $\<v_1,v_i\>=1$ belong to the neighbors $i\in N(1)$, and so this value is determined by \eqref{eq:relative}.
In conclusion, any other balanced arc-transitive realization $\bar v$ to the same eigenvalue (and of the same radius) must have a cosine vector of the form
%
$$\bar u=(2^1,1^8;x_1,...,x_6;y_1,...,y_8;z),$$
%
where the $x_i$ match up with the 0-entries in $u$, the $y_i$ match up with the $-1$-entries in $u$, and $z$ matches with the $-2$-entry.

%Suppose that there is another balanced arc-transitive realization $v'$ of $G$ to the same eigenvalue and with cosine vector $u'\in\RR^n$. 
%We can assume that $v'$ has the same radius as the 24-cell, so that $u'_1=u_1 = 2$.
%By \eqref{eq:relative} we also have $u_i'=u_i=1$ for all $i\in N(1)$.
%%Thus $u'=(2,1,...,1,x_1,...,x_6,y_1,...,y_8,z)$, where the assignment of the components is as shown in the table below:
%Thus we can assume that $u'$ has components as shown in the table below:
%%
%\begin{center}
%\begin{tabular}{l||c|c|c|c|c}
%$u^{\phantom\prime}$ & $2$ & $1,...,1$ & $0,...,0$ & $-1,...,-1$ & $-2$ \\
%\hline
%$\overset{\phantom.}{u'}$ & $2$ & $1,...,1$ & $x_1,...,x_6$ & $\phantom+y_1,...,y_8$ & $\phantom+z$
%\end{tabular}
%\end{center}
%
As discussed in \cref{res:cosine_vectors}, we can assume $\<u,\bar u\>=0$, which expands to
%
$$(*)\quad 0=\<u,\bar u\> = 4 + 8  - y_1-\cdots -y_8 - 2z.$$
%
A (full-dimensional) arc-transitive realization is always centered at the origin, which means $v_1+\cdots +v_n=0$, or in terms of the cosine vector
%
$$(**)\quad 0=\sum_{i\in V} \bar u_i = 2+8 + x_1+\cdots + x_6 + y_1+\cdots +y_8 + z $$
%
We can add $(*)$ and $(**)$ to obtain $z=22+x_1+\cdots+ x_6$.

Finally, every component $\bar u_i=\<\bar v_1,\bar v_i\>$ of the cosine vectors must satisfy $-2=\<\bar v_1,-\bar v_1\>\le \< \bar v_1,\bar v_i\> \le \<\bar v_1,\bar v_1\>=2$, thus $x_i,z\in[-2,2]$.
But this is incompatible with $z=22+x_1+\cdots+ x_6$.
%
%So any other balanced arc-transitive realization of $G$ to the same eigenvalue must have a cosine vector of the form $u'=(2^1,1^8,x^6,y^8,z^1)$ (after an appropriate rescaling).
%The first two entries must agree, because these follow from arc-transitivity.
%Also, the other entries are grouped according to the orbits of $D_\delta$.
%Now, if $u$ and $u'$ were orthogonal, then
%%
%$$(*)\quad 0=\<u,u'\>=4+8\cdot 1 + 0\cdot x-8\cdot y-2z = 12-8y-2z.$$
%%
%Note further, that each (full-dimensional) arc-transitive realization must be centered, \ie\
%%
%$$(**)\quad 0=\sum_{i\in V} u'_i = 2+8\cdot 1+6\cdot x+8\cdot y+z = 10+6x+8y+z.$$
%%
%If we add $(*)$ and $(**)$, we get $22+6x-z=0\implies z=6x+22$.
%Finally, observe that $
%x,z\in[-2,2]$, which is not compatible with $z=6x+22$.
Thus, no second such realization can exist, and the skeleton of the 24-cell is a spectral realization.

Note that we essentially used the shape of the cosine vector of the 24-cell.
The same argument works essentially unchanged \eg\ for the skeleton of the cuboctahedron (also arc-transitive) whose cosine vector is $(2^1,1^4,0^2,(-1)^4,(-2)^1)$,

\vspace{0.5em}
\begin{center}
\includegraphics[width=0.2\textwidth]{img/cuboctahedron}
\end{center}
\end{example}






%We have previously seen that the cosine vector is contained in the arrangement space of $v$.
%
%Now suppose we have two irreducible $\Sigma$-realizations $v,v'$ of the same graph.
%Let $u,u'\in\RR^n$ denote their cosine vectors.
%If $\<u,u'\>\not=0$, then the arrangement spaces cannot be orthogonal either, and by \cref{res:...}, $v$ can be deformed into $v'$.
%
%Now suppose that $v$ is balanced to the eigenvalue $\theta\in\Spec(G)$.
%We ask whether the $\theta$-eigenspace of $G$ is $\Sigma$-irreducible.
%If it is not, then we can write $\Eig_G(\theta)=U\oplus U'$ with orthogonal $\Sigma$-invariant subspaces $U,U'\subseteq\RR^n$, where $U$ is the arrangement space of $v$.
%The subspace $U'$ gives rise to another $\Sigma$-realization $v'$ with cosine vector $u'$.
%We then have $\<u,u'\>=0$.
%In other words, if we can show that no other cosine vector can be perpendicular to $u$, then $\Eig_G(\theta)$ must be $\Sigma$-irreducible.






\iffalse

\newpage

\section{Distance-transitive realizations}
\label{sec:distance_transitive}

We have seen that balanced arc-transitive realizations are not necessarily spectral, and we needed full local dimension to show rigidity.
Some of the assumptions can be weakened when we consider distance-transitivity instead of arc-transitivity.


%One of the major difficulties with arc-transitive realizations is, that they are not necessarily spectral realizations, not even if they have an eigenvalue.
%This~is~caused~by eigenspaces of  $G$ that are not necessarily irreducible invariant \wrt\ some~\mbox{arc-tran}\-sitive group of symmetries.


%The major difficulty in the previous sections was that an arc-transitive realization (even if it has an eigenvalue) might not be a spectral realization.
%This~is~caused~by eigenspaces of  $G$ that are not necessarily irreducible invariant \wrt\ some~\mbox{arc-tran}\-sitive group of symmetries.

In this section we shall discuss a stronger form of symmetry, \emph{distance-transitivity}, about which much stronger statements can be made.

\subsection{Distance-transitive graphs}
\label{sec:distance_transitive_graphs}

%The statements of \Cref{conj:arc_transitve} can actually be proven in a more restrictive context, which still yields many interesting polytopes.

For this section, let $\dist(i,j)$ denote the \emph{graph-theortical distance} of two vertices $i,j\in V$.
The \emph{diameter} $$\diam(G):=\max_{i,j\in V}\dist(i,j)$$ of $G$ is the maximal distance between any two of its vertices.
For any $i\in V$ and~$\delta\in$ $\{0,...,\diam(G)\}$, let
%
$$N_\delta(i):=\{j\in V\mid\dist(i,j)=\delta\}$$
%
denote the $\delta$-th neighborhood of $i$.

%Most conjectures about the spectral properties of arc-transitive realizations can~be actually proven for the following strictly stronger symmetry:

\begin{definition}\label{def:distance_transitive}
A group $\Sigma\subseteq\Aut(G)$ acts \emph{distance-transitively} on $G$ if it acts~transitively on the vertex-pairs in all of the sets
%
$$D_\delta:=\{(i,j)\in V\times V \mid \dist(i,j)=\delta\} ,\quad\text{for each $\delta\in\{0,...,\diam(G)\}$}.$$
%
%where $\dist(i,j)$ denotes the graph-theoretic \emph{distance} between two vertices $i,j\in V$, and $\diam(G)=\max_{i,j\in V}\dist(i,j)$ is called the \emph{diameter} of $G$.
\end{definition}

It is easily seen that distance-transitivity implies arc-transitivity.
%
The notions of distance-transitive graph and realization are defined accordingly.
%Note that in the definition of a distance-transitive polytope, the distance between vertices is still meant in the graph-theoretic sense along the edge-graph, rather than via the Euclidean distance.

%\begin{example}
%Examples for distance-transitive graphs are: complete graphs, cycle graphs, the Petersen graph, ...
%\end{example}

\begin{example}
Complete graphs and cycle graphs are distance-transitive.
More~ge\-ne\-rally, the edge-graph of almost every regular polytope is distance-transitive (the only exceptions are the edge-graphs of the 24-cell, 120-cell and 600-cell).
%
%In fact, we shall see that every regular polytope is distance-transitive, \mbox{excluding} these three exceptions.
\end{example}

%Distance-transitive graphs admit a generalization to the so-called \emph{distance-regular} graphs that share all their spectral properties, but usually have a small symmetry group (generically, one even has $\Aut(G)=\{\id\}$).
%But since our main focus lies in deriving spectral properties from the \emph{symmetry} of a realization, we are less interested in this generalization.


\begin{observation}
It follows from distance-transitivity that for any two vertices~$i,j\in$ $V$ and distances $\delta_i,\delta_j\in\{0,...,\diam(G)\}$ the cardinality of the set
%
$$N_{\delta_i}(i)\cap N_{\delta_j}(j)$$
%
only depends on $\dist(i,j)$.
The following parameters are therefore well-defined:
%
%\begin{equation}
$$
c_\delta := |N_{\delta-1}(i)\cap N_1(j)|,\quad 
a_\delta := |N_\delta(i)\cap N_1(j)|,\quad 
b_\delta := |N_{\delta+1}(i)\cap N_1(j)|,
$$
%\end{equation}
%
whenever $\dist(i,j)=\delta$ (the order of the parameter names appears counter intuitive, but is standard in the \mbox{literature}, so we shall adopt it).

The collection of these parameters is called the \emph{intersection array} of $G$, and~many properties of the graph, including its spectral properties, are already determined by this array.
It was therefore found interesting to study graphs which are solely defined by the existence of the intersection array.
These so-called \emph{distance-regular} graphs are a well-studied generalization of distance-transitive graphs.

The generic distance-regular graph has few, or even no symmetries, and thus, this generalization is of less interest for us.
Still, the reader familiar with this graph class will recognize some of the arguments below.
\end{observation}

%Th spectral properties of $G$ are completely determined by 
%
%Many relevant properties of $G$, especially many spectral properties, can be infer\-red from only knowing the parameters $a_\delta,b_\delta$ and $c_\delta$.
%In fact, there exists a generalization of distance-transitive graphs, the so-called \emph{distance-regular} graphs, which are defined solely by the existence of these parameters.
%In this context, the collection of these parameters is called the \emph{intersection array} of $G$.
%
%There exists a huge literature concerning distance-regular graphs, and the reader familiar with these will recognize some of the intermediate results below.
%However, the usual distance-regular graphs has a small symmetry group (generically, one even finds $\Aut(G)=\{\id\}$).
%Since we are interested in deducing spectral properties from geometric symmetries, this generalization is less relevant for us.


\subsection{Distance-transitive realizations}
\label{sec:distance_transitive_realizations}

\begin{observation}
For a distance-transitive realization $v$ and vertex $i\in V$ thereof, let $u\in\RR^n$ be the vector with components $u_j:=\<v_i,v_j\>$ for all $j\in V$.
This vector is contained in the arrangement space of $G$ (see equation \eqref{eq:eigenvector}).
Because a distance-transitive graph is vertex-transitive, this vector does not depend on the choice of $i\in V$.
We call this vector the \emph{cosine vector} of $v$.

Again, by distance-transitivity, the component $u_j=\<v_i,v_j\>$ does actually only depend on $\dist(i,j)$.
For this reason, we can also write $u_\delta$ for the value of every component $u_j$ with $\dist(i,j)=\delta$.
The sequence $\{u_0,u_1,...,u_{\diam(G)}\}$ is known as the \emph{cosine sequence} of $v$.
\end{observation}

The following is a key observation: for distance-transitive realizations of $G$ with eigenvalue $\theta$, the cosine sequences (and thus, also the cosine vectors) depend only on $\theta$ and the intersection array of $G$, but not on the specific realization.

\begin{theorem}\label{res:distance_transitive_eigenvalue_implies_spectral}
If a distance-transitive realization $v$ has an eigenvalue $\theta$, then
\begin{myenumerate}
	\item $v$ is irreducible, and
	\item $v$ is the $\theta$-realization of $G$.
\end{myenumerate}
\end{theorem}

The idea of the proof is to show that the cosine vector of $v$ does only depend (up to scale) on $\theta$ and the intersection array of $G$, but not on the exact distance-transitive realization.
So any two distance-transitive realizations with the same eigenvalue have arrangement spaces with non-trivial intersection, which is not possible if both are irreducible.

\begin{proof}[Proof of \cref{res:distance_transitive_eigenvalue_implies_spectral}]
Let $v$ be any distance-transitive realization of $G$ with eigenvalue $\theta$.
We can assume that $v$ is normalized, as $(i)$ and $(ii)$ are independent of this fact.
The proof proceeds in three steps.
%We show that the consine sequence $u_\delta$ is already uniquely determined by $\theta$ and independent of $v$.

\emph{Step 1}:
Fix $i,j\in V$ with $\delta:=\dist(i,j)$. Then $N(j)$ decomposes as follows:
%
$$N(j)=
\underbrace{\big(N_{\delta-1}(i)\cap N(j)\big)}_{=:\,W_c} \cupdot
\underbrace{\big(N_{\delta}(i)\cap N(j)\big)}_{=:\,W_a} \cupdot
\underbrace{\big(N_{\delta+1}(i)\cap N(j)\big)}_{=:\,W_b}.
$$
%
Since $v$ has eigenvalue $\theta$, we have
%
\begin{align*}
\theta u_\delta 
=  \<v_i,\theta v_j\> 
\overset{\eqref{eq:eigenvalue}} = \Big\< v_i, \sum_{\mathclap{k\in N(j)}} v_k\Big\> 
&= 
\sum_{\mathclap{k\in W_c}} \<v_i,v_k\>+
\sum_{\mathclap{k\in W_a}} \<v_i,v_k\>+
\sum_{\mathclap{k\in W_b}} \<v_i,v_k\>
\\ &= c_\delta u_{\delta-1} + a_\delta u_\delta + b_\delta u_{\delta+1}.
\end{align*}
%
Rearranging for $u_{\delta+1}$ yields a three term recurrence for the components of the cosine sequence that only involves $\theta$ and the intersection array:
%
\begin{equation}
\label{eq:recurrence}
u_{\delta+1} = \frac1{b_\delta}\big((\theta-a_\delta)u_\delta-c_\delta u_{\delta-1}\big).
\end{equation}
%
Moreover, we have initial conditions (assuming that $v$ is normalized)
%
$$u_0=[r(v)]^2 \overset{\eqref{eq:radius}}= \frac dn,
\qquad 
u_1=\omega(v)\overset{\eqref{eq:cosine_and_length}}=\frac{d\theta}{2|E|}.$$
%
The initial conditions only depends on $d$, $\theta$ and the intersection array of $G$, and consequently, so does $u_\delta$ as a whole.

\emph{Step 2}:
The initial conditions are linear in $d$.
Also, the recurrence \eqref{eq:recurrence} is linear, and thus, all entries of $u_\delta$ are linear in $d$.
Thus if $u\in\RR^n$ is the cosine vector, then $u':=u/d$ is a vector in the arrangement space of $v$ that %depends only on $\theta$ and the intersection array.
Also, $u'$ is contained in the arrangement space of $G$.

%Consider the vector $w\in\RR^n$ defined by its components $w_i:=\<v_1,v_i\>/d$ for all $i\in V$.
%This vectors is contained in the arrangement space of $v$ (see \cref{res:realizations_and_arrangement_spaces} $(ii)$).
%The~\mbox{$i$-th~compo}\-nent of $w$ equals $u_{\dist(1,i)}/d$, which, after dividing~out $d$, is determined only by $G$ and $\theta$.

Since $v$ was chosen arbitrarily, we found that $u'$ is contained in the arrangement space of every distance-transitive realization of $G$ with eigenvalue $\theta$.

\emph{Step 3}:
Fix a distance-transitive group $\Sigma\subseteq\Aut(G)$.
The eigenspace~$\Eig_G(\theta)$ is $\Sigma$-invariant, and decomposes as $\Eig_G(\theta)=$ $U_1\oplus\cdots\oplus U_m$ into \mbox{mutually} orthogonal irreducible $\Sigma$-invariant subspaces $U_i\subseteq\Eig_G(\theta)$.
Each of the $U_i$ is the arrangement space of a distance-transitive realization of $G$ with eigenvalue $\theta$, hence, each one contains the vector $u'\in\RR^n$ defined in step 2.
Since the $U_i$ are mutually orthogonal, that is, disjoint, this can only be if $m=1$ and $\Eig_G(\theta)=U_1$.

We found that $\Eig_G(\theta)$ is irreducible \wrt\ any distance-transitive $\Sigma\subseteq\Aut(G)$, and thus, every distance-transitive realization $v$ with eigenvalue $\theta$ must be irredu\-cible.
Also, its arrangement space must be all of $\Eig_G(\theta)$ and $v$ is the $\theta$-realization of~$G$.
\end{proof}

On the level of arrangement spaces, the previous lemma states that all eigenspaces of $G$ are irreducible invartiant subspaces \wrt\ to every distance-transitive group $\Sigma\subseteq\Aut(G)$.

But are the eigenspaces the only irreducible invariant subspaces?
In terms of realizations the question can be phrased as whether there is a flexible distance-transitive realization.
We do not have an answer to this in the general case.
We can give an answer in certain special cases, \eg\ when $\diam(G)=2$.


\begin{corollary}
For every distance-transitive group $\Sigma\subseteq\Aut(G)$ of symmetries of $G$, the eigenspace of $G$ are $\Sigma$-invariant subspaces of $\RR^n$.
%In particular, all distance-transitive $\Sigma\subseteq\Aut(G)$ have the same invariant subspaces.
\end{corollary}

%The distance-transitive symmetries of a graph seem to be a kind of 

\begin{corollary}
It is not possible to realize the distance-transitive symmetries of $G$ in separation.
More formally, any distance-transitive realization of $G$ automatically realizes \ul{all} the symmetries of $G$.
\end{corollary}

\begin{example}\label{ex:dodecahedron_irreducible}
In \cref{ex:not_full_local_dim} we used that all spectral realizations of the edge-graph of the dodecahedron are irreducible.
This follows from \cref{res:distance_transitive_eigenvalue_implies_spectral} and the fact that this edge-graph is distance-transitive. 
\end{example}

\begin{remark}
The proof of \cref{res:distance_transitive_eigenvalue_implies_spectral} suggests a generalization to groups $\Sigma\subseteq\Aut(G)$ that do not act distance-transitively, but which still act transitively the $D_\delta$ where $\delta\in \{0,...,\hat\delta\}=:\Delta$ comes from an initial segment $\Delta$ of $\{0,...,\diam(G)\}$.

Suppose that not every balanced $\Sigma$-realization of $G$ is spectral.
Than we can assume that there are two irreducible balanced $\Sigma$-realizations $v$ and $v'$ to the same eigenvalue and with orthogonal arrangement spaces.
Then their cosine vectors $u,u'\in\RR^n$ agree in all the components associated with distances $\delta\in\Delta$, but also satisfy $\<u,u'\>=0$.
These are opposing restrictions on this pair of vectors.

Suppose $u=(\check u, \hat u)$ and $u'=(\check u,\hat u')$ so that $u$ and $u'$ agree on the components in $\check u$, but disagree on the components in $\hat u$ \resp\ $\hat u'$.
Then the orthogonality condition above implies
%
\begin{equation}\label{eq:orthogonal}
0 = \<u,u'\> = \|\check u\|^2 +\<\hat u,\hat u'\>\quad\implies\quad \<\hat u,\hat u'\> = -\|\check u\|^2<0.
\end{equation}
%
For normalized realizations we have $\|u\|^2=\|\check u\|^2+\|\hat u\|^2=1$ and respectively for $u'$.
Conclusively, if $\|\check u\|^2> 1/2$ then \eqref{eq:orthogonal} cannot be satisfied.
\end{remark}

%\begin{example}
%The \emph{Shrikande graph} is the smallest distance-regular graph that is not distance-transitive.
%However, it is still arc-transitive, that is, $\Aut(G)$ acts transitively on $D_0$ and $D_1$.
%
%The spectrum of $G$ is $\{(-2)^9,2^6,6^1\}$.
%In particular, the smallest eigenvalue $-2$ has a suspiciously large multiplicity and we are going to check whether the eigenspace decomposes into several irreducible invariant subspaces.
%\end{example}

%\begin{example}
%The eigenspaces of an arc-transitive graph with $\diam(G)=2$ are irreducible \wrt\ any arc-transitive group $\Sigma\subseteq\Aut(G)$.
%\end{example}


\fi




\iffalse

As in the arc-transitive case, we have to assume rigidity to show that $v$ is spectral.
Of course, full local dimension is sufficient to imply all the nice properties as it did in \cref{res:full_local_dimension_is_good}.
More generally, for distance-transitive realizations it would~be~suffi\-cient to show that
%
$$\{ v_j-v_i\mid j\in N_\delta(i)\}$$
%
spans $\RR^d$ for just one $\delta\in\{1,...,\diam(G)\}$, but we were not able to do this.

%Since flexible realizations can be found somewhere \enquote{in the middle} of a transition between two realizations with eigenvalue,

Since the eigenspaces of a distance-transitive graph are exactly the invariant subspaces of every distance-transitive realization of it, it would also be enough to show that all eigenspaces have different dimension, so that no two spectral realizations exist to transition between.

This is not the case in general, but already shows that some cases must be rigid. 
For example, every distance-transitive graph with an even number of vertices and diameter two has three eigenvalues.
One of which is simple, and the other two cannot be of the same multiplicity.
However, graphs with $\diam(G)=2$ can be excluded more generally.



\begin{theorem}
If $G$ is distance-transitive (or distance-regular), then
\begin{myenumerate}
\item
$G$ has exactly $\diam(G)+1$ distinct eigenvalues.
\item
$\Spec(G)\subset[-\deg(G),\deg(G)]$.
\item
$\theta\in \Spec(G)$ has multiplicity one, if and only of $\theta\in\{\pm\deg(G)\}$.
\end{myenumerate}
\end{theorem}



A \emph{sign change} in the cosine sequence is a pair of distances $\delta_1,\delta_2\in\{0,...,\diam(G)\}$, $\delta_1<\delta_2$, so that $u_{\delta_1}\!\cdot u_{\delta_2}<0$ and $u_\delta=0$ for all $\delta$ with $\delta_1<\delta<\delta_2$.

\begin{theorem}[\cite{...}, Theorem 1.12]
\label{res:sign_changes}
If $v$ is the $\theta_k$-realization of a distance-transitive (actually, distance-regular) graph, then the cosine sequence of $v$ has exactly $k-1$ sign changes.
\end{theorem}


The result above applies if we already know that the distance-transitive realization has an eigenvalue.
As for arc-transitive realizations, it is not clear whether there is any irreducible distance-transitive realization without an eigenvalue.
We can prove this the existence of an eigenvalue in certain special cases.

\begin{proposition}\label{res:multiplicity}
If any two eigenvalues of $G$ have distinct multiplicities, then~any irreducible distance-transitive realization of $G$ is rigid and has an eigenvalue.
%
\begin{proof}
\TODO
\end{proof}
\end{proposition}

A distance-transitive graph $G$ of diameter two has only three distinct eigenvalues, one of which has multiplicity one.
If the graph has an even number of vertices, then the other eigenvalues cannot have the same multiplicity and \cref{res:multiplicity} applies.

Thus, for example, the distance-transitive realizations of the Petersen graph are rigid and have an eigenvalue.


\begin{proposition}
If $\diam(G)=2$, then every irreducible distance-transitive realization $v$ of $G$ is rigid and has an eigenvalue.
%
\begin{proof}
It suffices to show that $v$ is rigid. 
Since $v$ is irreducible, having an eigenvalue then follows via \cref{res:rigid_implies_eigenvalue}.

If $\diam(G)=2$, then $\Spec(G)=\{\deg(G)=\theta_1>\theta_2>\theta_3\}$.
The largest eigenvalue is always simple and gives a 1-dimensional realization which is always rigid.

Since $\theta_1$ is always simple, and 1-dimensional realizations are always rigid, hence spectral, the only way $G$ could be flexible would be if $\theta_2$ and $\theta_3$ have the same dimension $\delta\ge 2$.

If there exist distance-transitive realizations of $G$ without eigenvalue, then they are of the form $\alpha v^2+\beta v^3$, where $v^i$ is the $\theta_i$-realization. In particular, $[0,1]\ni t\mapsto v(t):=t v^2+(1-t) v^3$ gives a continuous transition between these two spectral realization.

Let $u_\delta^i$ be the cosine sequence of $v^i$. Then by \cref{res:sign_changes}
%
$$u_0^2 \ge u_1^2 \ge u_2^2\quad\text{and}\quad u_0^3 \ge u_2^3\ge u_1^3.$$
%
Consequently, there must be a $t\in[0,1]$, so that the cosine sequence $u(t)$ of $v(t)$ has $u_1(t)=u_2(t)$.

This can be interpreted as follows: for every vertex $i\in V$, all $v_j,j\in V\setminus\{i\}$ are contained in a hyperplane $\mathcal H_i$ parallel to $v_i^\bot$.
Since $v$ is full-dimensional, we can choose a basis $v_{i_1},...,v_{i_d}$ of $\RR^d$, and the intersection of all $\mathcal H_{i_k}$ is a point $p\in\RR^d$.
So all vertices, except for maybe the $v_{i_k}$, must be in $p$.
\end{proof}
\end{proposition}

\fi

%\begin{theorem}
%Each distance-transitive realization is a spectral realization.
%%
%\begin{proof}
%We proceed in several steps.
%
%\emph{Step 1}: For a vertex $i\in V$, let
%$N_\delta(i):=\{j\in V\mid \dist(i,j)=\delta\}$ denote~the~set~of vertices at distance $\delta$ from $i$.
%Because of distance-transitivity, the cardinality of the intersection $N_{\delta_1}(i)\cap N_{\delta_2}(j)$ does only depend on $\delta_1,\delta_2$ and $\dist(i,j)$, but not on the choice of the involved vertices.
%So for two vertices $i,j\in V$ with $\dist(i,j)=\delta$~we can then define
%%
%$$
%a_\delta:=|N_{\delta-1}(i)\cap N_{1}(j)|,\quad
%b_\delta:=|N_{\delta}(i)\cap N_{1}(j)|,\quad
%c_\delta:=|N_{\delta+1}(i)\cap N_{1}(j)|.
%$$
%%
%Note that $a_\delta+b_\delta+c_\delta=|N_\delta(i)|$.
%
%\emph{Step 2}:
%Again, because of distance-transitivity, the value of $\<v_i,v_j\>$ only depends on $\dist(i,j)$. Consequently, we can define the so-called \emph{cosine sequence} $u_\delta$ for~$\delta\in\{0,...,\diam(G)\}$ of $v$, that is $u_\delta=\<v_i,v_j\>$ whenever $\dist(i,j)=\delta$.
%We now show that $u_\delta$ of a realization with eigenvalue $\theta$ only depends on $\theta,a_\delta,b_\delta$ and $c_\delta$.
%
%Let $i,j\in V$ with $\dist(i,j)=\delta$. Then
%%
%$$\sum_{\mathclap{k\in N(j)}} v_k = \sum_{\mathclap{k\in N_{\delta-1}(i)\cap N(j)}} v_k.$$
%\end{proof}
%\end{theorem}
